Finite-time Non-overshooting Leader-following Consensus Control for Multi-Agent Systems

This paper addresses the finite-time non-overshooting leader-following consensus problem for multi-agent systems, whose agents are modeled by a dynamical system topologically equivalent to the integrator chain. Based on the weighted homogeneity, a nonlinear consensus control protocol is designed. A tuning scheme ensures the finite-time stability of the consensus error such that the agents do not have overshoots in the first component of the state vector. Simulations are presented to demonstrate the effectiveness of the proposed design.

==> Revised_paper_0119/data/III_Problem_Formulation.tex <==
\section{Problem Formulation}\label{PF}

Consider a MAS composed of $N\!\!+\!\!1$ agents, characterized by the agent dynamics, the transmitted data, and the communication network, as Fig. \ref{fig:transmission}. 

\subsubsection{Agent dynamics}
the agent dynamics is as follows
\begin{equation}\label{eq:dynamic}
\begin{aligned}
 &\dot x_{i}(t)\!\!=\!\!Ax_i(t)\!\!+\!\!Bu_i(t),\;\; i\!\!=\!\!\overline{0,N}, \;\;t\!\!\in\!\!\R_+ \\
 &A\!\!=\!\!\left(\begin{smallmatrix}
      \textbf{0}_{n-1} & I_{n-1}  \\
       0  & \textbf{0}_{n-1}^\top
 \end{smallmatrix}\right), \quad B\!\!=\!\!\left(\begin{smallmatrix}
      \textbf{0}_{n-1}   \\
       1  
 \end{smallmatrix}\right),
\end{aligned}
\end{equation}
where $x_0\!\!\in\!\!\R^n$ is the state of the leader, with $u_0\!\!=\!\!0$; and $x_i\!\!\in\!\!\R^n$, $i\!\!=\!\!\overline{1,N}$ be the state of followers, with $u_i\!\!\in\!\!\R$, $i\!\!=\!\!\overline{1,N}$ be the control input to be designed. 


\subsubsection{Transmitted data} the transmitted data of agent $i$ is $(x_i,v_i)\!\!\in\!\!\R^{n}\!\!\times\!\!\R^n$, where $v_i\!\!:=\!\!f_{v_i}(x_i,x_{j_1},\dots,x_{j_{n_i}},v_{j_1},\dots,v_{j_{n_i}})$, $f_{v_i}\!:\!\R^{n}\!\!\times\!\!\R^{n_in}\!\!\!\times\!\!\R^{n_in}\!\!\to\!\!\R^{n}$, $n_i$ is the number of agents which could convey information to agent $i$. 


\begin{remark}
  If $v_i$, $\forall i\!\!=\!\!\overline{0,N}$ be unavailable, the setting corresponds to some classical configurations of MAS \cite{olfati2004consensus,zhu2023robust,9285180}; a quasi-decentralized configuration is achieved by letting $v_0\!\!=\!\!0$, $v_1(t)\!\!=\!\!\ldots\!\!=\!\!v_N(t)\!\!=\!\!u_g(t)$, $u_g\!:\!\R\!\!\to\!\!\R$ \cite{li2023generalized}; 
in addition, \cite{ning2020bipartite, hong2006tracking,ren2007multi,liu2011synchronization} report a distributed design with $v_{j_l}\!\!=\!\!u_{j_l}$, $l\!\!=\!\!\overline{1,{n_i}}$, $i\!\!=\!\!\overline{1,N}$. The extension of the transmitted data with the vector $v_i$ helps agents gather more information useful for control design.  
\end{remark}
 

\subsubsection{Communication network}
the communication network is described by a fixed and directed graph, and denoted by $\mathcal{G}\!\!=\!\!\{\mathcal{V},\mathcal{E},\mathcal{W}\}$. Here, $\mathcal{V}\!\!\!=\!\!\!\{\overline{0,N}\}$ represents the set of vertices, with vertex $0$ (the leader) serving as the root and vertices $\overline{1,N}$ (followers) serving as the terminals of at least one directed path originating from the root. Detailed definitions on $\mathcal{V}$, $\mathcal{E}$, and $\mathcal{W}$ are presented further on (Section \ref{GT}). Regarding this graph, we have $v_0\!\!=\!\!\textbf{0}_n$. 



\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.7\linewidth]{transmission.pdf}
    \caption{The configuration of the MAS: agent $i$, $i\!\!=\!\!\overline{1,N}$ receives the transmitted data $(x_{j_l},v_{j_l})\!\!\in\!\!\R^n\!\!\times\!\!\R^n$, $l\!\!=\!\!\overline{1,n_i}$, and send out $(x_i,v_i)\!\!\in\!\!\R^n\!\!\times\!\!\R^n$. }
    \label{fig:transmission}
\end{figure}

\subsubsection{Control problem}
regarding the MAS defined above, we introduce some new definitions based on the classical leader-following consensus introduced in \cite{ni2010leader}. 

\begin{Def}\label{def:lf_consensus}
    \textit{Let $e\!\!=\!\!(e_1^\top\!\!,\dots,e_N^\top\!)^\top$ with 
$e_i\!\!=\!\!x_i\!\!-\!\!x_0$  be the consensus error.
The MAS \eqref{eq:dynamic} with some  $u_i$, $i\!\!=\!\!\overline{1,N}$ achieves}
\\
    % $\bullet$ \textit{asymptotic consensus \cite{ni2010leader} if 
    % $\lim_{t\!\to+\infty}\|e(t)\|\!\!=\!\!0$, $\forall e(0)\!\!\in\!\!\R^{Nn}$};\\
    % $\bullet$ \textit{finite-time consensus \cite{wang2010finite} if there exists locally bounded settling time function $T\!:\!\R^{Nn}\!\to\!\R_+$ such that
    %     $\lim_{t\!\to\!T(e(0))}\|e(t)\|\!\!=\!\!0$, $\forall e(0)\!\!\in\!\!\R^{Nn}$;}
    a) \textit{finite-time \cite{wang2010finite} (resp., asymptotic \cite{ni2010leader}) consensus  if $\lim_{t\!\to T}\|e(t)\|\!\!=\!\!0$, $\forall e(0)\!\!\in\!\!\R^{Nn}$, $T\!\!=\!\!T_c(e(0))$  (resp., $T\!\!=\!\!+\infty$);}
    % $\bullet$ fixed-time consensus if finite-time consensus is achieved and the settling time function is globally bounded i.e., $T(x_i(0)\!-\!\!x_0(0))\!\!\leq\!\!T_{max}$, $i\!\!=\!\!\overline{1,N}$, $T_{max}\!\!>\!\!0$ is independent on the system state;  
% $\bullet$ \textit{practical fixed-time consensus if there exists $T_r\!\!>\!\!0$ such that 
% \begin{equation}\label{eq:def_pfx_lfconsensus}
%         \lim_{t\!\to\!T_r}\|x_i(t)\!\!-\!\!x_0(t)\|\!\!\leq\!\!r,\;\; \forall i\!\!=\!\!\overline{1,N}
%     \end{equation}
%     for any $x_i(0)\!\!\in\!\!\R^n$, $i\!\!=\!\!\overline
%     {0,N}$ and $\forall r\!\!>\!\!0$, where $T_r$ is independent on the system state;}  
    % $\bullet$ non-asymptotic consensus if finite-time$\backslash$fixed- time$\backslash$practical fixed-time consensus is achieved; 
    % $\bullet$ \textit{distributed consensus if a consensus defined above is achieved and $u_i$ is dependent only on the local information of agent $i$; }
    \\
b) \textit{finite-time (resp., asymptotic) non-overshooting consensus if the finite-time (resp., asymptotic) consensus is achieved and there exists a non-empty set $\Omega\!\!\subset\!\!\Sigma\!\!:=\!\!\{e\!\!\in\!\!\R^{Nn}\!:\!(I_N\!\!\otimes\!\!\eta_1^\top)e\!\!\leq\!\!{0}\}$ being strictly positively invariant for the error system.
            % for all $x_{i,1}(0)\!\!-\!\!x_{0,1}(0)\!\!\leq\!\!0$, $x_{i,1}(t)\!\!-\!\!x_{0,1}(t)\!\!\leq\!\!0$, $\forall t\!\!>\!\!0$, $\forall i\!\!=\!\!\overline{1,N}$.
            }
\end{Def}
\begin{remark}
  The positive invariance of $\Omega$ guarantees the non-overshooting stabilization of $e$ if $e(0)\!\!\in\!\!\Omega$. In other words, if the follower’s first state component is initially behind the leader, this condition guarantees this behindness in the transient phase of reaching consensus.   
\end{remark}

The problem of finite-time/asymptotic non-overshooting consensus is inspired by the practical reason of safety-critical control systems \cite{ames2016control}, with its notion drawn from the theory of non-overshooting stabilizers \cite{krstic2006nonovershooting,polyakov2023finite}. To address this problem, this paper  extends the concept of non-overshooting (safety) control to MAS by a proper design of a transmitted vector $v_i\!\!=\!\!f_{v_i}(x_i,x_{j_1},\dots,x_{j_{n_i}},v_{j_1},\dots,v_{j_{n_i}})$, $i\!\!=\!\!\overline{1,N}$ and a distributed control protocol $u_i\!\!=\!\!f_{u_i}(v_i)$, $f_{u_i}\!:\!\R^{n}\!\!\to\!\!\R $,
$i\!\!=\!\!\overline{1,N}$ such that the closed-loop error equation 
\begin{equation}\label{eq:nonovershooterrordy}
    \dot e\!\!=\!\! f(e),\;\; f\!:\!\R^{Nn}\!\!\to\!\!\R^{Nn}
\end{equation}
is globally finite-time\footnote{The system $\dot{x}(t)\!\!=\!\!f(x(t))$, $t\!\!\in\!\!\R_+$, $x(0)\!\!=\!\!x_0\!\!\in\!\! \R^n,$ is globally finite-time stable \cite{orlov2004finite} if it is Lyapunov stable \cite{khalil2009lyapunov} and there exists a settling-time function $T(x_0)$, $T\!\!:\!\!\mathbb{R}^{n}\!\!\to\!\!\mathbb{R}_+$ such that $\|x(t)\|\!\!=\!\!0$,  $\forall t\!\!\geq\!\! T(x_0)$. } (asymptotically) stable, and properly
designed a non-empty set $\Omega\!\!\in\!\!\Sigma$  is strictly positively invariant for the error equation \eqref{eq:nonovershooterrordy}. 

\begin{remark}
    The consensus control protocol obtained in resolving the above-defined problem is valid for the MAS with nonlinear agent dynamics 
    \begin{equation*}
    \left\{\begin{array}{ll}
        \!\!\!\dot x_i\!\!=\!\!f_s(x_i,u_i),  \\
         \!\!\!y_i\!\!=\!\!f_o(x_i,u_i),
    \end{array}\right.f_s\!\!:\!\!\R^n\!\!\times\!\!\R^m\!\!\to\!\!\R^n, \;\;f_o\!\!:\!\!\R^n\!\!\times\!\!\R^m\!\!\to\!\!\R^o,\;\;i\!\!=\!\!\overline{0,N}
    \end{equation*}
    % provided that there exists a coordinate transformation such that the latter system be transformed into the chain of integrator, \textit{i.e.,}
    which is topologically equivalent \cite{isidori1985nonlinear} to the dynamics \eqref{eq:dynamic}. 
\end{remark}















 




































==> Revised_paper_0119/data/II_Preliminaries_generalized_homogeneity_graph_theory.tex <==
\section{Preliminaries}\label{Pre}
\subsection{Elements of Graph Theory}\label{GT}
A fixed directed graph $\mathcal{G}$ is characterized by the   \textit{vertex set} $\mathcal{V}$, the \textit{edge set}
$\mathcal{E}$ and the \textit{weighted adjacency matrix}
$\mathcal{W}$. Specifically, the vertex set
$\mathcal{V}\!\!=\!\!\{\overline{1,N}\}$ is a collection of all nodes at the graph indexed by $i\!\!=\!\!\overline{1,N}$. The edge set
$\mathcal{E}\!\!=\!\!\{(i,j)|i,j\!\!\in\!\! \mathcal{V}\}$, $(i,j)\!\!\in\!\! \mathcal{E}$ if node $j$ could transfer its local information to node $i$; $n_i$ denotes the number of incoming edges of node $i$. The weighted adjacency matrix
$\mathcal{W}\!\!=\!\!\{w_{ij}\}\!\!\in\!\!\R^{N\!\times\!N}$, with $w_{ij}$, $i,j\!\!\in\!\!\mathcal{V}$, $w_{ij}\!\!=\!\!1$ if $(i,j)\!\!\in\!\! \mathcal{E}$, and $w_{ij}\!\!=\!\!0$ otherwise. 
The \textit{self-loop} is excluded in this paper, \textit{i.e.,} $w_{ii}\!\!=\!\!0$.
The \textit{Laplacian matrix} associated to the graph $\mathcal{G}$ is defined as $\mathcal{L}\!\!=\!\!\{l_{ij}\}\!\!\in\!\!\R^{N\!\times\!N}$, where $l_{ij}\!\!=\!\!-w_{ij}$ for $i\!\!\neq \!\!j$, and $l_{ij}\!\!=\!\!\sum^N_{k=1}\!\!w_{ik}$ for $i\!\!=\!\!j$.
The latter immediately implies that $\sum_{j=1}^N\!\!l_{ij}\!\!=\!\!0$, $\forall i\!\!=\!\!\overline{1,N}$.
A \textit{directed path} from vertex $j$ to vertex $i$ is formulated if 
 there is a sequence of vertices $\overline{i_1, i_s}$, with $i_1\!\!=\!\!j$, $i_s\!\!=\!\!i$ and $(i_{\iota+1},i_\iota)\!\!\in\!\!\mathcal{E}$, $\iota\!\!=\!\!\overline{1,s\!\!-\!\!1}$, $2\!\!\leq\!\!s\!\!\in\!\!\mathbb{N}_+$. 
 If there exists a vertex $i_r$ has at least one directed path from itself to any one of the rest nodes while $(i_r,j)\!\!\notin\!\!\mathcal{E}$, $\forall j\!\!\in\!\!\mathcal{V}$,  
we call $i_r$ the \textit{root}. 
The graph connected and acyclic is called the \textit{tree}.
The tree with a unique root and where every other vertex has exactly one incoming edge is called the \textit{directed spanning tree}. The directed graph with a unique root contains a directed spanning tree, and the associated Laplacian matrix has one simple zero eigenvalue while all others have positive real parts \cite{ren2005consensus}.
\begin{lem}\label{lem:unique}
    \textit{Let $\mathcal{G}_{lf}\!\!=\!\!\{\mathcal{V}_{lf},\mathcal{E}_{lf},\mathcal{W}_{lf}\}$ denote a directed graph with a unique root labeled by $0$, where $\mathcal{V}_{lf}\!\!=\!\!\{\overline{0,N}\}$, $\mathcal{W}_{lf}\!\!=\!\!\{w_{ij}\}\!\!\in\!\!\R^{(N\!+\!1)\!\times\!(N\!+\!1)}$, and
the associated Laplacian matrix be  $\mathcal{L}\!\!=\!\!\{l_{ij}\}\!\!\in\!\!\R^{(N\!+\!1)\!\times\!(N\!+\!1)}$. Then }
\\
 a)\textit{
there exists an invertible matrix $E\!\!\in\!\!\R^{(N+1)\!\times\!(N+1)}$ such that 
$$E^{-1}\!\!\mathcal{L}E
    \!\!=\!\!\left(\begin{smallmatrix}
    0 & \textbf{0}_N^\top\\
    \textbf{0}_N & \TL
    \end{smallmatrix}\right),$$ with $\TL\!\!\in\!\!\R^{N\!\times\!N}$ being invertible.}
% the matrix
% \begin{equation}\label{eq:TL}
%     \TL\!\!=\!\!\left(\begin{smallmatrix}
%         l_{11} & \dots & l_{1N}\\
%         \vdots & \ddots & \vdots\\
%         l_{N1} & \ldots & l_{NN}
%         \end{smallmatrix}\right)\!\!\in\!\!\R^{N\!\times\!N},
% \end{equation}
% which is reduced from the $\mathcal{L}$ by eliminating the first line and the first column, has full rank. }
\\ 
b)\textit{ the algebraic equation $\omega_0\!\!=\!\!\textbf{0}_m$,
 \begin{equation}\label{eq:lin_alge}
 	\omega_i\!\!=\!\!\tfrac{1}{\sum_{j=0}^N\!\!w_{ij}}\sum\nolimits_{j=0}^N\!\! w_{ij}\!\!\left(M(x_i\!\!-\!\!x_j)\!\!+\!\!\omega_j\right), \;M\!\!\in\!\! \R^{m\times n}, \omega_i\!\!\in\!\!\R^m,i\!\!=\!\!\overline{1,N}
 \end{equation}
has a unique solution, where $w_{ij}\!\!\in\!\!\R$ is the element of the matrix $\mathcal{W}_{lf}$, and $x_i$, $i\!\!=\!\!\overline{0,N}$ is the state vector of MAS \eqref{eq:dynamic}.  }
\end{lem}


\begin{proof}
Claim a) is obtained by referring the Lemma 3 of \cite{guan2012impulsive} with $l_{0j}\!\!=\!\!0$, $\forall j\!\!=\!\!\overline{0,N}$ since the root is labeled by $0$. 
% Since $\mathcal{G}_{lf}$ is a directed graph with a unique root, then the associated Laplacian matrix $\mathcal{L}$ has a simple zero eigenvalue with all others having positive real parts. In addition, since the root is labeled by $0$, then $l_{0j}\!\!=\!\!0$, $\forall j\!\!=\!\!\overline{0,N}$. Let the invertible matrix $E\!\!=\!\!\left(\begin{smallmatrix}
%     1 & \textbf{0}_{N}^\top  \\
%          \textbf{1}_{N} & I_N
% \end{smallmatrix}\right)$, then
% \begin{equation*}
%     E^{-1}\!\!\mathcal{L}E\!\!=\!\!\!\!\left(\begin{smallmatrix}
%         0 & l_{01} & \ldots & l_{0N} \\
%         0 & l_{11}\!-\!l_{01} & \ldots & l_{1N}\!-\!l_{0N} \\
%         \vdots & \vdots & \ddots & \vdots \\
%         0 & l_{N1}\!-\!l_{01} & \ldots & l_{NN}\!-\!l_{0N} \\
%     \end{smallmatrix}\right)\!\!
%     \!\!=\!\!\!\left(\begin{smallmatrix}
%     0 & \textbf{0}_N^\top\\
%     \textbf{0}_N & \TL
%     \end{smallmatrix}\right).
% \end{equation*}
% The latter shows the eigenvalues of $\TL$ corresponding to the non-zero eigenvalues of $\mathcal{L}$. The first claim is proven. 

For claim b), rewrite \eqref{eq:lin_alge}, with $\omega_{0}\!\!=\!\!\textbf{0}_m$, as 
 \begin{equation*}\begin{aligned}
 	% \sum\nolimits_{j=0}^Nw_{ij}\omega_i\!\!-\!\!\sum\nolimits_{j=0}^N w_{ij}\omega_j\!\!&=\!\!-\sum\nolimits_{j=0}^N w_{ij}M(x_j\!\!-\!\!x_i),\\
  \sum\nolimits_{j=0}^Nw_{ij}\omega_i\!\!-\!\!\sum\nolimits_{j=1}^N w_{ij}\omega_j\!\!&=\!\!-\!\!\sum\nolimits_{j=0}^N w_{ij}M(x_j\!\!-\!\!x_i).
  %\TL u\!\!&=\!\!-(\TL\!\otimes\!K) e,
  \end{aligned}\end{equation*}
The latter is equivalent to $\TL_i \omega\!\!=\!\!(\TL_i\!\otimes\!M) e$, 
yielding a compact form $\TL \omega\!\!=\!\!(\TL\!\!\otimes\!\!M) e$, $\omega\!\!=\!\!(\omega_1^\top,\dots, \omega_N^\top)^\top$, $\TL_i$ is the $i_{th}$ line of $\TL$. Since $\TL$ is invertible the latter algebraic equation has a unique solution $\omega\!\!=\!\!(I_N\!\!\otimes\!\!M) e$. The proof is completed. 
\end{proof}

% \subsection{stability notions}

% Consider an autonomous system 
% \begin{equation}\label{eq:stab_def}
%     \dot{x}(t)\!\!=\!\!f(x(t),q(t)),\;\;  \; x\!\!\in\!\! \R^n,\;t\!\!>\!\!0,\;  q\!\!\in\!\!\R^p
% \end{equation}
% where $f\!:\!\R^n\!\!\times\!\!\R^p\!\!\to\!\!\R^n$ is a continuous vector field satisfying $f(\textbf{0},\textbf{0})\!\!=\!\!\textbf{0}$. Let $S(t,x(0))$ be the solution of \eqref{eq:stab_def}, $\forall x(0)\!\!\in\!\!\R^n$.
% \begin{Def}
% \textit{Let $q\!\!=\!\!\textbf{0}$, the origin of the system \eqref{eq:stab_def}
% is globally finite-time stable \cite{orlov2004finite} if it is Lyapunov stable \cite{khalil2009lyapunov} and for all $x(0)\!\!\in\!\! \R^n$, there exists a locally bounded settling-time function $T\!:\!\mathbb{R}^{n}\!\!\to\!\!\mathbb{R}_{+}$, such that $\|S(t,x(0))\|\!\!=\!\!0$, $\forall t\!\!>\!\!T(x(0))$.}

% $\bullet$ \textit{Lyapunov stable \cite{khalil2009lyapunov} if for all $\epsilon\!\!>\!\!0$, there exists $\delta\!\!=\!\!\delta(\epsilon)\!\!>\!\!0$ such that $\|x(0)\|\!\!<\!\!\delta\!\!\Rightarrow\!\!\|S(t,x(0))\|\!\!<\!\!\epsilon$, $\forall t\!\!>\!\!0$;}

% $\bullet$ \textit{globally finite-time stable \cite{orlov2004finite} if it is Lyapunov stable \cite{khalil2009lyapunov} and for all $x(0)\!\!\in\!\! \R^n$, there exists a locally bounded settling-time function $T\!:\!\mathbb{R}^{n}\!\!\to\!\!\mathbb{R}_{+}$, such that $\|S(t,x(0))\|\!\!=\!\!0$ for all $t\!\!>\!\!T(x(0))$;}

% $\bullet$ \textit{globally fixed-time stable \cite{polyakov2011nonlinear} if it is globally finite-time stable and there exists $T_{\max}\!\!>\!\!0\!:\!T(x(0))\!\!\leq\!\!T_{\max}$, $\forall x(0)\!\!\in\!\!\R^n$, where $T_{\max}$ is independent of $x(0)$;}

% $\bullet$ \textit{globally practical fixed-time stable \cite{polyakov2020generalized} if it is Lyapunov stable and for all $r\!\!>\!\!0$, there exists $T_r\!\!>\!\!0\!:\!\|S(t,x(0))\|\!\!\leq\!\!r$, $\forall t\!\!\geq\!\!T_r$, where $T_r$ is independent of $x(0)$. } 
% \end{Def}
% \begin{Def}\cite{sontag1989tac}
% \textit{Let $q\!\!\neq\!\!\textbf{0}$, system \eqref{eq:stab_def} is said to be input-to-state stable (ISS)    if there exist $\beta\!\!\in\!\! \mathscr{KL}$ and $\gamma\!\!\in\!\!\mathscr{K}$ such that}
% 	\begin{equation*}
% 	    \|x(t)\|\!\!\leq\!\! \beta\left(\|x(0)\|,t\right)\!\!+\!\!\gamma\left(\|q\|_{L^{\infty}}\right),\;\;
% 	 \forall x(0)\!\!\in\!\! \R^n, \;\forall q\!\!\in\!\! L^{\infty}(\R,\R^p).
% \end{equation*}
% \end{Def}


\subsection{Elements of Homogeneity Theory}
Homogeneity describes the \textit{symmetry} with respect to a transformation called \textit{dilation}. For example, let a function $h\!:\!\R^n\!\!\to\!\!\R$, whose homogeneity is represented as $\exists\mu\!\!\in\!\!\R$ such that $h(\exp(s)x)\!\!=\!\!\exp(\mu s)h(x)$, $\forall s\!\!\in\!\!\R$. In this example, the argument $x$ is uniformly scaled by $\exp(s)$, which is the simplest case of dilation. However, consider a non-uniform scaling on $x$, which can be denoted as $x\!\!\to\!\!\dn(s)x$, where $\dn(s)$ is an operator maps $\R^n$ to $\R^n$, $\forall s\!\!\in\!\!\R$. To be a dilation, $\dn(s)$ has to satisfy:
\\
$\bullet$ \textit{group property}: $\dn(0)\!\!=\!\!I_n$, and $\dn(a\!\!+\!\!b)\!\!=\!\!\dn(a)\dn(b)$, $a,b\!\!\in\!\!\R$;
\\
$\bullet$ \textit{limit property}: $\lim_{s\rightarrow \pm \infty}\|\mathbf{d}(s)x\|\!\!=\!\!\exp(\pm \infty)$, $x\!\!\in\!\!\R^n\backslash\{ \mathbf{0}\}$.\\
In many cases, we require the continuity of $\dn(s)$, which is determined by the continuity of function $s\!\!\mapsto\!\!\dn(s)x$, $\forall x\!\!\in\!\!\R^n$. We say $\dn(s)$ is a \textit{monotone dilation} if the latter function is strictly increasing \cite{polyakov2020generalized}. The \textit{linear dilation} is defined as
$\mathbf{d}(s)\!\!=\!\!\exp(sG_\dn)$, $s\!\!\in\!\! \mathbb{R}$, $G_\dn\!\!\in\!\!\R^{n\times n}$ is anti-Hurwitz and known as the \textit{generator} of the dilation. Particularly, if
$G_\dn\!\!=\!\!\diag\{r_i\}_{i=1}^n$, $r_i\!\!\in\!\!\R_+$, $i\!\!=\!\!\overline{1,n}$, the generated dilation is called the \textit{weighted dilation}. 
% The dilation can be cataloged into the following types:
% $\bullet$ \textit{standard dilation} [L. Euler, 18th c.]:
% $\mathbf{d}(s)\!\!=\!\!\exp(s)I_n$, $s\!\!\in\!\! \mathbb{R}$;
% $\bullet$ \textit{weighted dilation} \cite{Zubov1957:IVM}: 
% $
% \mathbf{d}(s)\!\!=\!\!\exp(s\cdot\diag\{r_i\}_{i=1}^n)$, $s\!\!\in\!\! \mathbb{R}$ for $r_i\!\!>\!\!0$, $i\!\!=\!\!\overline{1,n}$,
% $\bullet$ \textit{linear dilation} \cite{polyakov2020generalized}:
% $\mathbf{d}(s)\!\!=\!\!{\rm exp}(s G_{\dn}),$
%  $s\!\!\in\!\! \mathbb{R}$, $G_{\dn}\!\!\in\!\! \mathbb{R}^{n\times n}$ is an anti-Hurwitz matrix known as the generator of dilation.
% $\bullet$ \textit{geometric dilation} \cite{Khomenuk1961:IVM,Kawski1995:NOLCOS}:
% a flow generated by an unstable vector field.
% It should be noted that the geometric dilation is nonlinear, while the standard dilation and the weighted dilation are the special case of the linear dilation by letting $G_\dn\!\!=\!\!I_n$ and $G_\dn\!\!=\!\!\diag\{r_i\}_{i=1}^n$, respectively. 
% 
The following result supports us in determining a proper $G_\dn\!\!\in\!\!\R^{n\times n}$ for a continuous linear control system $\dot x\!\!=\!\!Ax\!\!+\!\!Bu$, $x\!\!\in\!\!\R^n$, $A\!\!\in\!\!\R^{n\times n}$, $B\!\!\in\!\!\R^{n\times m}$, $u\!\!\in\!\!\R^{m\times n}$.

\begin{lem}\cite{polyakov2020generalized}
\textit{Given $\mu\!\!\neq\!\! 0$, a nilpotent $A\!\!\in\!\!\R^{n\times n}$, and a matrix $B\!\!\in\!\!\R^{n\times m}$ such that $(A,B)$ controllable, then there always exists an anti--Hurwitz matrix $G_{\dn}$ satisfying:
\begin{equation}\label{eq:G_d}
	AG_{\dn}\!\!=\!\!(\mu I_n\!\!+\!\!G_{\dn})A, \quad G_{\dn}B\!\!=\!\!B.
\end{equation}
}
\end{lem}
If $(A,B)$ takes a canonical form as \eqref{eq:dynamic}
then the equation \eqref{eq:G_d} has an explicit solution $G_\dn\!\!=\!\!\diag\{1\!\!-\!\!\mu(n\!\!-\!\!k)\}_{k\!=\!1}^n$, $\mu\!\!<\!\!\tfrac{1}{n-1}$.
Based on the concept of dilation, the homogeneity is defined below.
\begin{Def}\cite{polyakov2020generalized}
	\textit{A vector field $f\!:\! \mathbb{R}^n \!\!\to\!\! \mathbb{R}^n$ (resp., function $h\!:\!\R^n\!\!\to\!\!\R$) is said to be $\dn$-homogeneous if there exists a $\mu\!\! \in\!\! \mathbb{R}$ such that
	\begin{equation*}\begin{aligned}
 \begin{array}{cc}
      f(\dn(s) x)\!\!=\!\!\exp(\mu s) \dn(s) f(x),\;\; \forall s\!\!\in\!\! \mathbb{R},\;\; \forall x \!\!\in\!\! \mathbb{R}^n  \\
      (resp.,\;h(\dn(s) x)\!\!=\!\!\exp(\mu s) h(x),\;\; \forall s\!\!\in\!\! \mathbb{R},\;\; \forall x \!\!\in\!\! \mathbb{R}^n) 
 \end{array}
\end{aligned}\end{equation*}
where $\dn$ is a dilation, $\mu$ is known as the homogeneity degree.}
\end{Def}

One main feature of homogeneous systems is the improved convergence rate characterized by its homogeneity degree $\mu$. 
\begin{lem}\label{lem1}
\textit{Let $f\!:\!\R^n\!\!\to\!\!\R^n$ be a continuous $\mathbf{d}$-homogeneous vector
field of degree $\mu\!\! \in\!\! \mathbb{R}$, and the origin of the system $\dot{x}\!\!=\!\!f(x)$ be globally asymptotically stable. Then the origin of the system $\dot{x}\!\!=\!\!f(x)$ is globally finite-time stable for $\mu\!\!\in\!\!\R_-$.}
\end{lem}



Another important feature of homogeneous systems is the robustness, in the sense of ISS\footnote{Input-to-State Stability. The system $\dot x(t)\!\!=\!\!f(x(t),q(t))$, $x\!\!\in\!\! \R^n$, $q\!\!\in\!\! \R^p$, $t\!\!\in\!\!\R_+$, $x(0)\!\!=\!\!x_0$ is ISS if there exist $\beta\!\!\in\!\! \mathscr{KL}$ and $\gamma\!\!\in\!\!\mathscr{K}$ such that
	\begin{equation*}
	    \|x(t)\|\!\!\leq\!\! \beta\left(\|x(0)\|,t\right)\!\!+\!\!\gamma\left(\|q\|_{L^{\infty}}\right),\;\;
	 \forall x(0)\!\!\in\!\! \R^n, \;\;\forall q\!\!\in\!\! L^{\infty}(\R,\R^p).
\end{equation*}}, with respect to disturbances.
\begin{lem}\cite{polyakov2020generalized}\label{lem:ISS}
\textit{Assume a continuous vector field $f_q\!:\!\mathbb{R}^n\!\!\times\!\!\R^p\!\!\to\!\! \mathbb{R}^{n+p}$ takes the form of
\begin{equation*}
  {f}_q(x,q)\!\!=\!\!\left(
                   \begin{smallmatrix}
                     f(x,q) \\
                     \mathbf{0}_p \\
                   \end{smallmatrix}
                 \right),\;\; x\!\!\in\!\! \mathbb{R}^{n}, \;\; q\!\!\in\!\! L^{\infty}\!(\R,\R^p),\;\;f\!:\!\R^n\!\!\times\!\!\R^p\!\!\to\!\!\R^n
\end{equation*}
and $\dn$-homogeneous of degree $\mu$ with respect to a dilation $\dn\!\!=\!\!\left(
                                             \begin{smallmatrix}
                                               \dn_x & \mathbf{0}_{n\!\times\! p} \\
                                               \mathbf{0}_{p\!\times\! n} & \dn_q \\
                                             \end{smallmatrix}
                                           \right)
$
in $\mathbb{R}^{n+p}$. If the system
%\begin{equation*}
$  \dot x\!\!=\!\!f(x,\mathbf{0})$ %, x(t)\in \mathbb{R}^{n}
%\end{equation*}
is asymptotically stable at the origin, then the system
%\begin{equation*}
$
  \dot x\!\!=\!\!f(x,q)%,\quad q\in L^{\infty}(\mathbb{R},\mathbb{R}^{m})
  $
%\end{equation*}
is ISS.}
\end{lem}





Next, we define the \textit{canonical homogeneous norm}.
\begin{Def}\label{def:hnorm}
	\textit{The functional $\|\cdot\|_{\mathbf{d}}\!:\!\R^n\!\!\to\!\! \R_{\geq0}$ defined as $\|\mathbf{0}\|_{\dn}\!\!=\!\!0$ and
$\|x\|_\mathbf{d}\!\!=\!\!\exp(s_x)$, where $s_x\!\!\in\!\! \mathbb{R}\!:\!\|\mathbf{d}(-s_x)x\|\!\!=\!\!1$, $\mathbf{d}$ is a linear monotone dilation,
	is called the canonical homogeneous norm induced by a norm $\|\cdot\|$ in $\mathbb{R}^n$.}
\end{Def}

The canonical homogeneous norm is not a norm in the usual sense but indeed a norm in $\R^n_{\dn}$ being homeomorphic to $\R^n$ \cite{polyakov2020generalized}. If $\dn(s)\!\!=\!\!\exp(s)I_n$, then, $\|\cdot\|_{\dn}\!\!=\!\!\|\cdot\|$.
Moreover, 
the canonical homogeneous norm has the following properties:
\\
	$\bullet$ homogeneous of degree $1$, {\it i.e.,} $\|\mathbf{d}(s)x\|_\mathbf{d}\!\!=\!\!\exp(s)\|x\|_\mathbf{d}$,  $\forall s\!\!\in\!\! \mathbb{R}$;\\
	$\bullet$  $\|x\|\!\!=\!\!1 \!\!\Leftrightarrow\!\! \|x\|_{\dn}\!\!=\!\!1$;
 \\
	$\bullet$ $\|\cdot\|_{\dn}$ is a locally Lipschitz continuous function on $\R^n \backslash \{\mathbf{0}\}$;
	% $\bullet$ if $\|\cdot\|\!\!\in\!\! \mathcal{C}^{1}(\R^n\backslash\{\mathbf{0}\},\R_{\geq0})$, then $\|\cdot\|_{\dn}\!\!\in\!\! \mathcal{C}^{1}(\R^n\backslash\{\mathbf{0}\},\R_{\geq0})$;
 \\
	$\bullet$ if  $\|x\|\!\!=\!\!\|x\|_P$, where $P\!\!\in\!\!\R^{n\!\times\!n}$ satisfies
	$P\!\!\succ\!\! 0$, $PG_{\dn}\!\!+\!\!G_{\dn}^{\top}P\!\!\succ\!\!0$,
	then, the linear dilation $\dn(s)\!\!=\!\!\exp(sG_{\dn})$ is monotone and
 %for $x\!\!\in\!\!\R^n\backslash\{\mathbf{0}\}$, we have
	\begin{equation*}\label{eq:part-deriv}
		\tfrac{\partial \|x\|_{\dn}}{\partial x}\!\!=\!\!\tfrac{\|x\|_{\dn}x^{\top}\!\dn^{\top}\!(-\ln\!\|x\|_{\dn}) P\dn(-\ln \!\|x\|_{\dn})}{x^{\top}\!\dn^{\top}\!(-\ln \!\|x\|_{\dn})PG_{\dn}\dn(-\ln \!\|x\|_{\dn})x},\;\; x\!\!\in\!\!\R^n\backslash\{\mathbf{0}\}.
	\end{equation*}

% Moreover, the definition of the \textit{homogeneous cone} is introduced as follows.
% \begin{Def}\cite{polyakov2023finite}
%    \textit{ A non-empty set $\Omega\!\!\in\!\!\R^n$ is said to be a $\dn$-homogeneous cone if $x\!\!\in\!\!\Omega\!\!\Rightarrow\!\!\dn(s)x\!\!\in\!\!\Omega$, $\forall s\!\!\in\!\!\R$. }
% \end{Def}

% The latter definition shows that for any $x\!\!\in\!\!\Omega$, the \textit{homogeneous curve} $H_c\!\!:=\!\!\{y\!\!\in\!\!\R^n\!:\!y\!\!=\!\!\dn(s)x,s\!\!\in\!\!\R\}$ belongs to $\Omega$ as well. In particular, if $\dn(s)\!\!=\!\!\exp(s)I_n$, then the homogeneous curve reduces to the \textit{ray} and $\Omega$ reduces to a positive cone in $\R^n$. 

% \subsection{positive system}

% % We first define the non-overshooting consensus.
% % \begin{Def}\label{def:nonovershootconsensus}
% %     \textit{Let $x_{i,1}$ denote the first component of the state variable of agent $i$, $i\!\!=\!\!\overline{1,N}$ at the multi-agent system \eqref{eq:dynamic}. If, for a specified control input $u_i$, $i\!\!=\!\!\overline{1,N}$, $x_{i,1}(t)$ is uniformly bounded by its final value $x_{i,1}(\infty)$, $\forall t\!\!\geq\!\!0$, $\forall i\!\!=\!\!\overline{1,N}$, then multi-agent system \eqref{eq:dynamic} exhibits non-overshooting consensus.}
% % \end{Def}

% %     Definition \ref{def:nonovershootconsensus} can be seen as an extension of the output (state) non-overshoot from the centralized control system to a distributed one,  as reported in Definition 5 of \cite{hollo1985modelling}. 
    
% %     Indeed, Definition \ref{def:nonovershootconsensus} can be extended into the agent state's $k_{th}$, $k\!\!=\!\!\overline{1,n}$ component. However, in most practical scenarios, if the controlled object is modeled as a double integrator or high-order integrator, its first state component represents the position variable, which more likely has to be subject to some physical constraints. For example, to reach a leader moving on the ground, the position variable of all followers must be constrained by its terminal value (the motion of the leader), while the other variables, such as velocities and torques, do not have to be subject to such a constraint. Furthermore, if Definition \ref{def:nonovershootconsensus} applies to any component of the state of agent $i$, it is named as the system non-overshoot \cite{hollo1985modelling}, which is not in our scope at present. 

% % In the existing literature, few results focus on non-overshooting consensus. Despite we notice the linear output regulation scheme proposed by \cite{8378231} could address this issue, we would like to give a linear back-stepping-based non-overshooting consensus protocol. Before proceeding, some necessary definitions and lemmas are included as follows.

% For a continuous-time LTI system,
%      \begin{equation}\label{eq:pos_LTI}\begin{aligned}
%           \dot x(t)\!\!=\!\!Ax(t),\;\;x\!\!\in\!\!\R^n, \; t\!\!>\!\!0,\;A\!\!=\!\!\{a_{ij}\}\!\!\in\!\!\R^{n\!\times\!n},
%     \end{aligned}
%     \end{equation}
%     we have the following definition.
% \begin{Def}\cite{farina2011positive}
%     \textit{System \eqref{eq:pos_LTI} is said to be positive if $x(t)\!\!\geq\!\!0$, $\forall t\!\!>\!\!0$,  $\forall x(0)\!\!\geq\!\!0$.}
% \end{Def}

% \begin{Def}\cite{farina2011positive}
%     \textit{The system matrix $A$ is Metzler if and only if its off-diagonal entries are all non-negative, \textit{i.e.,} $a_{ij}\!\!\geq\!\!0$, $\forall i\!\!\neq\!\!j$.}
% \end{Def}

% \begin{lem}\cite{farina2011positive}
% \textit{System \eqref{eq:pos_LTI} is positive if and only if the system matrix $A$ is Metzler.}
% \end{lem}




% \begin{remark}
%     Compared to the actively researched consensus control protocol $u_i\!\!=\!\!\sum_{j=0}^N K(x_j\!\!-\!\!x_i)$, the control protocol \eqref{eq:lin_control} requires the neighbors' control inputs $u_j$. This design does not affect the distributed nature of this control protocol and has attracted some academic attention, .
% \end{remark}










%\section{Upgrading the linear control to a homogeneous one}




% \subsection{Canonical Homogeneous Norm}
% \begin{myDef}
% 	The functional $\|x\|_{\mathbf{d}}:~\mathbb{R}^n\mapsto \R_{\geq0}$ defined as $\|\mathbf{0}\|_{\dn}\!=\!0$,
% 	\begin{equation*}
% 		\|x\|_\mathbf{d}\!=\!{\rm exp}(s_x),\mathrm{where}\;s_x\in \mathbb{R}:\|\mathbf{d}(-s_x)x\|\!=\!1, x\in \mathbb{R}^n\setminus\{\mathbf{0}\}
% 	\end{equation*}
% 	is called the canonical homogeneous norm in $\mathbb{R}^n$, where $\mathbf{d}$ is a \textit{linear monotone dilation}.
% \end{myDef}

% The canonical homogeneous norm has the following properties \cite{Polyakov2020:Book}:
% \begin{itemize}
% 	\item  $\|\mathbf{d}(s)x\|_\mathbf{d}={\rm exp}(s)\|x\|_\mathbf{d}$,
% 	for $x\in \mathbb{R}^n$ and $s\in \mathbb{R}$;
% 	\item $ \|x\|_\mathbf{d}=\|-x\|_\mathbf{d}$, $\|x\|=1 \Leftrightarrow \|x\|_{\dn}=1$;
% 	\item $\|x \|_{\dn}$ is locally Lipschitz continuous on $\R^n\backslash\{\mathbf{0}\}$;
% 	\item if $\|\cdot\|\in C^{1}(\R^n\backslash\{\mathbf{0}\},\R_+)$, then $\|\cdot\|_{\dn}\in C^{1}(\R^n\backslash\{\mathbf{0}\},\R_+)$;
% 	\item if  $\|x\|=\|x\|_P$, where   $P$ satisfies
% 	\begin{equation*}
% 		P\succ 0,\;\; PG_{\dn}+G_{\dn}^{\top}P\succ0,
% 	\end{equation*}
% 	then the linear dilation $\dn(s)\!=\!\exp(sG_{\dn})$ is monotone and
% 	\begin{equation*}
% 		\tfrac{\partial \|x\|_{\dn}}{\partial x}\!=\!\tfrac{\|x\|_{\dn}x^{\top}\!\dn^{\top}\!(-\ln \|x\|_{\dn}) P\dn(-\ln \|x\|_{\dn})}{x^{\top}\!\dn^{\top}\!(-\ln \|x\|_{\dn})PG_{\dn}\dn(-\ln \|x\|_{\dn})x}, \; x\!\in\!\R^n\backslash\{\mathbf{0}\}.
% 	\end{equation*}
% \end{itemize}
% \subsection{Homogeneous System}
% \begin{myDef}
% 	A vector field $f: \mathbb{R}^n \mapsto \mathbb{R}^n$  (resp. a function $h:\R^n\mapsto \R$) is said to be $\dn$-homogeneous if there exists a $\mu \in \mathbb{R}$ such that
% 	\begin{equation*}\begin{aligned}
% 		&f(\dn(s) x)={\rm exp}(\mu s) \dn(s) f(x),\;\; s\in \mathbb{R},\; x \in \mathbb{R}^n\\
% 	(&\text{resp.  } h(\dn(s) x)={\rm exp}(\mu s) h(x),\;\; s\in \mathbb{R},\; x \in \mathbb{R}^n),
% \end{aligned}\end{equation*}
% where $\dn$ is a dilation and the scalar $\mu$ is known as the homogeneous degree of $f$ (resp. of $h$).
% \end{myDef}

% The following result is an adaption of  \cite{Hong2001:Aut}, \cite{Andrieu_etal2008:SIAM_JCO} to the case of linear dilation and can be found in \cite{Polyakov2020:Book}.
% \begin{lem}\label{lemadd1}
% Assume a continuous vector field $\tilde{f}:\mathbb{R}^{n+\omega}\mapsto \mathbb{R}^{n+\omega}$ takes the form of
% \begin{equation*}
%   \tilde{f}(x,q)=\left(
%                    \begin{smallmatrix}
%                      f(x,q) \\
%                      \mathbf{0} \\
%                    \end{smallmatrix}
%                  \right),\;\; x\in \mathbb{R}^{n}, \; q\in \mathbb{R}^{\omega}
% \end{equation*}
% and $\dn$-homogeneous of a degree $\mu$ with respect to a dilation $\dn=\left(
%                                              \begin{smallmatrix}
%                                                \dn_x & \mathbf{0} \\
%                                                \mathbf{0} & \dn_q \\
%                                              \end{smallmatrix}
%                                            \right)
% $
% in $\mathbb{R}^{n+\omega}$. If the system
% %\begin{equation*}
% $  \dot x=f(x,\mathbf{0})$ %, x(t)\in \mathbb{R}^{n}
% %\end{equation*}
% is asymptotically stable at the origin, then the system
% %\begin{equation*}
% $
%   \dot x=f(x,q)%,\quad q\in L^{\infty}(\mathbb{R},\mathbb{R}^{m})
%   $
% %\end{equation*}
% is ISS.
% \end{lem}

% The latter lemma  shows that the robustness of a homogeneous perturbed system is equivalent to the asymptotic stability of the unperturbed system. This essentially simplifies the robustness analysis of homogeneous systems.
% %\begin{lem}\label{lemadd2}
% %Let function $\dot x=f(x,q(t))$ is $\dn$-homogeneous of a degree $\mu$ and $\dn$ is a strictly monotone dilation in $\mathbb{R}^{n}$, i.e. $\|\dn\|\leq \mathrm{e}^{\beta s}$, for $s\leq 0$.
% %If there exist $f_0>0$ such that
% %\begin{equation*}
% %  \sup_{z}\|f(z,0)-f(z,q(t))\|\leq f_0,
% %\end{equation*}
% %and
% %\begin{equation*}
% %  \exists \gamma>\frac{f_0}{\beta}: \sup_{z}\langle f(z,\mathbf{0})+\gamma G_{\dn}z,z\rangle\leq0,
% %\end{equation*}
% %then for any $q\in L^{\infty}(\mathbb{R},\mathbb{R}):\|q\|_{\infty}\in [0,f_0]$ the origin of the system
% %\end{lem}






==> Revised_paper_0119/data/IV_Supervisor-based_Homogeneous_Control_Protocol.tex <==

















% The conventional linear consensus protocol can only guarantee asymptotic consensus (see, e.g., \cite{4118472,ren2005consensus,yu2010some}). This means consensus can be achieved as time goes to infinity. Such a long-term transient process may influence the control performance. However, the design of the consensus
% protocol with fast convergence rates may involve challenges and complexities.
% Recall (see Section \ref{Intro} and \ref{Pre}) that homogeneous systems can be finite-time stable or even fixed-time stable. This motivates us to find the approach to get some novel consensus protocol that can ensure  the closed-loop consensus error equation \eqref{eq:error_dynamics} to be  homogeneous of a desired degree.  Then, the fast convergence  could be performed by the MAS.


% To demonstrate our basic idea, let us consider first the design of  the  well-known linear consensus control protocol \cite{1333204}.
% %let us suggest a possible design of a linear consensus protocol.
% \begin{lem}\label{lem:lin_cont}
% 	Let Assumption \ref{assum1}, \ref{assum:bound} hold. Let $(X,Y)\in \R^{n\times n} \times \R^{m\times n}$ be a solution of the linear matrix inequality
% 	\begin{equation}\label{eq:LMI_lin}
% 	 X\!\succ\! 0,\;\; I_{N}\otimes (AX\!+\!X A^{\top}\!)\!+\! \tilde{\mathcal{L}}\!\otimes\! BY\!+\!(\tilde{\mathcal{L}}\!\otimes\! BY)^{\top}\prec 0,
% 	\end{equation}
% where
% \begin{equation}\begin{aligned}
%   \tilde{\mathcal{L}}=\left(
%                         \begin{matrix}
%                           -l_{11} & \dots & -l_{1N} \\
%                           \vdots & \ddots & \vdots \\
%                           -l_{N1} & \ldots & -l_{NN} \\
%                         \end{matrix}
%                       \right).
% \end{aligned}
% \label{eq:Ltiled}
% \end{equation}
% Let the linear consensus protocol be
% \begin{equation}\begin{aligned}\label{eq:linear_cp}
% 		u_i=K\sum\nolimits^N_{j=0}w_{ij}(\xi_j-\xi_i),\;\; i=\overline{1,N}
% \end{aligned}\end{equation}
% with $K=YX^{-1}$. Then the error equation
% \eqref{eq:error_dynamics} is ISS with respect to $q=(\xi_0,\dot
% \xi_0)$.
% \end{lem}

% Although the proof of the above lemma is straightforward,
% we still give the detailed proof in Appendix A since we will reuse it later for the homogeneous design.

% Let us recall the basic idea of upgrading a linear control to a homogeneous one.
% The  simplest scalar control system  $$\dot x=u,\;\; x\in \mathbb{R},\;u\in \mathbb{R}$$ with the linear control $$u=-kx, \;\; k\in \mathbb{R}_+$$ is globally asymptotically stable.
%  If the control $u$ is transformed to the homogeneous controller
%   $$u=-k |x|^{1+\mu}\mathrm{sign}(x),$$
%    then for $\mu\!=\!0$ we will have the original linear controller, for  $\mu\!<\!0$ the closed-loop system is finite-time stable, and for $\mu\! >\!0$ is nearly fixed-time stable. Similarly, for a multi-input system $$\dot x=Ax+Bu,\;\; x\in \mathbb{R}^n,\;u\in \mathbb{R}^m,\;A\in\mathbb{R}^{n\times n},\;B\in\mathbb{R}^{n\times m}$$ it can be shown \cite{Wang_etal2020:RNC} that
%    the linear stabilization controller
% \begin{equation*}
% u=Kx,\;\; K\in \mathbb{R}^{m\times n}
% \end{equation*}
% can be transformed (``upgraded") to the homogeneous form
% \begin{equation}\label{eq:homo_single}
% u=K_0 x+\|x\|^{\mu+1}_{\dn}(K-K_0)\dn(-\ln\|x\|_{\dn})x, \;\; K_0\in \R^{m\times n}
% \end{equation}
% such that the closed-loop multi-input system is finite-time stable for $\mu<0$ and nearly fixed-time stable  for $\mu>0$, where $\dn$ is a linear dilation in $\R^n$ and $\|\cdot\|_{\dn}$ is the canonical homogeneous norm.  In this paper  we generalize this upgrading approach to the consensus control of MAS. %The key difficulty of the design is the existence of a certain topology of the decentralized \textbf{MAS}, which does not allow the scheme developed for the centralized MIMO system to be implemented directly.




%\textcolor{blue}{In our case, we propose to expand this ``upgrading'' idea to the consensus control of MAS,i.e., upgrading the linear control \eqref{eq:linear_cp} to a $\dn$-homogeneous (quasi-decentralized) consensus protocol. Below, specific protocol design and theoretical analysis are carried out. }
%a homogeneous one $\|x\|^{\mu+1}_{\dn}K\dn(-\ln\|x\|_{\dn})x$, where $\dn$ is a properly defined linear monotone dilation and $\|\cdot\|_{\dn}$ is the canonical homogeneous norm}. Below we follow this idea to ``upgrade'' the classical linear consensus protocol \eqref{eq:linear_cp} of degree $0$ to a protocol of degree $\mu\neq 0$.}


%The linear control protocol \eqref{eq:linear_cp} (the error equation \eqref{eq:lin_compacterror}) is homogeneous of the zero degree.
%It guarantees consensus errors converge to a zone, rather than zeros. Moreover, for the case of the non-zero degree, not only ISS, but also the global finite-time convergence can be guaranteed.
%\textit{An algorithm for upgrading of a linear control to a generalized homogeneous one is developed in \cite{Wang_etal2021:RNC}.
%It suggests to replace the linear feedback $Ke$ with the homogeneous one $\|e\|_{\dn}^{1+\mu}  K \dn(-\ln \|e\|_{\dn}) e$,
%where $\dn$ is a properly defined linear monotone dilation and $\|\cdot\|_{\dn}$ is the canonical homogeneous norm.}
%Below we follow this idea in order to design a $\dn$-homogeneous (quasi-decentralized) control protocol of degree $\mu\neq 0$.




==> Revised_paper_0119/data/I_Introduction.tex <==
\section{Introduction}\label{Intro}

Consensus in Multi-Agent Systems (MAS) has been an important research topic over the past two decades. This study seeks some control protocol to ensure all agents' states reach an agreement. In particular, the leader-following consensus, where the agreement is the leader's state, has received substantial focus \cite{ni2010leader,guan2012finite,li2023generalized}. Despite considerable research progress, there has been limited research addressing leader-following consensus in the context of both time constraints, which affect the convergence rate, and space constraints, which impact the safety of agent movements.

The primary technique involved in the control problem considering time constraints is the finite-time stability strategy, which ensures the system state reaches equilibrium at a time dependent on the initial system state. This method, known since the 1960s \cite{fuller1960relay,korobov1979solution,haimo1986finite,bhat2000finite}, has seen considerable development and application in recent years, particularly in addressing the consensus problem for the MAS \cite{wang2008finite,guan2012finite,li2023generalized}. 
%The fixed-time stability technique, an extension of finite-time stability, assumes a global bound on convergence time and has also been integrated into consensus control protocols design \cite{zuo2017fixed,ning2019practical,du2020distributed}. Furthermore, a recent development in the non-asymptotic control strategy, known as the prescribed-time stability technique, allows an arbitrary setting of the convergence time and offers a new possibility to integrate into the consensus control \cite{ning2018prescribed,ding2023prescribed}.

On the other hand, numerous results have focused on the consensus under space constraints. Specifically, constrained consensus, first introduced in \cite{5404774} and actively studied by \cite{lin2013constrained,liu2017constrained,qiu2016distributed}, aiming at a consensus limiting each agent to a closed convex set. Additionally, research on positive systems \cite{de2001stabilization, rami2007controller, farina2011positive} contributes to the consensus study, leading to the positive consensus, which means a consensus with agent states being positive \cite{6681911,7892854,8862888,su2017positive,su2018positive}. 
% The pioneering result on positive consensus is obtained by \cite{6681911}, which proposes a centralized control protocol, followed by a distributed control design approach \cite{7892854}, and has been further developed by \cite{8862888, su2017positive,su2018positive}. 
Moreover, the study of non-overshooting stabilization \cite{phillips1988conditions,krstic2006nonovershooting,schmid2010unified}, which ensures that a partial system state is uniformly bounded by its terminal value, has been integrated into the consensus research by \cite{8378231}. 
Nevertheless, few works focus on consensus considering both time and space constraints. This topic is vital as it contributes to the MAS's working efficiency and safety. 

This paper aims to address the consensus problem under both time and space constraints. Specifically, we tackle the finite-time non-overshooting leader-following consensus problem for MAS with high-order integrator dynamics. The MAS operates under a directed graph that allows local transmission of both the agents' states and a supporting vector using only local information, similar to the configurations in \cite{ning2020bipartite, hong2006tracking, ren2007multi, liu2011synchronization}. Regarding this MAS, we propose a consensus control protocol that guarantees finite-time convergence, improving upon \cite{li2023generalized} by a distributed design. The main technique for achieving finite-time convergence is homogeneity-based control.

Homogeneity is a property characterizing a wide class of systems, including all linear systems and a large subset of nonlinear systems. An asymptotically stable homogeneous system can exhibit finite-time convergence with a negative homogeneity degree. This motivates the ``upgrading" from linear control to homogeneous control \cite{wang2021generalized, polyakov2020generalized}, which is one of the most effective ways to obtain a homogeneous control.

Based on the above establishment, we propose a linear protocol that ensures asymptotic non-overshooting consensus, where the followers' first state component does not exceed the one of the leader. This non-overshooting behavior is ensured by the strict positive invariance of the consensus error within a linear cone. Building on this, the linear protocol is upgraded to a homogeneous one, resulting in a finite-time non-overshooting consensus protocol. This ensures consensus error achieves finite-time stability and strict positive invariance within a homogeneous cone. Additionally, a class of disturbances affecting agent dynamics is characterized, under which the homogeneous protocol can maintain the non-overshooting property. Finally, simulations confirm the control effectiveness.






% Homogeneity is an important property of systems that describes a kind of nonlinearity and covers all linear systems as well as a large class of nonlinear systems. An asymptotically stable homogeneous system can exhibit finite-time convergence with a negative homogeneity degree. Upgrading the classical linear control to a homogeneous one is a practical approach to obtaining homogeneous controls \cite{wang2021generalized,polyakov2020generalized}. In the context of consensus control for MAS, \cite{li2023generalized} proposes a quasi-decentralized homogeneous control protocol relying on a global-broadcasting signal, which may hinder its contribution.

% This paper aims to resolve the consensus problem considering both time and space constraints. To this end, we address the finite-time non-overshooting leader-following consensus problem for a MAS of high-order integrator dynamics. 
% This MAS operates under a directed graph that facilitates the local transmission of both the agent's state and a supporting vector based on local information, similar to the configurations in \cite{ning2020bipartite, hong2006tracking,ren2007multi,liu2011synchronization}. 
% Specifically, we introduce a homogeneous consensus control protocol that guarantees finite-time consensus. This protocol improves upon \cite{li2023generalized}, featuring a fully distributed control. 
% Then, we propose a linear protocol that ensures non-overshooting asymptotic consensus, meaning the followers' first state does not exceed the leader's first state. This is technically ensured by the strict positive invariance of the consensus error within a linear cone. 
% This linear protocol allows an upgrade to a homogeneous design, resulting in a finite-time non-overshooting consensus protocol. This ensures that the consensus error achieves finite-time stability and strict positive invariance within a homogeneous cone. 
% Additionally, we characterize a class of agent model disturbances for which the homogeneous protocol preserves the non-overshooting property and is robust in the ISS sense. Finally, simulations confirm the effectiveness of the results. 




% We assume the MAS operates with high-order integrator dynamics and is governed by a directed graph that facilitates the local transmission of both the agent's state and a supporting vector based on local information, similar to the configurations in \cite{ning2020bipartite, hong2006tracking,ren2007multi,liu2011synchronization}. 
% To address the time constraint, we propose a homogeneous consensus control protocol that guarantees finite-time consensus. This protocol improves upon \cite{li2023generalized}, featuring a fully distributed design.
% To address the space constraint, we propose a linear protocol that ensures non-overshooting asymptotic consensus, meaning the followers' first state does not exceed the leader's first state. This is technically ensured by the asymptotic stability and strict positive invariance of the consensus error within a linear cone.
% The linear protocol can be upgraded to a homogeneous design, resulting in a finite-time non-overshooting consensus protocol. This ensures the MAS achieves finite-time consensus with the strict positive invariance of the consensus error within a homogeneous cone. 
% Additionally, we characterize a class of additive disturbances for which the homogeneous protocol preserves the non-overshooting property and remains robust in the ISS sense. Finally, simulations confirm the effectiveness of the results. 

The remainder of this paper is structured as follows. Section \ref{PF} describes the problem to be studied. Section \ref{Pre} provides some useful knowledge and results.  Section \ref{MR2} outlines the design of the linear non-overshooting consensus protocol and its upgrade to a homogeneous one. Section \ref{SR} presents simulations. Finally, Section \ref{Con} concludes this work.

\textit{Notations}:
$\R$ is the set of real numbers; 
$\R_+$ ({\it{resp.,}} $\R_{-}$) is the set of positive ({\it{resp.,}} negative) real numbers; 
$\R_{\geq0}\!\!=\!\!\R_+\!\!\cup\!\{0\}$;
$\mathbb{N}_+$ is the set of positive integers;
a series of positive integers $1,\dots,N$ is denoted as $\overline{1,N}$; 
let $n\!\!\in\!\!\mathbb{N}_+$, $\R^n$ and $\R^{n\times n}$ denote the  $n\!\!\times\!\! 1$ real vector and the $n\!\!\times\!\! n$ real matrix, respectively; 
$\R^n_{+}$ ({\it{resp.,}} $\R^n_{-}$) denotes the $n\!\!\times\!\! 1$ real vector whose elements are positive ({\it{resp.,}} negative);
$I_n$ is the $n\!\!\times\!\!n$ identity matrix;  
$\diag\{\sigma_i\}_{i=1}^n$ is the (block) diagonal matrix with the diagonal entry $\sigma_i$ of proper dimension; 
$\{\sigma_{ij}\}$ is the $n_1\!\!\times\!\!n_2$ (block) matrix of a proper dimension with element $\sigma_{ij}$, $i\!\!=\!\!\overline{1,n_1}$, $j\!\!=\!\!\overline{1,n_2}$, $n_1,n_2\!\!\in\!\!\mathbb{N}_+$; 
$\mathbf{1}_{n}\!\!\in\!\!\R^n$ ({\it{resp.,}} $\mathbf{0}_{n}\!\!\in\!\!\R^n$) with elements are all ones ({\it{resp.,}} zeros);  
let $P\!\!=\!\!\{P_{ij}\}\!\!\in\!\!\R^{n_1\!\times\!n_2}$, $P_{ij}\!\!\in\!\!\R$, $P\!\!\geq\!\!0 ({\it{resp.,}} \leq\!\!0)$ means $P_{ij}\!\!\geq\!\!0({\it{resp.,}} \leq\!\!0)$, $\forall i\!\!=\!\!\overline{1,n_1}$, $\forall j\!\!=\!\!\overline{1,n_2}$;
let $P\!\!\in\!\! \R^{n\times n}$, $P\!\!\succ\!\! 0( {\it{resp.,}}\!\!\prec\!\! 0)$ means that $P$ is symmetric and positive ({\it{resp.,}} negative) definite; $P$ is anti-Hurwitz if $-P$ is Hurwitz; 
$\exp(P)\!\!=\!\!\sum_{i=0}^\infty\!\!\tfrac{P^i}{i!}$;
$\lambda_{\max}(P)$ ($resp.,$ $\lambda_{\min}(P)$) represents the maximum ($resp.,$ minimum) eigenvalue of $P$;
$\otimes $ represents the Kronecker product; 
$\textbf{B}(R)$ is a ball centered at the origin of radius $R\!\!\in\!\!\R_+$;
$\eta_i\!\!\in\!\!\R^n$ ({\it resp.,} $\xi_i\!\!\in\!\!\R^N$) is the $i_{th}$ element of the canonical Euclidean basis in $\R^n$ ({\it resp.,} $\R^N$);
let $x\!\!=\!\!(x_1,\dots,x_n)^\top\!\!\!\!\in\!\!\R^n$, $\|x\|$ is a norm in $\R^n$; $\|x\|_{P}\!\!=\!\!\sqrt{x^{\top}\!\!Px}$,  $P\!\!\in\!\! \R^{n\times n}$ satisfies $P\!\!\succ\!\!0$; 
$\|x\|_{\infty}\!\!=\!\!\max_{i=\overline{1,n}}|x_i|$;
% $\mathcal{C}(X,Y)$ denotes the class of continuous functions$:\!X\!\!\to\!\!Y$ with $X$ and $Y$ are the subsets of normed vector spaces;
% $\mathcal{C}^p(X,Y)$ denotes the class of functions$\!:\!X\!\!\to\!\!Y$ which are differentiable at least up to order $p\!\!\in\!\!\mathbb{N}_+$;
the function $\alpha\!:\!\R_{\geq0}\!\!\to\!\!\R_{\geq0}$ is said to be of \textit{class $\mathscr{K}$} if  it is continuously strictly increasing with $\alpha(0)\!\!=\!\!0$; the function $\beta\!:\!\R_{\geq0}\!\!\times\!\!\R_{\geq0}\!\!\to\!\!\R_{\geq0}$ is said to be of \textit{class $\mathscr{KL}$} if for each fixed $t$ the function $s\!\!\mapsto\!\! \beta(s,t)$ is of class $\mathscr{K}$ and for each fixed $s$ the function $t\!\!\mapsto\!\! \beta(s,t)$ is continuously strictly decreasing; $L^\infty(\R,\R^n)$ is the space of Lebesgue measurable essentially bounded functions $q\!:\!\R\!\!\to\!\!\R^n$ with a norm 
$\|q\|_{L^\infty}\!\!:=\!\!\mathrm{ess} \sup_{t\in\R_+}\!\!\|q(t)\|_\infty\!\!<\!\!+\infty$. 
%a normal (Gaussian) distribution is denoted by $\mathcal{N}(\mu_{\mathcal{N}},\sigma_\mathcal{N}^2)$ with the mean value $\mu_{\mathcal{N}}\!\!\in\!\!\R$ and variance $\sigma_\mathcal{N}^2$, $\sigma_\mathcal{N}\!\!\in\!\!\R_+$.

==> Revised_paper_0119/data/V_MR.tex <==
%\newpage
\subsection{Distributed Homogeneous Consensus}\label{MR1}

In contrast to the quasi-decentralized homogeneous leader-following consensus control relying on a centralized design of $v_i$, $i\!\!=\!\!\overline{0,N}$ in \cite{li2023generalized}, we propose a distributed scheme.

\begin{thm}\label{thm:state_con}
\it{Let $\mu\!\!\in\!\![-1,\tfrac{1}{n-1})$. Let $(X,Y)\!\!\in\!\!\R^{n\!\times\!n}\!\!\times\!\!\R^{1\!\times\!n}$ be the solution of the following LMI:
\begin{equation}\label{eq:LMI_P_U}
 X\!\!\succ\!\!0,\quad G_\dn X\!\!+\!\!XG_\dn\!\!\succ\!\!0, \quad AX\!\!+\!\!X A^\top\!\!\!\!-\!\!BY\!\!-\!\!Y^\top\!\! B^\top\!\!\!\!\prec\!\!0,
\end{equation}
where $G_\dn\!\!=\!\!\diag\{1\!\!-\!\!\mu(n\!\!-\!\!k)\}_{k\!=\!1}^n$. Let $\dn$ be a dilation group generated by $G_\dn$. 
Let the transmitted vector 
\begin{equation}\label{eq:def_vi}\begin{aligned}
v_0\!\!=\!\!\textbf{0}_n,\quad v_i\!\!=\!\!\tfrac{1}{\sum_{j=0}^Nw_{ij}}\sum\nolimits_{j=0}^N w_{ij}\left(x_i\!\!-\!\!x_j\!\!+\!\!v_j\right), \;\; i\!\!=\!\!\overline{1,N}
 \end{aligned}\end{equation}
 and the distributed homogeneous consensus protocol
% \begin{equation*}
%  	u_i\!\!=\!\!\tfrac{1}{\sum_{j=0}^N\!w_{ij}}\!\!\sum\nolimits_{j=0}^N \!\!w_{ij}\!\!\left(\|v_i\|_{\dn}^{1+\mu}K\dn(-\ln\|v_i\|_{\dn})(x_j\!\!-\!\!x_i)\!\!+\!\!u_j\right)\!,i\!\!=\!\!\overline{1,N}
%  \end{equation*}
 \begin{equation}\label{eq:homo_control}
 	u_i\!\!=\!\!-\|v_i\|_{\dn}^{1+\mu}K\dn(-\ln\|v_i\|_{\dn})v_i,\;\; i\!\!=\!\!\overline{1,N}
 \end{equation}
with $K\!\!=\!\!YX^{-1}$, $\|\cdot\|_\dn$ is induced by the weighted Euclidean norm $\|\cdot\|_P$, $P\!\!=\!\!X^{-1}$,
% \begin{equation}\label{eq:def_vi}\begin{aligned}
% v_i\!\!=\!\!\tfrac{1}{\sum_{j=0}^Nw_{ij}}\sum\nolimits_{j=0}^N w_{ij}\left(x_i\!\!-\!\!x_j\!\!+\!\!v_j\right), \; \;i\!\!=\!\!\overline{1,N}.
%  \end{aligned}\end{equation}
such that 
\\
$\bullet$ equation \eqref{eq:def_vi}, \eqref{eq:homo_control} and \eqref{eq:nonovershooterrordy} have unique solution $v_i$, $u_i$ and $e_i$, $i\!\!=\!\!\overline{1,N}$, respectively;
\\
$\bullet$ closed-loop error equation \eqref{eq:nonovershooterrordy} is globally finite-time stable for $\mu\!\!\in\!\![-1,0)$.

% b) globally exponentially stable for $\mu\!\!=\!\!0$, 

% c) globally practical fixed-time stable for $\mu\!\!\in\!\!(0,\tfrac{1}{n-1})$.
}

\end{thm}

\begin{proof}
Recall Lemma \ref{lem:unique} with $\omega_i\!\!=\!\!v_i$, $ i\!\!=\!\!\overline{0,N}$, $M\!\!=\!\!I_n$, the equation \eqref{eq:def_vi} has a unique solution $v\!\!=\!\!e$, $v\!\!=\!\!(v_1^\top,\dots,v_N^\top)^\top$.
%&=\!\!-(I_N\!\otimes\!K)\diag\{\|(\xi_i^\top\!\!\!\otimes\!\! I_n) e\|_{\dn}^{1+\mu}\!\!\dn(-\ln\|(\xi_i^\top\!\!\!\otimes\!\! I_n) e\|_{\dn})\}_{i=1}^Ne,
In this case, the closed-loop error equation \eqref{eq:nonovershooterrordy} 
yielding
\begin{equation}\label{eq:exp_error_dy}\begin{aligned}
\dot e\!\!=&f(e)\\
  % \!\!=&\!\!\left(I_N\!\otimes\!A\!\!-\!\!(I_N\!\otimes\!BK)\diag\{\|v_i\|_{\dn}^{1+\mu}\!\!\dn(-\ln\|v_i\|_{\dn})\}_{i=1}^N\right)e\\
  % \!\!=&\!\!\left(I_N\!\otimes\!A\!\!-\!\!(I_N\!\otimes\!BK)\diag\{\|e_i\|_{\dn}^{1+\mu}\!\!\dn(-\ln\|e_i\|_{\dn})\}_{i=1}^N\right)e\\
    \!\!=&\!\left(I_N\!\!\otimes\!\!A\!\!-\!\!\diag\{\|(\xi_i^\top\!\!\!\otimes\!\!I_n)e\|_{\dn}^{1+\mu}\!BK\dn(-\!\!\ln\!\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn})\}_{i=1}^N\right)e,
\end{aligned} \end{equation}
% \begin{equation*}
% \begin{cases}
%  	\dot e\!\! =\!\! (I_N\!\! \otimes \!\!A)e \!\!-\!\! (I_N\!\!\otimes \!\!B)u,\\
%   u \!\!=\!\! -\diag\{\|v_i\|_{\dn}^{1+\mu}K\dn(-\ln\|v_i\|_{\dn})\}_{i=1}^Nv,\\
%   v \!\!=\!\! e, 
% \end{cases}
% \end{equation*}
has a unique solution.
We notice equation \eqref{eq:exp_error_dy} is completely decoupled component-wise, \textit{i.e.,} the dynamics of $e_i$ can be written as $\dot e_i\!\!=\!\!f_{i}(e_i)\!\!=\!\!
  (A\!\!-\!\!\|e_i\|_{\dn}^{1+\mu}\!\!BK\dn(-\ln\|e_i\|_{\dn}))e_i$,  $f_{i}\!\!:\!\!\R^n\!\!\to\!\!\R^n$, $i\!\!=\!\!\overline{1,N}$.
In this case, the stability of $e_i\!\!\in\!\!\R^n$, $i\!\!=\!\!\overline{1,N}$ is exhibited by $e\!\!\in\!\!\R^{Nn}$. 

We first concentrate on the homogeneity.
Equation \eqref{eq:G_d} implies $(I_N\!\otimes\!A)\tilde\dn(s)\!\!=\!\!\exp(\mu s)\tilde\dn(s)(I_N\!\otimes\!A)$ and $\exp(s)(I_N\!\otimes\!B)\!\!=\!\!\tilde\dn( s)(I_N\!\otimes\!B)$ \cite{polyakov2020generalized}, where $\tdn\!\!=\!\!I_N\!\!\otimes\!\!\dn$.
The vector field $e\!\!\mapsto\!\!f(e)$ is $\tilde\dn$-homogeneous of degree $\mu\!\!\in\!\!\R$ with respect to $e\!\!\to\!\!\tilde\dn(s)e$ since
$f(\tilde\dn(s)e)\!\!=\!\!\exp(\mu s)\tilde\dn(s)f(e)$, $\forall s\!\!\in\!\!\R$.
Similarly, 
% using the formula $A\dn(s)\!\!=\!\!\exp(\mu s)\dn(s)A$ and $\exp(s)B\!\!=\!\!\dn( s)B$, 
 $e_i\!\!\mapsto\!\!f_{i}(e_i)$ be $\dn$-homogeneous of degree $\mu\!\!\in\!\!\R$ with respect to $e_i\!\!\to\!\!\dn(s)e_i$ since $f_i(\dn(s)e)\!\!=\!\!\exp(\mu s)\dn(s)f_i(e)$, $\forall s\!\!\in\!\!\R$. 





% . To show this, we have the following calculation:
% \begin{equation*}\begin{aligned}
% &f_a(\tilde\dn(s)e)\!\!=\!\!\left(I_N\!\!\otimes\!\!A\right)\tilde\dn(s)e\!\!-\!\!(I_N\!\!\otimes\!\!BK)\\
% &\!\!\times\!\!\diag\{\|(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\tilde\dn(s)e\|_{\dn}^{1+\mu}\!\!\dn(-\ln\|(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\tilde\dn(s)e\|_{\dn})\}_{i=1}^N\tilde\dn(s)e\\
% &\!\!=\!\!\exp(\mu s)\tilde\dn(s)\left(I_N\!\!\otimes\!\!A\right)e\!\!-\!\!(I_N\!\!\otimes\!\!BK)\\
% &\!\!\times\!\!\diag\{\|\dn(s)(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn}^{1+\mu}\!\!\dn(-\ln\|\dn(s)(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn})\}_{i=1}^N\tilde\dn(s)e\\
% &\!\!=\!\!\exp(\mu s)\tilde\dn(s)\left(I_N\!\!\otimes\!\!A\right)e\!\!-\!\exp(s(1\!\!+\!\!\mu))(I_N\!\!\otimes\!\!BK)\\&\!\!\times\!\!\diag\{\|(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn}^{1+\mu}\!\!\dn(-\ln\|(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn})\}_{i=1}^N\tilde\dn(-s)\tilde\dn(s)e\\
% &\!\!=\!\!\exp(\mu s)\tilde\dn(s)\left(I_N\!\!\otimes\!\!A\right)e\!\!-\!\exp(\mu s)(I_N\!\!\otimes\!\exp(s)BK)\\&\!\!\times\!\!\diag\{\|(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn}^{1+\mu}\!\!\dn(-\ln\|(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn})\}_{i=1}^Ne\\
% &\!\!=\!\!\exp(\mu s)\tilde\dn(s)\left(I_N\!\!\otimes\!\!A\right)e\!\!-\!\exp(\mu s)\tilde\dn(s)(I_N\!\!\otimes\!\!BK)\\&\!\!\times\!\!\diag\{\|(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn}^{1+\mu}\!\!\dn(-\ln\|(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn})\}_{i=1}^Ne\\
% &\!\!=\!\!\exp(\mu s)\tilde\dn(s)f_a(e).
%   \end{aligned}\end{equation*}



Then, we prove $\|e_i\|_\dn$ be the Lyapunov candidate for  $\dot e_i\!\!=\!\!f_{i}(e_i)$. Indeed,
\begin{equation*}\begin{aligned}
&\tfrac{d \|e_i\|_{\dn}}{d t}
%\\
% &=\!\!\tfrac{\|e_i\|_{\dn}e_i^{\top}\dn^{\top}\!\!\!(-\ln \|e_i\|_\dn)P\dn(-\ln \|e_i\|_\dn)\dot e_i}
% {e_i^{\top}\dn^{\top}\!\!\!(-\ln \|e_i\|_\dn)PG_{\dn}\dn(-\ln \|e_i\|_\dn)e_i}\\
% &=\!\!\tfrac{\|e_i\|_{\dn}e_i^{\top}\dn^{\top}\!\!\!(-\ln \|e_i\|_\dn)P\dn(-\ln \|e_i\|_\dn)(A\!-\!\|e_i\|_{\dn}^{1+\mu}BK\dn(-\ln\|e_i\|_{\dn}))e_i}
% {e_i^{\top}\dn^{\top}\!\!\!(-\ln \|e_i\|_\dn)PG_{\dn}\dn(-\ln \|e_i\|_\dn)e_i}\\
% &=\!\!\tfrac{\|e_i\|_\dn^{1+\mu}e_i^{\top}\dn^{\top}\!\!\!(-\ln \|e_i\|_\dn) P(A\!-\!BK)\dn(-\ln \|e_i\|_\dn)e_i}
% {e_i^{\top}\dn^{\top}\!\!\!(-\ln \|e_i\|_\dn)PG_{\dn}\dn(-\ln \|e_i\|_\dn)e_i}\\
\!\!=\!\!\tfrac{\|e_i\|_\dn^{1+\mu}e_i^{\top}\dn^{\top}\!\!\!(-\ln \|e_i\|_\dn) P(AX\!+\!XA^\top\!\!\!-\!BY\!-\!Y^\top\!\!\! B^\top)P\dn(-\ln \|e_i\|_\dn)e_i}
{e_i^{\top}\dn^{\top}\!\!\!(-\ln \|e_i\|_\dn)P(G_{\dn}X\!+\!XG_\dn )P\dn(-\ln \|e_i\|_\dn)e_i}.
	\end{aligned}\end{equation*}
We have $\tfrac{d \|e_i\|_{\dn}}{d t}\!\!<\!\!0$ since \eqref{eq:LMI_P_U} is satisfied. Since the latter analysis is valid for any $i\!\!=\!\!\overline{1,N}$, then we have the error equation $\dot e\!\!=\!\!f(e)$ being globally asymptotically stable. Finally,  the proof is completed by recalling Lemma \ref{lem1}. 
\end{proof}
For $\mu=-1$ the control \eqref{eq:homo_control} has a discontinuity at the point $v_i=\textbf{0}_{n}$. In this case, solutions of the closed-loop system are understood in the sense of  Filippov \cite{Filippov1988:Book}. 
Moreover, if some model uncertainty is introduced to the dynamics of agents \eqref{eq:dynamic} as below,
\begin{equation}\label{eq:dynamic_disturb}
\begin{aligned}
 \dot x_{i}(t)\!\!=\!\!Ax_i(t)\!\!+\!\!Bu_i(t)\!\!+\!\!q_{i}(t),\;\;  q_{i}\!\!\in\!\!L^\infty\!(\R,\R^{n}),\;\;i\!\!=\!\!\overline{0,N}.
\end{aligned}
\end{equation}
The error equation becomes
\begin{equation}\label{eq:exp_error_dy_disturb}\begin{aligned}
 	\dot e&\!\!=\!\!f(e,q)\\
  &\!\!=
    \!\!\!(I_N\!\!\otimes\!\!A)e
    \!\!-\!\!\diag\{\!\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn}^{1\!+\!\mu}\!BK\dn(\!-\!\!\ln\!\!\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn})\!\}_{i=1}^N\!e\!\!+\!\!q,
\end{aligned} \end{equation}
with $f\!:\!\R^{Nn}\!\!\times\!\!\R^{Nn}\!\!\to\!\!\R^{Nn}$, $q\!\!=\!\!((q_{1}\!\!-\!\!q_{0})^\top,\dots,(q_{N}\!\!-\!\!q_{0})^\top)^\top\!\!\!\!\!\in\!\!L^\infty\!(\R,\R^{Nn})$. 
\begin{Coro}\label{remark:ISS}
  {\it Let the conditions of Theorem \ref{thm:state_con} hold. Let $\mu\!\!\in\!\!(-1,0)$. The error equation \eqref{eq:exp_error_dy_disturb} is ISS with respect to $q\!\!\in\!\!L^\infty\!(\R,\R^{Nn})$.}
\end{Coro}
\begin{proof}
Recall Lemma \ref{lem:ISS}, let $f_q(e,q)\!\!=\!\!(f^\top\!\!(e,q),\textbf{0}^\top_{Nn})^\top$, $f_q\!\!:\!\!\R^{Nn}\!\!\times\!\!\R^{Nn}\!\!\to\!\!\R^{2Nn}$. It is validated that 
$f_q(\tdn(s)e,\exp(\mu s)\tdn(s)q)\!\!=\!\!\exp(\mu s)\diag\{\tdn(s),\exp(\mu s)\tdn(s)\}f_q(e,q)$, $\forall s\!\!\in\!\!\R$. Thus we have 
the vector field $f_q\!\!:\!\!\R^{Nn}\!\!\times\!\!\R^{Nn}\!\!\to\!\!\R^{2Nn}$ be  
homogeneous of degree $\mu$ with respect to dilation $(e,q)\mapsto (\tdn(s)e,\exp(\mu s)\tdn(s)q)$. The asymptotic stability of $\dot e\!\!=\!\!f(e,\textbf{0})$ is guaranteed by Theorem \ref{thm:state_con}.
Therefore, the claimed property is obtained.
\end{proof}



\section{Finite-time Non-overshooting Consensus Control Design}\label{MR2}

%In this section, we continue the design of $v_i\!\!\in\!\!\R^n$, based on which innovate a linear non-overshooting leader-following consensus protocol. Furthermore, by designing a scaling scheme for the linear control gain, we upgrade the linear control to a homogeneous one, reaching the finite-time non-overshooting leader-following consensus.
%In this section, we propose a scheme of non-overshooting consensus control design.


\subsection{Asymptotic Non-overshooting Consensus}
For a constant $\lambda\!\!\in\!\!\R_+$, let us introduce the row vectors
\begin{equation*}\begin{aligned}
    h_k\!\!=\!\!-\eta^\top_1\!\!(A\!\!+\!\!\lambda I_n)^{k-1},\;\; k\!\!=\!\!\overline{1,n}
\end{aligned}\end{equation*}
% where $\xi_1\!\!=\!\!(1, 0,\dots,0)^\top\!\!\!\!\in\!\!\R^n$ is the first element of the canonical Euclidean basis in $\R^n$,
and consider a positive cone 
\begin{equation}\label{eq:lin_positive_cone}\begin{aligned}
    \Omega\!=\!\{e\!\in\!\R^{Nn}\!:\! (I_N\!\otimes\! H)e\!\geq\!{0}\}\!\subset\!\Sigma, \;\; H\!=\!(h^\top_1,\dots,h^\top_n)^\top\!, 
\end{aligned}\end{equation}
where $\Sigma\!\!=\!\!\{e\!\!\in\!\!\R^{Nn}\!:\!(I_N\!\!\otimes\!\!\eta_1^\top)e\!\!\leq\!\!{0}\}$.

\begin{thm}\label{thm:linear}
\textit{ Let $\lambda\!\!\in\!\!\R_+$. Let the transmitted vector $v_i$ be given by \eqref{eq:def_vi}, and the consensus control protocol be defined as
\begin{equation}\label{eq:lin_control}
    u_i\!\!=\!\!-K_{lin} v_i,\;\;
K_{lin}\!\!=\!\!\eta_1^\top\!\!(A\!\!+\!\!\lambda I_n)^n,\;\;i\!\!=\!\!\overline{1,N}.
\end{equation}
The control \eqref{eq:lin_control} asymptotically stabilizes the error equation \eqref{eq:nonovershooterrordy}, and renders $\Omega$ strictly positively invariant for the equation \eqref{eq:nonovershooterrordy}. Moreover, if
\begin{equation}\label{eq:lambda}\begin{aligned}
    \sum\nolimits_{\zeta=0}^{k-1}\!\!C_\zeta^{k-1}\!\!\lambda^\zeta\eta^\top_{k-\zeta}e_i(0)\!\!\leq\!\!{0},\;\; \forall k\!\!=\!\!\overline{2,n},\;\;\forall i\!\!=\!\!\overline{1,N},
\end{aligned}\end{equation}
with $C_\zeta^{k-1}\!\!=\!\!\tfrac{(k-1)!}{(k-1-\zeta)!\zeta!}$ then $e(0)\!\!\in\!\!\Omega$.} 
\end{thm}
\begin{proof}
Equation \eqref{eq:def_vi} has unique solution $v\!\!=\!\!e$ by recalling Theorem \ref{thm:state_con}, then \eqref{eq:lin_control} is compactly written as $u\!\!=\!\!-(I_N\!\otimes\!K_{lin}) e$, $u\!\!=\!\!(u_1,\dots,u_N)^\top\!\!\!\in\!\!\R^N$, and the error equation \eqref{eq:nonovershooterrordy} becomes
 \begin{equation}\label{eq:error_closed}\begin{aligned}
 	\dot e\!\!=\!\!f(e)
  %(I_N\!\!\otimes\!\!A)e\!\!+\!\!(I_N\!\!\otimes\!\!B)u
  \!\!=\!\!(I_N\!\!\otimes\!\!(A\!\!-\!\!BK_{lin}))e,\;\;e\!\!=\!\!(e_1^\top\!\!,\dots,e_N^\top\!)^\top
  \end{aligned}\end{equation}
  which is decoupled component-wise satisfying $\dot e_i\!\!=\!\!f_i(e_i)\!\!=\!\!(A\!\!-\!\!BK_{lin})e_i$, $f_i\!\!:\!\!\R^n\!\!\to\!\!\R^n$, $e_i\!\!=\!\!(e_{i,1},\dots,e_{i,n})^\top\!\!\!\in\!\!\R^n$.
Let the barrier function $\phi_{i}\!\!=\!\!(\phi_{i,1},\dots,\phi_{i,n})^\top$, $\phi_{i,k}\!:\!\R^n\!\!\to\!\!\R$ be
\begin{equation}\label{eq:varphidef}\begin{aligned}
    \phi_{i,1}\!\!=\!\!-e_{i,1},\quad \phi_{i,k}\!\!=\!\!\dot\phi_{i,k-1}\!\!+\!\!\lambda\phi_{i,k-1},\;\;k\!\!=\!\!\overline{2,n}\\
\end{aligned}\end{equation}
namely,
    $\phi_{i,k}\!\!=\!\!h_{k-1}\dot e_i\!\!+\!\!\lambda h_{k-1}e_i\!\!=\!\!h_{k-1}A e_i\!\!-\!\!h_{k-1} BK_{lin} e_i\!\!+\!\!\lambda h_{k-1}e_i$.
    %\pi_k&\!\!=\!\!-(\xi^\top_1(A+\lambda I_n)^{k-1})\!\otimes\!I_{m_j}.
Since $h_{k-1}B\!\!=\!\!{0}$, then
$\phi_{i,k}\!\!=\!\!h_{k-1}(A\!\!+\!\!\lambda I_n)e_i
    \!\!=\!\!h_ke_i$.
Thus $\phi_i\!\!=\!\!He_i$, 
% $H\!\!=\!\!(
%        h_1^\top, \ldots,  h_n^\top
%     )^\top\!\!\!\!=\!\!(
%        -\xi_1, -(A^\top\!\!\!\!+\!\lambda I_n)\xi_1, \ldots,  -((A\!+\!\lambda I_n)^{n-1})^\top\!\!\xi_1
%     )^\top$,
and can be compactly written as 
$\phi\!\!=\!\!(\phi_1^\top,\dots,\phi^\top_N)^\top\!\!\!\!=\!\!(I_N\!\!\otimes\!\!H)e$.
The positive orthant $\{\phi\!\!\in\!\!\R^{Nn}\!\!:\!\!\phi\!\!\geq\!\!{0}\}$  is identical with the positive cone $\Omega$. Furthermore, $I_N\!\otimes\!H$ is invertible if and only if $H$ is invertible.
Indeed, matrix $H$ is the observability matrix of the pair $(-\eta_1^\top,A\!\!+\!\!\lambda I)$, while yields zero-state observability {\it{i.e.,}} suppose a continuous linear system $\dot x\!\!=\!\!(A\!\!+\!\!\lambda I)x$, $x\!\!\in\!\!\R^n$, $y\!\!=\!\!-\eta_1^\top x\!\!\in\!\!\R$,  if  $y\!\!=\!\!0$, one has $x\!\!=\!\!\textbf{0}$. 
Thus $H$ and $I_N\!\!\otimes\!\!H$ are invertible, and 
$e\!\!=\!\!(I_N\!\!\otimes\!\!H^{-1})\phi$.
Besides, since $h_n B\!\!=\!\!-1$, then
\begin{equation*}\begin{aligned}
    \dot\phi_{i,n}\!\!=\!\!h_{n} \dot e_i
    \!\!=\!\!h_{n}A e_i\!\!-\!\!h_nBK_{lin} e_i
      %\!\!=\!\!h_{n}Ae_i\!\!-\!\!h_n(A\!\!+\!\!\lambda I_n)e_i
      \!\!=\!\!-\lambda h_n e_i
      \!\!=\!\!-\lambda\phi_{i,n}.
\end{aligned}\end{equation*}
Together \eqref{eq:varphidef} we have 
$    \dot\phi_i\!\!=\!\!(A\!\!-\!\!\lambda I_{n})\phi_i$,
and
\begin{equation}\label{eq:barr_dy}\begin{aligned}
    \dot\phi\!\!=\!\!(I_N\!\!\otimes\!\!(A\!\!-\!\!\lambda I_{n}) )\phi.
\end{aligned}\end{equation}
 Since $I_N\!\!\otimes\!\!(A\!\!-\!\!\lambda I_{n})$ is Metzler, then $\phi$-system \eqref{eq:barr_dy} is positive \cite{farina2011positive} and $\Omega\!\!=\!\!\{\phi\!\!\in\!\!\R^{Nn}\!:\!\phi\!\!\geq\!\!{0}\}$ be strictly positively invariant. 


Next is to prove $\phi(e(0))\!\!=\!\!(\phi_1^\top(e_1(0)),\dots,\phi^\top_N(e_N(0)))^\top\!\!\!\geq\!\!{0}$. The latter inequality is guaranteed by $\phi_i(e_i(0))\!\!\geq\!\!{0}$, $\forall i\!\!=\!\!\overline{1,N}$, and $\phi_i(e_i(0))\!\!\geq\!\!{0}$ is guaranteed by $\phi_{i,k}(e_i(0))\!\!\geq\!\!{0}$, $\forall k\!\!=\!\!\overline{1,n}$.
Indeed, for any $k\!\!\geq\!\!2$, we have 
$    \phi_{i,k}(e_i(0))\!\!=\!\!h_ke_i(0)
    %&\!\!=\!\!-\xi^\top_1(A\!\!+\!\!\lambda I_n)^{k-1}e_i(0)\\
    % \!\!=\!\!h_1(A\!\!+\!\!\lambda I_n)^{k-1}e_i(0)
    \!\!=\!\!\sum\nolimits_{\zeta=0}^{k-1}C_\zeta^{k-1}\lambda^\zeta h_1A^{k\!-\!1\!-\!\zeta}e_i(0)$.
Notice that for $\zeta\!\!=\!\!k\!\!-\!\!1$, we have $h_1A^0\!\!=\!\!-\eta_1^\top$; for $\zeta\!\!=\!\!k\!\!-\!\!2$, we have $h_1A\!\!=\!\!-\eta_2^\top$, \textit{etc.} Then,  
    $\phi_{i,k}(e_i(0))
    \!\!=\!\!-\!\!\sum\nolimits_{\zeta=0}^{k-1}C_\zeta^{k-1}\lambda^\zeta\eta^\top_{k-\zeta}e_i(0)$.
Therefore, $\phi_{i,k}(e_i(0))\!\!\geq\!\!0$, $\forall k\!\!=\!\!\overline{2,n}$, $\forall i\!\!=\!\!\overline{1,N}$  provided \eqref{eq:lambda} holds. The latter implies $\phi(e(0))\!\!\!\geq\!\!{0}$, {\it i.e.,} $e(0)\!\!\in\!\!\Omega$.

Finally, notice that equation \eqref{eq:barr_dy} is asymptotically stabilized to the origin. Recall $e\!\!=\!\!(I_N\!\!\otimes\!\!H^{-1})\phi$, equation \eqref{eq:error_closed} has solution $e(t)\!\!=\!\!(I_N\!\!\otimes\!\!H^{-1})\exp( I_{N}\!\!\otimes\!\!(A\!\!-\!\!\lambda I)t)(I_N\!\!\otimes\!\!H)e(0)$, which means the consensus error $e\!\!\in\!\!\R^{Nn}$ is asymptotically stable. 
\end{proof}

\begin{Coro}
{\it Given $e(0)\!\!\in\!\!\mathrm{int}\Sigma$, inequality \eqref{eq:lambda} always holds if $\lambda\!\!\in\!\!\R_+$ is large enough.} 
\end{Coro}
\begin{proof}
   $e(0)\!\!\in\!\!\mathrm{int}\Sigma$ implies $\phi_{i,1}(0)\!\!\geq\!\!0$, $\forall i\!\!=\!\!\overline{1,N}$. Besides, inequality \eqref{eq:lambda} can be written as 
\begin{equation*}\begin{aligned}
    -\lambda^{k-1}\!\!\phi_{i,1}(0)\!\!+\!\!\sum\nolimits_{\zeta=0}^{k-2}C_\zeta^{k-1}\lambda^\zeta\eta^\top_{k-\zeta}e_i(0)\!\!\leq\!\!{0},\;\; \forall k\!\!=\!\!\overline{2,n},\;\forall i\!\!=\!\!\overline{1,N},
\end{aligned}\end{equation*}
which always holds for a sufficient large $\lambda\!\!\in\!\!\R_+$.
\end{proof}


% By a proper scaling of the control gain $K_{lin}$, the linear control given by \eqref{eq:lin_control} can be upgraded into a homogeneous one \cite{wang2021generalized,li2023generalized,polyakov2020generalized}. 
 %Let us recall the basic idea of this operation. 
% For a multi-input system 
% \begin{equation*}
% \dot x\!\!=\!\!Ax\!\!+\!\!Bu,
% \end{equation*}
% where
% $x\!\!\in\!\! \mathbb{R}^n$, $u\!\!\in\!\! \mathbb{R}^m$, $A\!\!\in\!\!\mathbb{R}^{n\times n}$ be nilpotent, $B\!\!\in\!\!\mathbb{R}^{n\times m}$, $(A,B)$ be controllable. 
% It can be shown \cite{wang2021generalized} that
%    the linear stabilization controller
% \begin{equation}\label{eq:lin_single}
% u\!\!=\!\!Kx,\;\; K\!\!\in\!\! \mathbb{R}^{m\times n}
% \end{equation}
% can be transformed into a homogeneous form
% \begin{equation}\label{eq:homo_single}
% u\!\!=\!\!\|x\|^{\mu+1}_{\dn}\!\!K\dn(-\ln\|x\|_{\dn})x, 
% \end{equation} 
% such that the closed-loop multi-input system be finite-time stable for $\mu\!\!\in\!\![-1,0)$ and practically fixed-time stable  for $\mu\!\!>\!\!0$, where $\dn$ is a linear dilation in $\R^n$ and $\|\cdot\|_{\dn}$ is the canonical homogeneous norm.  The transformation from  \eqref{eq:lin_single} to the \eqref{eq:homo_single} is referred to as \textit{upgrading}. This process involves designing an appropriate scaling scheme for the linear control gain $K$. 
%In this paper, a similar scheme is developed by using the special structure of the transmitted vector $v_i$, $i\!\!=\!\!\overline{1,N}$.





\subsection{Finite-time Non-overshooting Consensus }
 By a proper scaling of the control gain $K_{lin}$, the linear control given by \eqref{eq:lin_control} can be upgraded into a homogeneous one \cite{wang2021generalized,li2023generalized,polyakov2020generalized}. 
In this paper, a similar scheme is developed by using the special structure of the transmitted vector $v_i$, $i\!\!=\!\!\overline{1,N}$.
%In this subsection, a homogeneous non-overshooting consensus protocol is designed by upgrading the linear one \eqref{eq:lin_control}.  With this control protocol, the finite-time non-overshooting leader-following consensus is guaranteed.

\begin{thm}\label{thm:finite_nonovershoot}
\it{Let $\mu\!\!\in\!\![-1,0)$. Let $P\!\!\in\!\!\R^{n\!\times\!n}$ be the solution of the following LMI:
\begin{equation}\label{eq:LMI_P}
\begin{aligned}
   P\!\!\succ\!\!0,\quad PG_\dn\!\!+\!\!G_\dn P\!\!\succ\!\!0, \quad P(A\!\!-\!\!BK_{lin})\!\!+\!\!(A\!\!-\!\!BK_{lin})^\top\!\!\! P\!\!\prec\!\!0,
\end{aligned}
\end{equation}
where $G_\dn\!\!=\!\!\diag\{1\!\!-\!\!\mu(n\!\!-\!\!k)\}_{k\!=\!1}^n$,  $K_{lin}$ is defined in \eqref{eq:lin_control}. Let $\dn$ be a dilation group generated by $G_\dn$. Let the transmitted vector $v_i\!\!\in\!\!\R^n$ be defined in \eqref{eq:def_vi},
and the homogeneous consensus control protocol
\begin{equation}\label{eq:homo_control_nonover}
 	u_i\!\!=\!\!-\|v_i\|_{\dn}^{1+\mu}K_{lin}\dn(-\ln\|v_i\|_{\dn})v_i,\;\; i\!\!=\!\!\overline{1,N}
 \end{equation}
with $\|\cdot\|_\dn$ be induced by the weighted Euclidean norm $\|\cdot\|_P$,
such that the error equation \eqref{eq:nonovershooterrordy} be globally finite-time stable and 
the homogeneous cone\footnote{A non-empty set $\Omega_\dn\!\!\in\!\!\R^n$ is said to be a homogeneous cone if $x\!\!\in\!\!\Omega_\dn\!\!\Rightarrow\!\!\dn(s)x\!\!\in\!\!\Omega_\dn$, $\forall s\!\!\in\!\!\R$.}
$$\Omega_{\dn}\!\!=\!\!\{e\!\!\in\!\!\R^{Nn}:\diag\{H\dn(-\ln \|e_i\|_{\dn})\}_{i=1}^Ne\!\!\geq\!\!{0}\}$$ be a strictly positively invariant set for the equation \eqref{eq:nonovershooterrordy}, and $e(0)\!\!\in\!\!\Omega_{\dn}\!\!\subset \!\!\Sigma$
if $e(0)\!\!\in\!\!\Omega$ and $\|e_i(0)\|_{ P}\!\!\leq\!\!1$, $\forall i\!\!=\!\!\overline{1,N}$, with $\Omega\!\!\subset\!\! \Sigma$  and $H$ are defined in \eqref{eq:lin_positive_cone}.
}

\end{thm}

\begin{proof}
Recall Theorem \ref{thm:state_con}, equation \eqref{eq:def_vi} has a unique solution $v\!\!=\!\!e$, then the equation \eqref{eq:homo_control_nonover} becomes
\begin{equation*}\begin{aligned}
u\!\!&=\!\!-\diag\{\|e_i\|_{\dn}^{1+\mu}\!\!K_{lin}\dn(\!\!-\!\!\ln\!\!\|e_i\|_{\dn})\}_{i=1}^Ne,\;\;u\!\!=\!\!(u_1,\dots,u_N)^\top\!\!\!\in\!\!\R^N.
\end{aligned} \end{equation*} 
Thus the closed-loop error equation \eqref{eq:nonovershooterrordy} becomes
\begin{equation}\label{eq:exp_error_nonover}\begin{aligned}
 	\dot e&\!\!=\!\!f(e)\\
    &\!\!=\!\!\!\left(\!\!I_N\!\!\otimes\!\!A\!\!-\!\!\diag\{\|(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn}^{1+\mu}\!\!BK_{lin}\dn(-\!\!\ln\!\!\|(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn})\}_{i=1}^N\!\!\right)\!\!e.
\end{aligned} \end{equation}
Similar with \eqref{eq:exp_error_dy}, the error equation \eqref{eq:exp_error_nonover} is component-wise decoupled and the stability of $e\!\!\in\!\!\R^{Nn}$ is equivalent to $e_i\!\!\in\!\!\R^n$, $i\!\!=\!\!\overline{1,N}$. Select $\|e_i\|_\dn$ as the Lyapunov candidate, and repeat the analysis in Theorem \ref{thm:state_con}, we can obtain the homogeneity of $e\!\!\mapsto\!\!f(e)$ and $e_i\!\!\mapsto\!\!f_i(e_i)$ as well as $\tfrac{d\|e_i\|_\dn}{dt}\!\!<\!\!0$, $i\!\!=\!\!\overline{1,N}$ since \eqref{eq:LMI_P} holds. Thus the homogeneous error equation 
\eqref{eq:exp_error_nonover} is globally finite-time stable for $\mu\!\!\in\!\![-1,0)$.


Consider the homogeneous barrier function $\phi_i\!\!:\!\!\R^{n}\!\!\to\!\!\R^{n}$ as 
$\phi_i(e_i)\!\!=\!\!H\dn(-\ln \|e_i\|_{\dn})e_i$. Then, 
\begin{equation*}\begin{aligned}
% \tfrac{d\phi_i}{dt}\!\!=&\!-\!\tfrac{\frac{d \|e_i\|_{\dn}}{dt}}{\|e_i\|_{\dn}}HG_\dn\dn(-\ln \|e_i\|_{\dn})e_i\!\!+\!\!H\dn(-\ln \|e_i\|_{\dn})\tfrac{d e_i}{dt}\\
\tfrac{d\phi_i}{dt}\!\!=\!\!-\!\tfrac{\frac{d \|e_i\|_{\dn}}{dt}}{\|e_i\|_{\dn}}&HG_\dn\dn(-\ln \|e_i\|_{\dn})e_i\\
&\!\!+\!H\dn(-\ln \|e_i\|_{\dn})\!\!\!\left(
\!\!A\!\!-\!\!\|e_i\|_{\dn}^{1+\mu}\!BK_{lin}\dn(-\ln\|e_i\|_{\dn})\!\!\right)\!\!e_i.
\end{aligned}\end{equation*}
Reusing $\dn(s)A\!\!=\!\!\exp(-\mu s)A\dn(s)$, $\dn( s)B\!\!=\!\!\exp(s)B$, $\forall s\!\!\in\!\!\R$ has
\begin{equation*}\begin{aligned}
&\tfrac{d\phi_i}{dt}
\!\!=\!\!\\&-\!\tfrac{\frac{d \|e_i\|_{\dn}}{dt}}{\|e_i\|_{\dn}}HG_\dn\dn(-\ln \|e_i\|_{\dn})e_i\!\!
+\!\!\|e_i\|_{\dn}^\mu H(A\!\!-\!\!BK_{lin})\dn(-\ln\|e_i\|_{\dn})e_i,
\end{aligned}\end{equation*}
and straightforwardly
\begin{equation}\label{eq:add}\begin{aligned}
\tfrac{d\phi_i}{dt}
\!\!=\!\!\|e_i\|_{\dn}^\mu H(A\!\!-\!\!BK_{lin}\!\!+\!\gamma_i G_\dn)\dn(-\ln \|e_i\|_{\dn})e_i,
\end{aligned}\end{equation}
where $\gamma_i\!\!=\!\!-\|e_i\|_{\dn}^{-\mu-1}\!\frac{d \|e_i\|_{\dn}}{dt}\!\!>\!\!0$,  $ e_i\!\!\in\!\!\R^{n}\backslash\{\textbf{0}\}$, $\forall i\!\!=\!\!\overline{1,N}$.
According to Theorem \ref{thm:linear}, 
$H(A\!\!-\!\!BK_{lin})H^{-1}\!\!=\!\!A\!\!-\!\!\lambda I_{n}$, which implies $H(A\!\!-\!\!BK_{lin})\!\!=\!\!(A\!\!-\!\!\lambda I_{n})H$. Besides, 
$HG_\dn\!\!=\!\!H(I_n\!\!+\!\!\Pi)\!\!=\!\!H\!\!+\!\!(
   \Pi^\top   h_1^\top,
     \ldots,
    \Pi^\top h_n^\top  
)^\top$, $\Pi\!\!=\!\!\diag\{\!-\!\mu(n\!\!-\!\!k)\}_{k\!=\!1}^n$.
We notice 
$h_k  \Pi \!\!=\!\!-\mu(n\!\!-\!\!k)h_k\!\!-\!\!\lambda\mu(k\!\!-\!\!1) h_{k-1}$,
which indicates 
% \begin{equation*}\begin{aligned}
%  \left(\begin{smallmatrix}
%      h_1 \Pi  \\
%      h_2 \Pi  \\
%      \vdots \\
%      h_n \Pi  \\
%  \end{smallmatrix}\right)\!\!=&\diag\{-\!\mu(n\!\!-\!\!k)\}_{k=1}^n H\!\!+\!\lambda\diag\{-\!\mu(k\!\!-\!\!1)\}_{k=1}^n A^\top\!\! H.
% \!\!=&\diag\{-\!\mu(n\!\!-\!\!k)\}_{k=1}^n H\!\!+\!\lambda((\mu(1\!\!-\!\!n)\!\!+\!\!1)I_n\!\!-\!\!G_\dn) A^\top\!\! H.
% \end{aligned}\end{equation*}
% In this case, we have 
$
HG_\dn
% \!\!=&\!H\!\!+\!\!H\Pi\\
% \!\!=\!\!\!H\!\!+\!\!\Pi H\!\!+\!\lambda\diag\{-\!\mu(k\!\!-\!\!1)\}_{k=1}^n A^\top\!\! H
% \!\!=&G_\dn H\!\!+\!\lambda\diag\{-\!\mu(k\!\!-\!\!1)\}_{k=1}^n A^\top\!\! H\\
\!\!=\!\! \Gamma H$
with $\Gamma\!\!=\!\!G_\dn \!\!+\!\lambda\diag\{-\!\mu(k\!\!-\!\!1)\}_{k=1}^n A^\top$.
Then \eqref{eq:add} becomes
\begin{equation}\label{eq:homo_phi_i}\begin{aligned}
\tfrac{d\phi_i}{dt}
% \!\!=&\|e_i\|_{\dn}^\mu H(A\!\!-\!\!BK_{lin}\!\!+\!\gamma_i G_\dn)\dn(-\ln \|e_i\|_{\dn})e_i\\
% \!\!=&\|e_i\|_{\dn}^\mu(A\!\!-\!\!\lambda I_{n}\!\!+\!\!\gamma_i\Gamma)H\dn(-\ln \|e_i\|_{\dn})e_i\\
\!\!=\!\!\|e_i\|_{\dn}^\mu(A\!\!-\!\!\lambda I_{n}\!\!+\!\!\gamma_i\Gamma)\phi_i.
\end{aligned}\end{equation}
Notice that $\Gamma\!\!\geq\!\!0$ for $\mu\!\!\in\!\![-1,0)$. This directly implies $A\!\!-\!\!\lambda I_{n}\!\!+\!\!\gamma_i\Gamma$ is Metzler.
%and $\phi_i$-system \eqref{eq:homo_phi} is positive \cite{farina2011positive}. 
Let $\phi_i$ be compactly presented as $\phi\!\!=\!\!(\phi_1^\top,\dots,\phi_N^\top)^\top\!\!=\!\!\diag\{H\dn(-\ln \|e_i\|_{\dn})\}_{i=1}^Ne$, with the dynamics
\begin{equation}\label{eq:homo_phi}\begin{aligned}
\tfrac{d\phi}{dt}
\!\!=\!\!(
     \tfrac{d^\top\!\!\!\phi_1}{dt},
     \ldots,
     \tfrac{d^\top\!\!\!\phi_N}{dt} 
)^\top\!\!\!\!=\!\!\diag\{\|e_i\|_{\dn}^\mu(A\!\!-\!\!\lambda I_{n}\!\!+\!\!\gamma_i\Gamma)\}_{i=1}^N\phi\!\!:=\!\!\Lambda\phi.
% \left(\begin{smallmatrix}
%      \|e_1\|_{\dn}^\mu(A\!-\!\lambda I_{n}\!+\!\gamma_1\Gamma) & \ldots & \textbf{0}_{n\times n} \\
%      \vdots & \ddots & \vdots \\
%           \textbf{0}_{n\times n} & \ldots & \|e_N\|_{\dn}^\mu(A\!-\!\lambda I_{n}\!+\!\gamma_N\Gamma) \\
% \end{smallmatrix}\right)
%      \!\!\phi\!\!:=\!\!\Lambda\phi.
\end{aligned}\end{equation}
Thus $\phi$-system \eqref{eq:homo_phi} is positive since $\Lambda\!\!\in\!\!\R^{Nn\!\times\!Nn}$ being Metzler \cite{farina2011positive}, and the homogeneous cone $\Omega_{\dn}\!\!=\!\!\{\phi\!\!\in\!\!\R^{Nn}:\phi\!\!\geq\!\!{0}\}$ is a strictly positively invariant set, which means for $e(0)\!\!\in\!\!\Omega_{\dn}\!\!\Rightarrow\!\!e(t)\!\!\in\!\!\Omega_{\dn}$, $\forall t\!\!\in\!\!\R_+$. Moreover, $\Omega_{\dn}\!\!\subset\!\!\Sigma$ by construction.

Next, we are supposed to prove $e(0)\!\!\in\!\!\Omega_{\dn}$, {\it{i.e.,}} $\phi(e(0))\!\!\geq\!\!{0}$, with
$\phi(e(0))\!\!=\!\!\diag\{H\dn(-\ln\|e_i(0)\|_\dn)\}_{i=1}^Ne(0)$.
%\!\!=&\!(I_N\!\!\otimes\!\!(H\dn(-\ln \|e(0)\|_{\tilde\dn})))e(0),\\
% \!\!=&\left(\begin{array}{cc}
%      H\dn(-\ln \|e(0)\|_{\tilde\dn})e_1(0)  \\
%      H\dn(-\ln \|e(0)\|_{\tilde\dn})e_2(0)  \\
%      \vdots \\
%      H\n(-\ln \|e(0)\|_{\tilde\dn})e_N(0)  \\
% \end{array}\right)
On the one hand, for all 
$i\!\!=\!\!\overline{1,N}$, $\|e_i(0)\|_P\!\!\leq\!\!1\!\!\Leftrightarrow\!\!\|e_i(0)\|_{\dn}\!\!\leq\!\!1\!\!\Leftrightarrow\!\!-\ln \|e_i(0)\|_{\dn}\!\!\geq\!\!0$ and $\|e_i(0)\|_P\!\!=\!\!1\!\!\Leftrightarrow\!\!\|e_i(0)\|_{\dn}\!\!=\!\!1\!\!\Leftrightarrow\!\!-\ln \|e_i(0)\|_{\dn}\!\!=\!\!0\!\!\Leftrightarrow\!\!\phi(e(0))\!\!=\!\!(I_N\!\!\otimes\!\!H)e(0)$. 
On the other hand, 
let $\phi_s:\R\!\!\to\!\!\R^{n}$ with an auxiliary function be
$\phi_s(s)\!\!=\!\!H\dn(s)x$, $s\!\!\in\!\!\R_{\geq0}$, $x\!\!\in\!\!\R^{n}$,
yields $\phi_s(0)\!\!=\!\!Hx\!\!\geq\!\!{0}$. We prove $\phi_s(s)$ is non-decreasing on $s\!\!\in\!\!\R_{\geq0}$. Indeed, 
$\tfrac{d\phi_s}{ds}
\!\!=\!\!H G_\dn\dn(s)x
\!\!=\!\!\Gamma \phi_s$,
% we consequently have 
% \begin{equation*}\begin{aligned}
% \phi_s(s)
% \!\!=\!\!\phi_s(0)\exp((I_N\!\otimes\!\Gamma)s). 
% \end{aligned}\end{equation*}
with
$\Gamma\!\!=\!\!G_\dn \!\!+\!\lambda\diag\{-\!\mu(k\!\!-\!\!1)\}_{k=1}^n A^\top$.
Notice that for $\mu\!\!\in\!\![-1,0)$, $\Gamma$ is anti-Hurwitz since it is a lower-triangular matrix with positive diagonal entries.
% $G_\dn$ is a diagonal matrix with positive entries, while $\lambda\diag\{-\!\mu(k\!\!-\!\!1)\}_{k=1}^n$ is a diagonal matrix with non-negative entries and 
% $\lambda\diag\{-\!\mu(k\!\!-\!\!1)\}_{k=1}^n A^\top$ is a lower-triangular matrix with zero diagonal elements, thus $\Gamma$ is anti-Hurwitz. 
Therefore,  
$\phi_s(s)\!\!\geq\!\!{0}$, $\forall s\!\!\in\!\!\R_{\geq0}$. 
% since for $\phi_s(0)\!\!\geq\!\!{0}$, $\phi_s(s)$ strictly increasing on $s\!\!\in\!\!\R_{\geq0}$. 
Based on the above, we have $\phi_i(e_i(0))\!\!\geq\!\!{0}$ if 
$\|e_i(0)\|_P\!\!\leq\!\!1$ and $He_i(0)\!\!\geq\!\!{0}$, $\forall i\!\!=\!\!\overline{1,N}$, and it is concluded as $\phi(e(0))\!\!\geq\!\!{0}$ provided 
$\|e_i(0)\|_P\!\!\leq\!\!1$, $\forall i\!\!=\!\!\overline{1,N}$ and $e(0)\!\!\in\!\!\Omega$.
\end{proof}


\subsection{Robustness Analysis}\label{RA}
Now we move to the disturbed case by considering the model uncertainty defined in \eqref{eq:dynamic_disturb}. The error equation is \begin{equation}\label{eq:exp_error_dy_disturb_non}\begin{aligned}
 	&\dot e\!\!=\!\!f(e,q)\\
  &\!\!=
    \!\!\!\left(\!\!I_N\!\!\otimes\!\!A
    \!\!-\!\!\diag\{\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn}^{1\!+\!\mu}\!BK_{lin}\dn(\!-\!\!\ln\!\!\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)e\|_{\dn})\}_{i=1}^N\!\!\right)\!\!e\!\!+\!\!q.
\end{aligned} \end{equation}
 with $q\!\!=\!\!((q_{1}\!\!-\!\!q_0)^\top,\dots,(q_{N}\!\!-\!\!q_0)^\top)^\top\!\!\!\in\!\!L^\infty\!(\R,\R^{Nn})$.

 Before analysis, according to \cite{boyd1994linear}, we claim $P(A\!\!-\!\!BK_{lin})\!\!+\!\!(A\!\!-\!\!BK_{lin})^\top\!\!\! P\!\!\prec\!\!0$ defined in \eqref{eq:LMI_P} of Theorem \ref{thm:finite_nonovershoot} implies that there exists $\rho\!\!\in\!\!\R_+$ such that
 \begin{equation}\label{eq:LMI_new}
    P(A\!\!-\!\!BK_{lin})\!\!+\!\!(A\!\!-\!\!BK_{lin})^\top\!\!\! P\!\!+\!\!\rho P\!\!\prec\!\!0.
 \end{equation}
% some transmission noise and model uncertainties. The disturbed transmitted data is presented as $x_i(t)\!\!+\!\!q_{x_i}(t)$ and $v_i(t)\!\!+\!\!q_{v_i}(t)$, $q_{x_i}\!\!\in\!\!L^\infty(\R,\R^n)$,  $q_{v_i}\!\!\in\!\!L^\infty(\R,\R^n)$, $i\!\!=\!\!\overline{0,N}$.
% The agent dynamic \eqref{eq:dynamic} considering some model uncertainties is as follows, 
% \begin{equation}\label{eq:dynamic_disturb}
% \begin{aligned}
%  &\dot x_{i}(t)\!\!=\!\!Ax_i(t)\!\!+\!\!Bu_i(t)\!\!+\!\!q_{m_i}(t),\;\; q_{m_i}\!\!\in\!\!L^\infty\!(\R,\R^{n}),\;i\!\!=\!\!\overline{0,N}, \;t\!\!>\!\!0.
% \end{aligned}
% \end{equation}
% With the considered disturbance, the equation \eqref{eq:def_vi} becomes
% \begin{equation}\label{eq:def_vi_disturb}\begin{aligned}
% v_i\!\!=\!\!\tfrac{1}{\sum_{j=0}^N\!w_{ij}}\!\!\sum\nolimits_{j=0}^N \!\!w_{ij}\!\!\left(x_i\!\!-\!\!x_j\!\!+\!\!v_j\!\!+\!\!d_j\right),\; d_j\!\!=\!\!q_{v_j}\!\!-\!\!q_{x_j},\;i\!\!=\!\!\overline{1,N}.
%  \end{aligned}\end{equation}
% where $v_0\!\!=\!\!\textbf{0}$, and $d_j\!\!\in\!\!L^\infty\!(\R,\R^n)$.




% \begin{lem}\label{lem:unique_vi_disturb}
%     \textit{Let matrix $\tilde{\mathcal{W}}\!\!\in\!\!\R^{N\!\times\!(N\!+\!1)}$ be inducted by eliminating the first line of the adjacency matrix $\mathcal{W}\!\!\in\!\!\R^{(N\!+\!1)\!\times\!(N\!+\!1)}$ of the studied graph. The algebraic equation \eqref{eq:def_vi_disturb} has a unique solution $ v\!\!=\!\! e\!\!+\!\!q_a$, where $q_a\!\!=\!\!(\TL^{-1}\tilde{\mathcal{W}}\!\!\otimes\!\!I_n)d\!\!\in\!\!L^\infty(\R,\R^{Nn})$, $\TL$ is defined in  Lemma \ref{lem:unique},  $d\!\!=\!\!(d_0^\top,\ldots,d_N^\top)^\top\!\!\!\!\in\!\!L^\infty(\R,\R^{(N\!+\!1)n})$.}
% \end{lem}

% \begin{proof}
%   Recall the analysis of Lemma \ref{lem:unique}, \eqref{eq:def_vi_disturb} becomes
%     % \begin{equation*}
%     % \begin{aligned}
% % \sum\nolimits_{j=0}^Nw_{ij} v_i\!\!-\!\!\sum\nolimits_{j=1}^N w_{ij}v_j\!\!=&\!\sum\nolimits_{j=0}^N w_{ij}(x_i\!\!-\!\!x_j)\!\!+\!\!\sum\nolimits_{j=0}^N w_{ij}d_j\\
% $(\TL_i\!\!\otimes\!\!I_n) v\!\!=\!\!(\TL_i\!\!\otimes\!\!I_n) e\!\!+\!\!({\mathcal{W}}_i\!\!\otimes\!\!I_n)d$,
%  % \end{aligned}
%  % \end{equation*}
%  where ${\mathcal{W}}_i$ is the $i_{th}$, $i\!\!=\!\!\overline{1,N}$ line of matrix $\mathcal{W}$. The latter equation yields a compact form
%  $(\TL\!\!\otimes\!\!I_n) v\!\!=\!\!(\TL\!\!\otimes\!\!I_n) e\!\!+\!\!(\tilde{\mathcal{W}}\!\!\otimes\!\!I_n) d$. Since $\TL$ is invertiable, the unique solution of \eqref{eq:def_vi_disturb} be $ v\!\!=\!\! e\!\!+\!\!q_a$.
% \end{proof}

%     Lemma \ref{lem:unique_vi_disturb} immediately implies \eqref{eq:homo_control_nonover} becomes 
%     \begin{equation}\label{eq:homo_control_disturb}
%  	    u\!\!=\!\!\diag\{\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!(e\!\!+\!\!q_a)\!\|_{\dn}^{1\!+\!\mu}\!\!K_{lin}\dn(\!-\!\!\ln\!\!\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!(e\!\!+\!\!q_a)\!\|_{\dn})\}_{i=\!1}^N\!\!(e\!\!+\!\!q_a). 
%  \end{equation}
% Taking the disturbance into consideration, the closed-loop error equation \eqref{eq:exp_error_nonover} becomes
% \begin{equation}\label{eq:exp_error_dy_disturb}\begin{aligned}
%  	&\dot e\!\!=\!\!f(e,q)\!\!=
%     \!\!(I_N\!\!\otimes\!\!A)e\!\!+\!\!q_b\\&
%     \!\!-\!\!\diag\{\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!(e\!\!+\!\!q_a)\!\|_{\dn}^{1\!+\!\mu}\!\!BK\dn(\!-\!\!\ln\!\!\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!(e\!\!+\!\!q_a)\!\|_{\dn})\}_{i=1}^N\!(e\!\!+\!\!q_a),
% \end{aligned} \end{equation}
% where $f\!:\!\R^{Nn}\!\!\times\!\!\R^{2Nn}\!\!\to\!\!\R^{Nn}$, $q_b\!\!=\!\!(q_{m_1}^\top\!\!\!\!-\!\!q_{m_0}^\top,\dots,q_{m_N}^\top\!\!\!\!-\!\!q_{m_0}^\top)^\top\!\!\!\!\!\in\!\!L^\infty\!(\R,\R^{Nn})$, and $q\!\!=\!\!(q_a^\top\!\!,q_b^\top)^\top\!\!\!\!\in\!\!L^\infty\!(\R,\R^{2Nn})$. 


\begin{Coro}\label{prop:1}
    \textit{Let the conditions of Theorem \ref{thm:finite_nonovershoot} hold. Then,
    \\
    $a)$ for $\mu\!\!\in\!\!(-1,0)$, the closed-loop error equation \eqref{eq:exp_error_dy_disturb_non} is ISS with respect to $q\!\!\in\!\!L^\infty\!(\R,\R^{Nn})$;
    \\
    $b)$ for $\mu\!\!\in\!\!(-1,0)$, and $q\!\!\in\!\!L^\infty\!(\R,\R_{-}^{Nn})$, the homogeneous cone
     $\Omega_{\dn}\!\!=\!\!\{e\!\!\in\!\!\R^{Nn}\!:\!\diag\{H\dn(-\ln \|e_i\|_{\dn})\}_{i=1}^Ne\!\!\geq\!\!{0}\}$ is  strictly positively invariant for equation \eqref{eq:exp_error_dy_disturb_non};
    \\
    $c)$ for $n\!\!=\!\!2$, $\mu\!\!=\!\!-1$, and $q_i\!\!=\!\!B\hat q_i$, $\hat q_i\!\!\in\!\!L^\infty(\R,\R)$, $i\!\!=\!\!\overline{0,N}$
    the error equation \eqref{eq:exp_error_dy_disturb_non} is globally finite-time stable and the homogeneous cone $\Omega_{\dn}\!\!=\!\!\{e\!\!\in\!\!\R^{2N}\!:\!\diag\{H\dn(-\ln \|e_i\|_{\dn})\}_{i=1}^Ne\!\!\geq\!\!{0}\}$ is  strictly positively invariant  for the error equation \eqref{eq:exp_error_dy_disturb_non} if 
    \begin{equation}\label{eq:upperq}
     \|\hat q_i\!\!-\!\!\hat q_0\|_{L^\infty}\!\!\leq\!\!\min\left\{\tfrac{\rho}{2|P^{1/2}|},\tfrac{\lambda\vartheta\;\lambda_{\min}(P^{-1/2}H^\top HP^{-1/2})}{\lambda^{1/2}_{\max}(P^{-1/2}\eta_1\eta_1^\top P^{-1/2})}\right\},\;\;\forall i\!\!=\!\!\overline{1,N}
     % {\color{red}\min_{i=\overline{1,N}}\tfrac{\lambda|\phi_i|^2\vartheta}{\phi_{i,1}}}
    %\text{find an explicit value}
    \end{equation}
    % and there exists $\sigma\!\!\in\!\!\R_{\geq0}$ such that
    % \begin{equation}\label{eq:con_sigma}\color{red}
    %     (n\!\!-\!\!1)\lambda\vartheta\phi_{i,n\!-\!1}\!\!+\!\!(\vartheta\!\!-\!\!\lambda\!\!+\!\!\sigma)\phi_{i,n}\!\!+\!\hat q_0\!\!-\!\!\hat q_i \!\!\geq\!\!0, \;\;\forall i\!\!=\!\!\overline{1,N}
    % \end{equation}
    with $\rho\!\!\in\!\!\R_+$ defined in \eqref{eq:LMI_new}, 
    % $\phi_i\!\!=\!\!H\dn(-\ln \|e_i\|_{\dn})e_i\!\!\in\!\!\R^2$, 
and $\vartheta\!\!=\!\!\tfrac{\rho}{2\lambda_{\max}(P^{-1/2}(PG_\dn \!+\!G_\dn P)P^{-1/2})}$.
    % , and $\phi_{i,1}\!\!\in\!\!\R$ is the first component of $\phi_i$.
    %$\vartheta\!\!=\!\!\tfrac{1}{2}\rho|P^{-1/2}(PG_\dn \!\!+\!\!G_\dn P)P^{-1/2}|^{-1}$.
}
    
\end{Coro}

\begin{proof}
%     Let $e\!\!\to\!\!\tilde\dn(s)e$, $q\!\!\to\!\!\tilde\dn_q (s)q$, $\tdn_q(s)\!\!=\!\!\left(\begin{smallmatrix}
%         1 & 0\\
%         0 & \exp(\mu s)
%     \end{smallmatrix}\right)\!\!\otimes\!\tilde\dn(s)$, $\forall s\!\!\in\!\!\R$. 
% Then, we have $f(\tilde\dn(s)e,\tilde\dn_q (s)q)\!\!=\!\!\exp(\mu s)\tdn(s)f(e,q)$
% \begin{equation*}\begin{aligned}
%     &f_a(\tilde\dn(s)e,\tilde\dn_q (s)q)\!\!=
%     \!\!(I_N\!\!\otimes\!\!A)\tdn(s)e\!\!+\!\!\exp(\mu s)\tdn(s)q_b\\&
%     \!\!-\!\!\diag\{\!\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!\tdn(s)\!(e\!\!+\!\!q_a)\!\|_{\dn}^{1\!+\!\mu}\!\!BK\dn(\!-\!\!\ln\!\!\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!\tdn(s)\!(e\!\!+\!\!q_a)\!\|_{\dn})\!\}_{i=\!1}^N\!\!\\&\!\!\times\!\!\tdn(s)\!(e\!\!+\!\!q_a).
% \end{aligned}\end{equation*}
% by using the formula $(I_N\!\!\otimes\!\!A)\tilde\dn(s)\!\!=\!\!\exp(\mu s)\tilde\dn(s)(I_N\!\!\otimes\!\!A)$, $\exp(s)(I_N\!\!\otimes\!\!B)\!\!=\!\!\tilde\dn( s)(I_N\!\!\otimes\!\!B)$, and $\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!\tdn(s)\!(e\!\!+\!\!q_a)\!\|_{\dn}\!\!=\!\!\|\!\dn(s)\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!(e\!\!+\!\!q_a)\!\|_{\dn}\!\!=\!\!\exp(s)\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!(e\!\!+\!\!q_a)\!\|_{\dn}$. Thus, we can immediately obtain that the vector field $f_q\!:\!\R^{Nn}\!\!\times\!\!\R^{2Nn}\!\!\to\!\!\R^{3Nn}$ with $f_{q}(e,q)\!\!=\!\!\left(\begin{smallmatrix}
%     f(e,q)\\
%     \textbf{0}_{2Nn}
% \end{smallmatrix}\right)$
% be homogeneous of degree $\mu$ with respect to the dilation $\left(\begin{smallmatrix}
%     e\\
%     q
% \end{smallmatrix}\right)\!\!\to\!\!\left(
%                                              \begin{smallmatrix}
%                                                \tilde \dn(s) & \mathbf{0}_{Nn\!\times\! 2Nn} \\
%                                                \mathbf{0}_{2Nn\!\times\! Nn} & \tilde\dn_q(s) \\
%                                              \end{smallmatrix}
%                                            \right)
% \left(\begin{smallmatrix}
%     e\\
%     q
% \end{smallmatrix}\right)$, $\forall s\!\!\in\!\!\R$. Together the stability of the  error equation $\dot e\!\!=\!\!f(e,\textbf{0})$ offered by Theorem \ref{thm:finite_nonovershoot}, we conclude the error equation \eqref{eq:exp_error_dy_disturb} is ISS with respect to $q\!\!\in\!\!L^\infty(\R,\R^{2Nn})$ by recalling Lemma \ref{lem:ISS}.
Claim a) is obtained by recalling Corollary \ref{remark:ISS}.

In addition, since $q\!\!\in\!\!L^\infty\!(\R,\R_{-}^{Nn})$, claim a) implies $\tfrac{d\|e_i\|_\dn}{dt}\!\!<\!\!0$, $\forall i\!\!=\!\!\overline{1,N}$ on $e\!\!\in\!\!\R^{Nn}$. Recall Theorem \ref{thm:finite_nonovershoot}, $\Lambda\!\!\in\!\!\R^{Nn\!\times\!Nn}$ defined in \eqref{eq:homo_phi} is Metzler on $e\!\!\in\!\!\R^{Nn}$. 
Consider the homogeneous barrier function $\phi_i\!\!:\!\!\R^{n}\!\!\to\!\!\R^{n}$ as 
$\phi_i(e_i)\!\!=\!\!H\dn(-\ln \|e_i\|_{\dn})e_i$.
Then, 
\begin{equation}\label{eq:homo_phi_iss}\begin{aligned}
\tfrac{d\phi}{dt}&\!\!=\!\!\Lambda\phi
\!\!-\!\!(I_N\!\!\otimes\!\!H)\diag\{\dn(-\!\!\ln \!\!\|e_i\|_{\dn})\}_{i=1}^N \tilde{q},\;\;\phi\!\!=\!\!(\phi_1^\top,\dots,\phi_N^\top)^\top
% &\!\!=\!\!g(\phi)
% \!\!+\!\!(I_N\!\!\otimes\!\!H G_\dn G_\dn^{-1})\diag\{\dn(-\ln \|e_i\|_{\dn})\}_{i=1}^N q.
\end{aligned}\end{equation}
% Since $HG_\dn\!\!=\!\!\Gamma H$, 
% \begin{equation*}\begin{aligned}
% \tfrac{d\phi}{dt}
% &\!\!=\!\!g(\phi)
% \!\!+\!\!(I_N\!\!\otimes\!\!\Gamma H G_\dn^{-1})\diag\{\dn(-\ln \|e_i\|_{\dn})\}_{i=1}^N q.
% \end{aligned}\end{equation*}
where $\tilde q\!\!=\!\!-q\!\!\in\!\!L^\infty\!(\R,\R^{Nn}_{+})$. 
Recall the definition of $H$ in  \eqref{eq:lin_positive_cone}, the matrix $\!\!-\!(I_N\!\!\otimes\!\!H)\diag\{\dn(-\ln \|e_i\|_{\dn})\}_{i=1}^N\!\!\geq\!\!0$. Therefore, the $\phi$-system \eqref{eq:homo_phi_iss} is positive \cite{farina2011positive}, and claim b) is obtained.

For claim c), we have $q\!\!=\!\!(I_N\!\!\otimes\!\!B)(\hat q_1\!\!-\!\!\hat q_0,\ldots,\hat q_N\!\!-\!\!\hat q_0)^\top$ in \eqref{eq:exp_error_dy_disturb_non}. 
It is clear the stability of error equation \eqref{eq:exp_error_dy_disturb_non} is equivalent to the stability of $\dot e_i\!\!=\!\!f_i(e_i,B(\hat q_i\!\!-\!\!\hat q_0))$, $i\!\!=\!\!\overline{1,N}$, $f_i\!\!:\!\!\R^2\!\!\times\!\!\R^2\!\!\to\!\!\R^2$. Let $\|e_i\|_\dn$ be the Lyapunov candidate, whose derivative along $\dot e_i\!\!=\!\!f_i(e_i,B(\hat q_i\!\!-\!\!\hat q_0))$ be
\begin{equation*}\begin{aligned}
&\tfrac{d \|e_i\|_{\dn}}{d t}\\
&\!\!=\!\!\!\tfrac{e_i^{\top}\!\!\!\dn^{\top}\!\!\!(\!\!-\!\!\ln \!\|e_i\|_\dn\!) (P(A\!-\!BK_{lin})\!+\!(A\!-\!BK_{lin} )^\top\!\!\!P)\dn(\!\!-\!\!\ln \!\|e_i\|_\dn\!)e_i\!+\!e_i^{\top}\!\!\dn^{\top}\!\!\!(\!\!-\!\!\ln \!\|e_i\|_\dn\!) PB(\hat q_i\!-\!\hat q_0) }
{e_i^{\top}\dn^{\top}\!\!\!(-\ln \|e_i\|_\dn)(PG_{\dn}+G_\dn P)\dn(-\ln \|e_i\|_\dn)e_i}.
	\end{aligned}\end{equation*}
% since $\dn(s)A\!\!=\!\!\exp(-\mu s)A\dn(s)$, $\dn(s)B\!\!=\!\!\exp(s)B$, $\forall s\!\!\in\!\!\R$. 
% {\color{red} Andrey:Please write this derivation with details---$>$}
It is noticeable that, in the latter equation, $e_i^{\top}\!\!\!\dn^{\top}\!\!\!(\!\!-\!\!\ln \!\|e_i\|_\dn\!) (P(A\!\!-\!BK_{lin})\!+\!(A\!-\!BK_{lin} )^\top\!\!\!P)\dn(\!\!-\!\!\ln \!\|e_i\|_\dn\!)e_i\!\!<\!\!-\rho$ since \eqref{eq:LMI_new} holds and $\|\dn(\!\!-\!\!\ln \!\|e_i\|_\dn\!)e_i\|_P\!\!=\!\!1$. In addition, $e_i^{\top}\!\!\dn^{\top}\!\!\!(\!\!-\!\!\ln \!\|e_i\|_\dn\!) PB(\hat q_i\!-\!\hat q_0)\!\!\leq\!\!\tfrac{\rho}{2}$ since \eqref{eq:upperq} holds.  Then $\tfrac{d \|e_i\|_{\dn}}{d t}\!\!\leq\!\!-\vartheta$, $\forall i\!\!=\!\!\overline{1,N}$, and the error equation \eqref{eq:exp_error_dy_disturb_non} is globally finite-time stable \cite{polyakov2020generalized}.
Moreover, since $\dn( s)B\!\!=\!\!\exp(s)B$, $\forall s\!\!\in\!\!\R$, $HB\!\!=\!\!-B$, the homogeneous barrier function  
$\phi_i(e_i)\!\!=\!\!H\dn(-\ln \|e_i\|_{\dn})e_i$ yields
\begin{equation}\label{eq:homo_phi_iss_mu-1}\begin{aligned}
\tfrac{d\phi}{dt}
% \!\!=&\diag\left\{\|e_i\|_{\dn}^{-1}\left(\bar\Lambda_i\!\!-\!\!\tfrac{(\hat q_i-\hat q_0)B\phi_i^\top}{|\phi_i|^2}\right)\right\}_{i=1}^N\phi
% ,\\
\!\!=\!\!\diag\left\{\|e_i\|_{\dn}^{-1}\left(\begin{smallmatrix}
    2\gamma_i\!-\!\lambda &  1\\
   \lambda\gamma_i\!-\!\tfrac{(\hat q_i\!-\!\hat q_0)\phi_{i,1}}{|\phi_i|^2}  & \gamma_i\!-\!\lambda\!-\!\tfrac{(\hat q_i\!-\!\hat q_0)\phi_{i,2}}{|\phi_i|^2}
\end{smallmatrix}\right)\right\}_{i=1}^N\!\!\phi
% &\!\!=\!\!g(\phi)
% \!\!+\!\!(I_N\!\!\otimes\!\!H G_\dn G_\dn^{-1})\diag\{\dn(-\ln \|e_i\|_{\dn})\}_{i=1}^N q.
\end{aligned}\end{equation}
with $\phi\!\!=\!\!(\phi_1^\top,\dots,\phi_N^\top)^\top$, 
% $\bar\Lambda_i\!\!=\!\!A\!\!-\!\!\lambda I_2\!\!+\!\!\gamma_i\Gamma$,  
$\gamma_i\!\!=\!\!-\!\tfrac{d \|e_i\|_{\dn}}{dt}\!\!>\!\!0$,
% and $\Gamma\!\!=\!\!G_\dn \!\!+\!\lambda A^\top\!\!\!\!\geq\!\!0$, 
$\forall i\!\!=\!\!\overline{1,N}$. Moreover, the system matrix of the $\phi$-system \eqref{eq:homo_phi_iss_mu-1} is Metzler if
\begin{equation}\label{eq:Metz}
    \lambda\gamma_i\!\!-\!\!\tfrac{(\hat q_i-\hat q_0)\phi_{i,1}}{|\phi_i|^2}\!\!\geq\!\!0, \;\;\forall i\!\!=\!\!\overline{1,N}
\end{equation}
which holds if $\|\hat q_i\!\!-\!\!\hat q_0\|_{L^\infty}\!\!\leq\!\!\tfrac{\lambda\gamma_i|\phi_i|^2}{\phi_{i,1}}$, $\forall i\!\!=\!\!\overline{1,N}$. We notice $\gamma_i\!\!\geq\!\!\vartheta$, $\forall i\!\!=\!\!\overline{1,N}$, 
 $\lambda^{1/2}_{\min}(P^{-1/2}\eta_1\eta_1^\top P^{-1/2})\!\!\leq\!\!\phi_{i,1}\!\!\leq\!\!\lambda^{1/2}_{\max}(P^{-1/2}\eta_1\eta_1^\top P^{-1/2})$, $\lambda_{\min}(P^{-1/2}H^\top HP^{-1/2})\!\!\leq\!\!|\phi_{i}|^2\!\!\leq\!\!\lambda_{\max}(P^{-1/2}H^\top H P^{-1/2})$. Then, \eqref{eq:Metz} holds if 
 $\|\hat q_i\!-\!\hat q_0\|_{L^\infty}\!\!\leq\!\!\tfrac{\lambda\vartheta\lambda_{\min}(P^{-1/2}H^\top HP^{-1/2})}{\lambda^{1/2}_{\max}(P^{-1/2}\eta_1\eta_1^\top P^{-1/2})}$,
as \eqref{eq:upperq} claims. Thus the $\phi$-system \eqref{eq:homo_phi_iss_mu-1} is positive \cite{farina2011positive}, and claim c) is proved. 
\end{proof}
% With the same disturbance defined above, the error equation \eqref{eq:error_closed} becomes
%  \begin{equation}\label{eq:error_closed_lin_disturb}\begin{aligned}
%  	\dot e\!\!=&f_b(e,q)\\
%   \!\!=&(I_N\!\!\otimes\!\!(A\!\!-\!\!BK_{lin}))e\!\!-\!\!(I_N\!\!\otimes\!\!BK_{lin})q_a\!\!+\!\!q_b.
%   \end{aligned}\end{equation}
% where$f_b\!:\!\R^{Nn}\!\!\times\!\!\R^{2Nn}\!\!\to\!\!\R^{Nn}$, $q_a\!\!\in\!\!L^\infty(\R,\R^{Nn})$ is defined in Lemma \ref{lem:unique_vi_disturb}; $q_b\!\!\in\!\!L^\infty(\R,\R^{Nn})$ and $q\!\!\in\!\!L^\infty(\R,\R^{2Nn})$ are defined in \eqref{eq:exp_error_dy_disturb}. 
% \begin{proposition}
%     Let the conditions of Theorem \ref{thm:linear} be satisfied, then the closed-loop error equation \eqref{eq:error_closed_lin_disturb} is ISS with respect to $q\!\!\in\!\!L^\infty(\R,\R^{2Nn})$.
% \end{proposition}
% \begin{proof}
%     Since Theorem \ref{thm:linear} guarantees that the system $\dot e\!\!=\!\!f_b(e,\textbf{0})$ be globally exponentially stable, thus we immediately obtain the claimed property. 
% \end{proof}



% Moreover, taking the disturbance defined above again, the closed-loop error equation \eqref{eq:exp_error_nonover} becomes 
% \begin{equation}\label{eq:exp_error_nonover_disturb}\begin{aligned}
%  	&\dot e\!\!=\!\!f_b(e,q)\!\!=
%     \!\!(I_N\!\!\otimes\!\!A)e\!\!+\!\!q_b\\&
%     \!\!-\!\!\diag\{\!\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!(e\!\!+\!\!q_a)\!\|_{\dn}^{1\!+\!\mu}\!\!BK_{lin}\dn(\!-\!\!\ln\!\!\|\!(\xi_i^\top\!\!\!\!\otimes\!\!I_n)\!(e\!\!+\!\!q_a)\!\|_{\dn})\}_{i=1}^N\!(e\!\!+\!\!q_a),
% \end{aligned} \end{equation}
% where $f_b\!:\!\R^{Nn}\!\!\times\!\!\R^{2Nn}\!\!\to\!\!\R^{Nn}$, $q_a\!\!\in\!\!L^\infty(\R,\R^{Nn})$ is defined in Lemma \ref{lem:unique_vi_disturb}; $q_b\!\!\in\!\!L^\infty(\R,\R^{Nn})$ and $q\!\!\in\!\!L^\infty(\R,\R^{2Nn})$ are defined in \eqref{eq:exp_error_dy_disturb}. 

% \begin{proposition}
%     \textit{Let the conditions of Theorem \ref{thm:finite_nonovershoot} hold, then the closed-loop error equation \eqref{eq:exp_error_nonover_disturb} is ISS with respect to $q\!\!\in\!\!L^\infty\!(\R,\R^{2Nn})$. }
% \end{proposition}
% \begin{proof}
%     Repeating the proof of Proposition \ref{prop:1}, we can obtain that the vector field $f_q\!:\!\R^{Nn}\!\!\times\!\!\R^{2Nn}\!\!\to\!\!\R^{Nn}$ with $f_{q}(e,q)\!\!=\!\!\left(\begin{smallmatrix}
%     f_b(e,q)\\
%     \textbf{0}_{2Nn}
% \end{smallmatrix}\right)$ is homogeneous with respect to the dilation $\left(\begin{smallmatrix}
%     e\\
%     q
% \end{smallmatrix}\right)\!\!\to\!\!\left(
%                                              \begin{smallmatrix}
%                                                \tilde \dn(s) & \mathbf{0}_{Nn\!\times\! 2Nn} \\
%                                                \mathbf{0}_{2Nn\!\times\! Nn} & \tilde\dn_q(s) \\
%                                              \end{smallmatrix}
%                                            \right)
% \left(\begin{smallmatrix}
%     e\\
%     q
% \end{smallmatrix}\right)$, $\forall s\!\!\in\!\!\R$. Using the stability property of $\dot e \!\!=\!\!f_b(e,\textbf{0})$ given in Theorem \ref{thm:finite_nonovershoot}, we complete the proof by recalling Lemma \ref{lem:ISS}.
% \end{proof}



% \newpage
% We let a nominal control input for the homogeneous control system be 
% \begin{equation*}
%  	u_{nom}\!\!=\!\!-\|e\|_{\tilde\dn}^{1+\mu}(I_N \!\!\otimes\!\! K)\!\tdn(-\ln\|e\|_{\tilde\dn})e.
%  \end{equation*}
% With the control $u_{nom}$, the closed-loop error equation is
%   \begin{equation*}\begin{aligned}
%  	\dot e\!\!=&f_{nom}(e)\\
%   \!\!=&(I_N\!\otimes\!A)e\!\!+\!\!(I_N\!\otimes\!B)u_{nom}\\
%    \!\!=&\left(I_N\!\!\otimes\!\!A\!\!-\!\!\|e\|_{\dn}^{1+\mu}(I_N\!\!\otimes\!\!BK)\tdn(-\ln\|e\|_{\tdn})\right)e.
%   % &\!\!=\!\!(I_N\!\otimes\!A)e\!\!+\!\!(I_N\!\otimes\!B)(u\!\!-\!\!u_{norm})\!\!+\!\!(I_N\!\otimes\!B)u_{norm}.
%   \end{aligned}\end{equation*}
% Using the identity $\tilde\dn(s)(I_N\!\otimes\!A)\!\!=\!\!\exp(-\mu s)(I_N\!\otimes\!A)\tilde\dn(s)$ and $\tilde\dn( s)(I_N\!\otimes\!B)\!\!=\!\!\exp(s)(I_N\!\otimes\!B)$. It is easy to show that $f_{nom}(e)$ is $\tdn$-homogeneous of degree $\mu\!\!\in\!\!\R$. 


% Next we show the equivalence between $u$ and $u_{nom}$ provided $\mu$ is sufficiently close to zero. 
% The difference between $u$ and $u_{nom}$ is 
% \begin{equation*}\begin{aligned}
% &u\!\!-\!\!u_{nom}\\
% \!\!=&\|e\|_{\tilde\dn}^{1+\mu}\!\!(I_N\!\!\otimes\!\! K)\\&\!\!\times\!\!\left(I_{Nn}\!\!-\!\!\diag\{\|(\xi_i^\top\!\!\!\otimes\!\! I_n) z\|_{\dn}^{1+\mu}\!\!\dn(-\ln\|(\xi_i^\top\!\!\!\otimes\!\! I_n) z\|_{\dn})\}_{i=1}^N\right)z\\
%  \end{aligned}\end{equation*}
% where $z\!\!=\!\!(z_1^\top,\dots,z_N^\top)^\top\!\!=\!\!\tdn(-\ln\|e\|_{\tdn})e$, and $(\xi_i^\top\!\!\!\otimes\!\! I_n)z\!\!=\!\!z_i$.
% The latter is equivalently written as
% \begin{equation*}\begin{aligned}
% &u\!\!-\!\!u_{nom}\\
% =&\|e\|_{\tilde\dn}^{1+\mu}\!\!(I_N\!\!\otimes\!\! K)\!\!\left(I_{Nn}\!\!-\!\!\diag\{\exp(D_\mu\ln\|(\xi_i^\top\!\!\otimes\!\! I_n) z\|_{\dn})\}_{i=1}^N\right)z,
%  \end{aligned}\end{equation*}
% where $D_\mu\!\!=\!\!\mu\diag\{n\!\!+\!\!1\!\!-\!\!k\}_{k=1}^n$. Let 
% \begin{equation*}\begin{aligned}
% &\sigma(\mu,z)
% \!\!=\!\!(I_N\!\!\otimes\!\! K)\!\!\left(I_{Nn}\!\!-\!\!\diag\{\exp(D_\mu\ln\|(\xi_i^\top\!\!\otimes\!\! I_n) z\|_{\dn})\}_{i=1}^N\right)z.
%  \end{aligned}\end{equation*}
% Denote $\sigma_i$ as the $i_{th}$ line of $\sigma$, then 
% \begin{equation*}\begin{aligned}
% &\tfrac{\partial\sigma_i}{\partial \mu}
% \!\!=\!\!-\!\diag\{n\!\!+\!\!1\!\!-\!\!k\}_{k=1}^n\!\!\exp((D_\mu\!\!+\!\!\epsilon I_n)\ln\| z_i\|_{\dn})\tfrac{\ln\|z_i\|_{\dn}z_i}{\|z_i\|_{\dn}^{\epsilon}},
%  \end{aligned}\end{equation*}
%   where $-\mu n\!\!<\!\!\epsilon\!\!<\!\!1$. The existence of $\epsilon$ is guaranteed by $\mu\!\!\in\!\!(-1/n,0)$. Then matrix $D_\mu\!\!+\!\!\epsilon I_n$ is anti-Hurwitz, which implies 
%   \begin{equation*}\begin{aligned}
% \lim_{\|z_i\|\!\to\!0}\|\exp((D_\mu\!\!+\!\!\epsilon I_n)\ln\| z_i\|_{\dn})\|\!\!=\!\!0.
%  \end{aligned}\end{equation*}
% In addition, 
%   \begin{equation*}\begin{aligned}
%   \left|\tfrac{\ln\|z_i\|_{\dn}z_i}{\|z_i\|_{\dn}^{\epsilon}}\right|\!\!=\!\!\tfrac{\ln\|z_i\|_{\dn}}{\|z_i\|_{\dn}^{\epsilon}}|z_i|\!\!\leq\!\!\tfrac{\ln\|z_i\|_{\dn}}{\|z_i\|_{\dn}^{\epsilon}}|P^{-1/2}|\|z_i\|_P.
%   \end{aligned}\end{equation*}
%   % If $\|z\|\!\!\to\!\!0$, then $\|z\|_{\tilde P}\!\!<1$ and $z_i\!\!\in\!\!B(1)$, thus we have
%   For $\|z_i\|\!\!\to\!\!0$, we have $\|z_i\|_P\!\!<\!\!1$, then   $\|z_i\|_P\!\!\leq\!\!\|z_i\|_\dn^{\lambda_{\min}(G_\dn)}\!\!=\!\!\|z_i\|_\dn$.
%   Then, 
%   \begin{equation*}\begin{aligned}
%   \lim_{\|z_i\|\!\to\!0}\left|\tfrac{\ln\|z_i\|_{\dn}z_i}{\|z_i\|_{\dn}^{\epsilon}}\right|\!\!\leq\!\!
%   \lim_{\|z_i\|\!\to\!0}\tfrac{\ln\|z_i\|_{\dn}}{\|z_i\|_{\dn}^{\epsilon}}|P^{-1/2}|\|z_i\|_\dn\!\!=\!\!
%   \lim_{\|z_i\|\!\to\!0}\tfrac{\ln\|z_i\|_{\dn}}{\|z_i\|_{\dn}^{\epsilon-1}}|P^{-1/2}|\!\!=\!\!0.
%   \end{aligned}\end{equation*}
  
%   Thus we have $\lim_{\|z_i\|\!\to\!0}\tfrac{\partial\sigma_i}{\partial \mu}\!\!=\!\!\textbf{0}$. Since 
% \begin{equation*}\begin{aligned}
% &\tfrac{\partial\sigma}{\partial \mu}
% \!\!=\!\!\left(\begin{array}{ccc}
%      \ldots  \\
%      \tfrac{\partial\sigma_i}{\partial \mu}\\
%      \ldots 
% \end{array}\right),
%  \end{aligned}\end{equation*}
% and $\|z\|\!\!\to\!\!0$ is equivalent to $\|z_i\|\!\!\to\!\!0$, $\forall i\!\!=\!\!\overline{1,N}$. We have $\lim_{\|z\|\!\to\!0}\tfrac{\partial\sigma}{\partial \mu}\!\!=\!\!\textbf{0}$. 
% Therefore, we conclude that the function $\sigma(\mu,z)$ is continuously differentiable on $(-1/n,0)\!\!\times\!\!\R^{Nn}$. 

% Mean-value theorem gives
% \begin{equation*}\begin{aligned}
% \|\sigma(\mu,z)\|_{\tilde P}^2\!\!=\!\!\|\sigma(0,z)\|_{\tilde P}\!\!+\!\!2|\mu|\sigma^\top(\tilde\mu,z)\tilde P\tfrac{\partial\sigma^\top\!\!\!(\tilde\mu,z)}{\partial \tilde\mu}|_{\tilde\mu\!\in\![-|\mu|,|\mu|]}.
%  \end{aligned}\end{equation*}
% Taking into account $\|z\|_{\tilde P}\!\!=\!\!1\!\!\Rightarrow\!\!\|z_i\|_P\!\!\leq\!\!1\!\!\Leftrightarrow\!\!\|z_i\|_\dn\!\!\leq\!\!1$, and $\|\sigma(0,z)\|_{\tilde P}\!\!=\!\!0$, we have $\|\sigma(\mu,z)\|_{\tilde P}^2\!\!\leq\!\!2|\mu|\varsigma$, with 
% \begin{equation*}\begin{aligned}
% \varsigma\!\!:=\!\!\sup_{|\tilde\mu|\!\leq\!|\mu|,\|z\|_{\tilde P}\!=\!1}\left|\sigma^\top\!\!\!(\tilde\mu,z)\tilde P\tfrac{\partial\sigma^\top\!\!\!(\tilde\mu,z)}{\partial \tilde\mu}\right|.
%  \end{aligned}\end{equation*}
% Since $\varsigma\!\!\to\!\!0$ as $\mu\!\!\to\!\!0$, hence $\sigma(\mu,z)\!\!\to\!\!\textbf{0}$ as $\mu\!\!\to\!\!0$ uniformly on $z$ from the unit ball.

% Since
%  \begin{equation*}\begin{aligned}
% u\!\!=&u_{nom}\!\!+\!\!\|e\|_{\tilde\dn}^{1+\mu}\sigma(\mu,z)\\
% =&-\!\!\|e\|_{\tilde\dn}^{1+\mu}\!\!\!\left((I_N \!\!\otimes\!\! K)\tdn(-\ln\|e\|_{\tilde\dn})e\!\!-\!\!\sigma(\mu,z)\right),
%  \end{aligned}\end{equation*}
% where $\sigma\!\!\to\!\!\textbf{0}$ provided $\mu$ is sufficiently close to zero. Thus we conclude that for a $\mu$ sufficiently close to zero, $u\!\!\approx\!\!u_{nom}$.



% We finish the stability by 
% proving that $\|e\|_{\tdn}$ is a Lyapunov candidate of the error equation provided $\mu$ is sufficiently close to zero. It is shown that, for a $\mu$ sufficiently close to $0$, we consider $u$ to be equivalent to $u_{nom}$. Therefore, the stability analysis on the $u_{nom}$ applies to $u$ as well. 
% \begin{equation*}\begin{aligned}
% &\tfrac{d \|e\|_{\tilde\dn}}{d t}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}z^{\top}\!\!\! (I_N\!\otimes\!P)\tilde\dn(-\ln \|e\|_{\tilde\dn})\dot e}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}z^{\top}\!\!\! (I_N\!\otimes\!P)\tilde\dn(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!A\!-\!\|e\|_{\dn}^{1+\mu}(I_N\!\otimes\!BK)\tdn(-\ln\|e\|_{\tdn}))e}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}^{1+\mu}z^{\top}\!\!\! (I_N\!\otimes\!P(A\!-\!BK))z}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}.
% 	\end{aligned}\end{equation*}
% It is clear $\tfrac{d \|e\|_{\tilde\dn}}{d t}\!\!<\!\!0$ provided \eqref{eq:LMI_P} holds. 


 
% where 
% \begin{equation*}\begin{aligned}
% &\|e\|_{\tilde\dn}z^{\top}\!\!\! (I_N\!\otimes\!P)\tilde\dn(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!B)(u\!\!-\!\!u_{norm})\\
% =&z^{\top}\!\!\! (I_N\!\otimes\!PB)(u\!\!-\!\!u_{norm})\\
% %=&\|e\|_{\tilde\dn}^{1+\mu}z^{\top}\!\!(I_N\!\!\otimes\!\! PBK)\sigma(\mu,z)
% \end{aligned}\end{equation*}
% and
% \begin{equation*}\begin{aligned}
% &\|e\|_{\tilde\dn}z^{\top}\!\!\! (I_N\!\otimes\!P)\tilde\dn(-\ln \|e\|_{\tilde\dn})((I_N\!\otimes\!A)e\!\!+\!\!(I_N\!\otimes\!B)u_{norm})\\
% =&\|e\|_{\tilde\dn}^{1+\mu}z^{\top}\!\!\! (I_N\!\otimes\!P(A\!\!-\!\!BK))z
% \end{aligned}\end{equation*}
% Then,
% \begin{equation*}\begin{aligned}
% \tfrac{d \|e\|_{\tilde\dn}}{d t}&=\!\!\tfrac{\|e\|_{\tilde\dn}^{1+\mu}(z^{\top}\!\!\! (I_N\!\otimes\!P(A\!\!-\!\!BK))z\!+\!z^{\top}\!\!\!(I_N\!\otimes\!PB)(u\!-\!u_{norm}))}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\\
% &\leq\!\!\tfrac{\|e\|_{\tilde\dn}^{1+\mu}(z^{\top}\!\!\! (I_N\!\otimes\!P(A\!\!-\!\!BK))z\!+\!|P^{1/2}BK||u\!-\!u_{norm}|)}

% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\\
% 	\end{aligned}\end{equation*}
% Since $|(I_N\!\otimes\!P^{1/2}BK)|$ is fixed, and $\sigma(\mu,z)\!\!\to\!\!\textbf{0}$ as $\mu\!\!\to\!\!0$ uniformly on $z$ from the unit ball. Then, for a sufficiently small $\mu$, there exists a small enough $\rho\!\!>\!\!0$ such that
% \begin{equation*}\begin{aligned}
% \tfrac{d \|e\|_{\tilde\dn}}{d t}
% &\leq\!\!\tfrac{\|e\|_{\tilde\dn}^{1+\mu}(z^{\top}\!\!\! (I_N\!\otimes\!P(A\!\!-\!\!BK))z\!+\!\rho)}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\!\!=\!\!\tfrac{\|e\|_{\tilde\dn}^{1+\mu}z^{\top}\!\!\! (I_N\!\otimes\!(P(A\!\!-\!\!BK)+\rho I_n))z}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\\
% 	\end{aligned}\end{equation*}



 

% The closed-loop error equation is 
% \begin{equation}\label{eq:homo_error_closed}\begin{aligned}
%  	\dot e\!\!=\!\!&f(e)\\
%   \!\!=\!\!&\left(I_N\!\!\otimes\!\!A\!\!-\!\!(I_N\!\!\otimes\!\!BK)\diag\{\|\theta_i\|_{\tilde\dn}^{1+\mu}\dn(-\ln\|\theta_i\|_{\tilde\dn})\}_{i=1}^N\right)e\\
%    \!\!=\!\!&\left(I_N\!\!\otimes\!\!A\right)e\\&-\!\!(I_N\!\!\otimes\!\!BK)\diag\{\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn}^{1+\mu}\!\!\dn(-\ln\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn})\}_{i=1}^Ne.
%   \end{aligned}\end{equation}
% The vector field $f(e)$ is $\tilde\dn$-homogeneous of degree $\mu\!\!\in\!\!\R$ with respect to $e\!\!\to\!\!\tilde\dn(s)e$, $\forall s\!\!\in\!\!\R$. To show this, we have the following calculation. 
% \begin{equation*}\begin{aligned}
% &f(\tilde\dn(s)e)\!\!=\!\!\left(I_N\!\!\otimes\!\!A\right)\tilde\dn(s)e\!\!-\!\!(I_N\!\!\otimes\!\!BK)\\
% &\!\!\times\!\!\diag\{\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)\tilde\dn(s)e\|_{\tilde\dn}^{1+\mu}\!\!\dn(-\ln\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)\tilde\dn(s)e\|_{\tilde\dn})\}_{i=1}^N\tilde\dn(s)e\\
% &\!\!=\!\!\exp(\mu s)\tilde\dn(s)\left(I_N\!\!\otimes\!\!A\right)e\!\!-\!\!(I_N\!\!\otimes\!\!BK)\\
% &\!\!\times\!\!\diag\{\|\tilde\dn(s)(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn}^{1+\mu}\!\!\dn(-\ln\|\tilde\dn(s)(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn})\}_{i=1}^N\tilde\dn(s)e\\
% &\!\!=\!\!\exp(\mu s)\tilde\dn(s)\left(I_N\!\!\otimes\!\!A\right)e\!\!-\!\!\exp(s(1\!\!+\!\!\mu))(I_N\!\!\otimes\!\!BK)\\&\!\!\times\!\!\diag\{\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn}^{1+\mu}\!\!\dn(-\ln\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn})\}_{i=1}^N\tilde\dn(-s)\tilde\dn(s)e\\
% &\!\!=\!\!\exp(\mu s)\tilde\dn(s)\left(I_N\!\!\otimes\!\!A\right)e\!\!-\!\!\exp(\mu s)(I_N\!\!\otimes\!\!\exp(s)BK)\\&\!\!\times\!\!\diag\{\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn}^{1+\mu}\!\!\dn(-\ln\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn})\}_{i=1}^Ne\\
% &\!\!=\!\!\exp(\mu s)\tilde\dn(s)\left(I_N\!\!\otimes\!\!A\right)e\!\!-\!\!\exp(\mu s)\tilde\dn(s)(I_N\!\!\otimes\!\!BK)\\&\!\!\times\!\!\diag\{\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn}^{1+\mu}\!\!\dn(-\ln\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn})\}_{i=1}^Ne\\
% &\Rightarrow f(\tilde\dn(s)e)\!\!=\!\!\exp(\mu s)\tilde\dn(s)f(e).
%   \end{aligned}\end{equation*}

% Let us show  $\|e\|_{\tilde\dn}$ is a Lyapunov function of the closed-loop error equation \eqref{eq:homo_error_closed}. Using the formula $\tilde\dn(s)(I_N\!\otimes\!A)\!\!=\!\!\exp(-\mu s)(I_N\!\otimes\!A)\tilde\dn(s)$ and $\tilde\dn( s)(I_N\!\otimes\!B)\!\!=\!\!\exp(s)(I_N\!\otimes\!B)$, we have the derivative of $\|e\|_{\tilde\dn}$ along \eqref{eq:homo_error_closed},
% \begin{equation*}\begin{aligned}
% &\tfrac{d \|e\|_{\tilde\dn}}{d t}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}z^{\top}\!\!\! (I_N\!\otimes\!P)\tilde\dn(-\ln \|e\|_{\tilde\dn})\dot e}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}z^{\top}\!\!\! (I_N\!\otimes\!P)\tilde\dn(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!A)e}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\\
% &-\!\!\tfrac{\|e\|_{\tilde\dn}z^{\top}\!\!\! (I_N\!\otimes\!P)\tilde\dn(-\ln \|e\|_{\tilde\dn})[(I_N\!\otimes\!BK)\diag\{\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)e\|_{\tilde\dn}^{1+\mu}\dn(-\!\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)e\|_{\tilde\dn})\}_{i=1}^N]e}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\\
% 	\end{aligned}\end{equation*}
%  where $z\!\!=\!\!\tilde\dn(-\ln \|e\|_{\tilde\dn})e$,
% \begin{equation*}\begin{aligned}
% \tilde\dn(-\ln \|e\|_{\tilde\dn})&(I_N\!\otimes\!A)\!\!=\!\! \|e\|^{\mu}_{\tilde\dn}(I_N\!\otimes\!A)\tilde\dn(-\ln \|e\|_{\tilde\dn}),
% \end{aligned}\end{equation*}
% \begin{equation*}\begin{aligned}
% \tilde\dn(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!BK)
% \!\!=\!\!\|e\|_{\tilde\dn}^{-1}(I_N\!\otimes\!BK),
% \end{aligned}\end{equation*}
% \begin{equation*}\begin{aligned}
% &\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)e\|_{\tilde\dn}^{1+\mu}\\
% \!\!=&\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)\tilde\dn(\ln \|e\|_{\tilde\dn})z\|_{\tilde\dn}^{1+\mu}\\
% \!\!=&\|\tilde\dn(\ln \|e\|_{\tilde\dn})(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn}^{1+\mu}\\
% \!\!=& \|e\|_{\tilde\dn}^{1+\mu}\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn}^{1+\mu}\\
% \end{aligned}\end{equation*}
% \begin{equation*}\begin{aligned}
% &\diag\{\dn(-\!\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)e\|_{\tilde\dn})\}_{i=1}^Ne\\
% \!\!=&\diag\{\dn(-\!\ln\|\tilde\dn(\ln \|e\|_{\tilde\dn})(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\}_{i=1}^Ne\\
% \!\!=&\diag\{\dn(-\!\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\}_{i=1}^Nz.
% \end{aligned}\end{equation*}
% In this case,
% \begin{equation*}\begin{aligned}
% &\tilde\dn(-\!\!\ln \!\!\|e\|_{\tilde\dn})(I_N\!\!\otimes\!\!BK)\diag\{\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn}^{1+\mu}\!\dn(-\!\ln\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)e\|_{\tilde\dn})\}e\\
% &=\!\!\|e\|_{\tilde\dn}^{\mu}\!(I_N\!\!\otimes\!\!BK)\diag\{\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)z\|_{\tilde\dn}^{1+\mu}\dn(-\!\ln\|(\tilde{\mathcal{L}}_i\!\!\otimes\!\!I_n)z\|_{\tilde\dn})\}_{i=1}^N z,
% \end{aligned}\end{equation*}
% and
% \begin{equation*}\begin{aligned}
% &\tfrac{d \|e\|_{\tilde\dn}}{d t}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}z^{\top}\!\!\! (I_N\!\otimes\!P)\tilde\dn(-\ln \|e\|_{\tilde\dn})\dot e}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}^\mu z^{\top}\!\!\! (I_N\!\otimes\!P)\left(I_N\!\otimes\!A\!-\!(I_N\!\otimes\!BK)\diag\{\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn}^{1+\mu}\dn(-\!\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\}_{i=1}^N\right)z}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z},\\
% % &=\!\!\tfrac{\|e\|_{\tilde\dn}^\mu z^{\top}\!\!\! (I_N\!\otimes\!P)\left(I_N\!\otimes\!A\!-\!(I_N\!\otimes\!BK)\diag\{\exp(D_\mu\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\}_{i=1}^N\right)z}
% % {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z},
% 	\end{aligned}\end{equation*}
% % where $D_\mu\!\!=\!\!\mu\diag\{n\!\!+\!\!1\!\!-\!\!k\}_{k=1}^n$, and $D_\mu$ is a Hurwitz matrix. 
% the latter can be equivalently written as 
% \begin{equation*}\begin{aligned}
% &\tfrac{d \|e\|_{\tilde\dn}}{d t}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}^\mu z^{\top}\!\!\! (I_N\!\otimes\!P(A\!-\!BK))z}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn}))z}\!\!+\!\!\tfrac{\|e\|_{\tilde\dn}^\mu z^{\top}\!\!\! (I_N\!\otimes\!P)(I_N\!\otimes\!BK)z}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn}))z}\\
% &-\!\!\tfrac{\|e\|_{\tilde\dn}^\mu z^{\top}\!\!\! (I_N\!\otimes\!P)(I_N\!\otimes\!BK)\diag\{\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn}^{1+\mu}\dn(-\!\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\}_{i=1}^Nz}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}^\mu z^{\top}\!\!\! (I_N\!\otimes\!P(A\!-\!BK))z}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn}))z}\!\!+\!\!\tfrac{\|e\|_{\tilde\dn}^\mu z^{\top}\!\!\! (I_N\!\otimes\!PBK)(I_{Nn}\!\!-\!\diag\{\exp(D_\mu\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\}_{i=1}^N)z}
% {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn}))z}\\
% % &=\!\!\tfrac{\|e\|_{\tilde\dn}^\mu z^{\top}\!\!\! (I_N\!\otimes\!P)\left(I_N\!\otimes\!A\!-\!(I_N\!\otimes\!BK)\diag\{\exp(D_\mu\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\}_{i=1}^N\right)z}
% % {z^{\top}\!\!\!(I_N\!\otimes\!PG_{\dn})z},
% 	\end{aligned}\end{equation*}
%  where $D_\mu\!\!=\!\!\mu\diag\{n\!\!+\!\!1\!\!-\!\!k\}_{k=1}^n$, and $D_\mu$ is a Hurwitz matrix since $\mu\!\!<\!\!0$. We would like to have $\|(I_{Nn}\!\!-\!\diag\{\exp(D_\mu\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\}_{i=1}^N)z\|\!\!\to\!\!0$ if $\mu$ is sufficiently close to zero. 
 
% Let the function $\sigma:\R\!\!\times\!\!\R^{Nn}\!\!\rightarrow\!\!\R^{Nn}$, 
% \begin{equation*}\begin{aligned}
% &\sigma(\mu,(\tilde{\mathcal{L}}\!\otimes\!I_n)z)\\
% &\!\!=\!\!(I_{Nn}\!\!-\!\diag\{\exp(D_\mu\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\}_{i=1}^N)z\\
% &\!\!=\!\!(I_{Nn}\!\!-\!\diag\{\exp(D_\mu\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\}_{i=1}^N)(\tilde{\mathcal{L}}^{-1}\!\otimes\!I_n)(\tilde{\mathcal{L}}\!\otimes\!I_n)z.
% \end{aligned}\end{equation*}
% \begin{equation*}\begin{aligned}
% &\frac{\partial\sigma_i}{\partial \mu}\\
% \!\!=&\!\!-\diag\{n\!\!+\!\!1\!\!-\!\!k\}_{k=1}^n\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn}\exp(D_\mu\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})z\\
% \!\!=&\!\!-\diag\{n\!\!+\!\!1\!\!-\!\!k\}_{k=1}^n\exp(D_\mu\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn})\\
% &\times\!\!(\tilde{\mathcal{L}}^{-1}\!\otimes\!I_n)(\tilde{\mathcal{L}}\!\otimes\!I_n)z\ln\|(\tilde{\mathcal{L}}_i\!\otimes\!I_n)z\|_{\tilde\dn}.
% \end{aligned}\end{equation*}













% Then
% \begin{equation*}\begin{aligned}
% \tfrac{d \|e\|_{\tilde\dn}}{d t}&\!
% \!=\!\!\tfrac{\|e\|_{\tilde\dn}^{1+\mu}e^{\top}\!\!\tilde\dn^{\top}\!\!\!(-\ln \|e\|_{\tilde\dn}) [I_N\!\otimes\!P(A\!-\!BK)]\tilde\dn(-\ln \|e\|_{\tilde\dn})e}
% {e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!PG_{\dn})\tilde\dn(-\ln \|e\|_{\tilde\dn})e}\\
% &\!
% \!=\!\!\tfrac{\|e\|_{\tilde\dn}^{1+\mu}e^{\top}\!\!\tilde\dn^{\top}\!\!\!(-\ln \|e\|_{\tilde\dn}) [I_N\!\otimes\!(P(A\!-\!BK)\!+\!(A\!-\!BK)^\top P)]\tilde\dn(-\ln \|e\|_{\tilde\dn})e}
% {e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!(PG_{\dn}\!+\!G_{\dn}P))\tilde\dn(-\ln \|e\|_{\tilde\dn})e}\!\!<\!\!0
% 	\end{aligned}\end{equation*}
% since $\eqref{eq:LMI_P}$ is fulfilled. 

% Therefore, we conclude that the error equation \eqref{eq:homo_error_closed} is finite-time stable at $e\!\!=\!\!\textbf{0}$ with $\mu\!\!\in\!\![-1,0)$. 





















%\newpage
% {\it{Part 1: Stability proof}}

% The control \eqref{eq:homo_control} is equivalently written as 
% \begin{equation*}\begin{aligned}
%  	\sum\nolimits_{j=0}^N\!\!w_{ij}u_i\!\!-\!\!\sum\nolimits_{j=0}^N\!\! w_{ij}u_j\!\!&=\!\!\|e\|_{\tilde\dn}^{1+\mu} K\dn(-\ln\|e\|_{\tilde\dn})\sum\nolimits_{j=0}^N w_{ij}(x_j\!\!-\!\!x_i)\\
%   \sum\nolimits_{j=0}^N\!\!w_{ij}u_i\!\!-\!\!\sum\nolimits_{j=1}^N\!\! w_{ij}u_j\!\!&=\!\!\|e\|_{\tilde\dn}^{1+\mu}K\dn(-\ln\|e\|_{\tilde\dn})\sum\nolimits_{j=0}^N\!\! w_{ij}(x_j\!\!-\!\!x_i)\\
%   \TL_i u\!\!&=\!\!-\|e\|_{\tilde\dn}^{1+\mu}(\TL_i\!\otimes\!K\dn(-\ln\|e\|_{\tilde\dn}))e\\
%   \TL u\!\!&=\!\!-\|e\|_{\tilde\dn}^{1+\mu}(\TL\!\otimes\! K\dn(-\ln\|e\|_{\tilde\dn}))e\\
%   \TL u\!\!&=\!\!-\|e\|_{\tilde\dn}^{1+\mu}(\TL\!\otimes\! K)\tilde\dn(-\ln\|e\|_{\tilde\dn})e.
%  \end{aligned}\end{equation*}
% Since $\TL$ has full rank, then the solution of the latter equation:
% \begin{equation*}\begin{aligned}
%  	 u\!\!&=\!\!-\|e\|_{\tilde\dn}^{1+\mu}(I_N\!\otimes\! K)\tilde\dn(-\ln\|e\|_{\tilde\dn})e.
%  \end{aligned}\end{equation*}
% The closed-loop error equation is 
% \begin{equation}\label{eq:homo_error_closed}\begin{aligned}
%  	\dot e&\!\!=\!\!f(e)\\
%   &\!\!=\!\![I_N\!\otimes\!A\!\!-\!\!\|e\|_{\tilde\dn}^{1+\mu}\!\!(I_N\!\otimes\!BK)\tilde\dn(-\ln\|e\|_{\tilde\dn})]e.
%   \end{aligned}\end{equation}
% The vector field $f(e)$ is $\tilde\dn$-homogeneous of degree $\mu\!\!\in\!\!\R$ with respect to $e\!\!\to\!\!\tilde\dn(s)e$, $\forall s\!\!\in\!\!\R$. 
% %$\mu\!\!\in\!\![-1,1/n]$ with respect to $e\!\!\to\!\!\tilde\dn(s)e$. 

% Let us show  $\|e\|_{\tilde\dn}$ is a Lyapunov function of the closed-loop error equation \eqref{eq:homo_error_closed}. Using the formula $\tilde\dn(s)(I_N\!\otimes\!A)\!\!=\!\!\exp(-\mu s)(I_N\!\otimes\!A)\tilde\dn(s)$ and $\tilde\dn( s)(I_N\!\otimes\!B)\!\!=\!\!\exp(s)(I_N\!\otimes\!B)$, we have the derivative of $\|e\|_{\tilde\dn}$ along \eqref{eq:homo_error_closed},
% \begin{equation*}\begin{aligned}
% &\tfrac{d \|e\|_{\tilde\dn}}{d t}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e\|_{\tilde\dn}) (I_N\!\otimes\!P)\tilde\dn(-\ln \|e\|_{\tilde\dn})\dot e}
% {e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!PG_{\dn})\tilde\dn(-\ln \|e\|_{\tilde\dn})e}\\
% &=\!\!\tfrac{\|e\|_{\tilde\dn}e^{\top}\!\tilde\dn^{\top}\!\!\!(-\ln \|e\|_{\tilde\dn}) (I_N\!\otimes\!P)\tilde\dn(-\ln \|e\|_{\tilde\dn})[I_N\!\otimes\!A\!-\!\|e\|_{\tilde\dn}^{1+\mu}\!\!(I_N\!\otimes\!BK)\tilde\dn(-\!\ln\|e\|_{\tilde\dn})]e}
% {e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!PG_{\dn})\tilde\dn(-\ln \|e\|_{\tilde\dn})e}\\
% 	\end{aligned}\end{equation*}
%  where
% \begin{equation*}\begin{aligned}
% \tilde\dn(-\ln \|e\|_{\tilde\dn})&(I_N\!\otimes\!A)\!\!=\!\! \|e\|^{\mu}_{\tilde\dn}(I_N\!\otimes\!A)\tilde\dn(-\ln \|e\|_{\tilde\dn}),
% \end{aligned}\end{equation*}
% \begin{equation*}\begin{aligned}
% \tilde\dn(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!BK)
% \!\!=\!\!\|e\|_{\tilde\dn}^{-1}(I_N\!\otimes\!BK).
% \end{aligned}\end{equation*}
% Then
% \begin{equation*}\begin{aligned}
% \tfrac{d \|e\|_{\tilde\dn}}{d t}&\!
% \!=\!\!\tfrac{\|e\|_{\tilde\dn}^{1+\mu}e^{\top}\!\!\tilde\dn^{\top}\!\!\!(-\ln \|e\|_{\tilde\dn}) [I_N\!\otimes\!P(A\!-\!BK)]\tilde\dn(-\ln \|e\|_{\tilde\dn})e}
% {e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!PG_{\dn})\tilde\dn(-\ln \|e\|_{\tilde\dn})e}\\
% &\!
% \!=\!\!\tfrac{\|e\|_{\tilde\dn}^{1+\mu}e^{\top}\!\!\tilde\dn^{\top}\!\!\!(-\ln \|e\|_{\tilde\dn}) [I_N\!\otimes\!(P(A\!-\!BK)\!+\!(A\!-\!BK)^\top P)]\tilde\dn(-\ln \|e\|_{\tilde\dn})e}
% {e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e\|_{\tilde\dn})(I_N\!\otimes\!(PG_{\dn}\!+\!G_{\dn}P))\tilde\dn(-\ln \|e\|_{\tilde\dn})e}\!\!<\!\!0
% 	\end{aligned}\end{equation*}
% since $\eqref{eq:LMI_P}$ is fulfilled. 

% Therefore, we conclude that the error equation \eqref{eq:homo_error_closed} is finite-time stable at $e\!\!=\!\!\textbf{0}$ with $\mu\!\!\in\!\![-1,0)$. 






















































































% % FIXED-TIME LIKE CONTROL
% For any given $T\!\!>\!\!0$, the homogeneous controller 
% \begin{equation}\label{eq:homo_control}
%  	u_i\!\!=\!\!\frac{1}{\sum_{j=0}^Nw_{ij}}\sum\nolimits_{j=0}^N w_{ij}\left[\hat K\dn(-\ln\|e/r\|_{\tilde\dn})(x_j\!\!-\!\!x_i)\!\!+\!\!u_j\right],\;i\!\!=\!\!\overline{1,N}.
%  \end{equation}
% where $\tilde \dn\!\!=\!\!I_N\!\otimes\!\dn$, $\dn$ is generated by $G_\dn\!\!=\!\!\diag\{n\!\!-\!\!k\!\!+\!\!1\}_{k\!=\!1}^n$, $\hat K\!\!=\!\!K\dn(\hat s)$ with
% \begin{equation*}
% \hat s\!\!\geq\!\!\ln\max\left\{\tfrac{1}{\rho T},1\right\}, \;\;r\!\!>\!\!0, \;\rho\!\!>\!\!0,
% \end{equation*}
% stabilize the error equation \eqref{eq:error_dy} at $e\!\!=\!\!\textbf{0}$ in a finite time and 
% \begin{equation*}
% \|e(0)\|\!\!\leq\!\!r, \Rightarrow e(t,e(0))\!\!=\!\!\textbf{0}, \forall t\!\!\geq\!\!T.
% \end{equation*}

% \begin{equation*}\begin{aligned}
%  	\sum\nolimits_{j=0}^Nw_{ij}u_i\!\!-\!\!\sum\nolimits_{j=0}^N w_{ij}u_j\!\!&=\!\!\hat K\dn(-\ln\|e/r\|_{\tilde\dn})\sum\nolimits_{j=0}^N w_{ij}(x_j\!\!-\!\!x_i),\;i\!\!=\!\!\overline{1,N}\\
%   \sum\nolimits_{j=0}^Nw_{ij}u_i\!\!-\!\!\sum\nolimits_{j=1}^N w_{ij}u_j\!\!&=\!\!\hat K\dn(-\ln\|e/r\|_{\tilde\dn})\sum\nolimits_{j=1}^N w_{ij}(x_j\!\!-\!\!x_i)\\
%   \TL_i u\!\!&=\!\!-(\TL_i\!\otimes\!\hat K\dn(-\ln\|e/r\|_{\tilde\dn}))e\\
%   \TL u\!\!&=\!\!-(\TL\!\otimes\!\hat K\dn(-\ln\|e/r\|_{\tilde\dn}))e\\
%   \TL u\!\!&=\!\!-(\TL\!\otimes\! K)\tilde\dn(\hat s)\tilde\dn(-\ln\|e/r\|_{\tilde\dn})e\\
%  \end{aligned}\end{equation*}
% Since $\TL$ has full rank, then the solution of the latter equation:
% \begin{equation*}\begin{aligned}
%  	 u\!\!&=\!\!-(I_N\!\otimes\! K)\tilde\dn(\hat s)\tilde\dn(-\ln\|e/r\|_{\tilde\dn})e.
%  \end{aligned}\end{equation*}
% The closed-loop error equation is 
% \begin{equation}\label{eq:homo_error_closed}\begin{aligned}
%  	\dot e&\!\!=\!\!(I_N\!\otimes\!A)e\!\!-\!\!(I_N\!\otimes\!B)u\\
%   &\!\!=\!\![I_N\!\otimes\!A\!\!-\!\!(I_N\!\otimes\!BK)\tilde\dn(\hat s)\tilde\dn(-\ln\|e/r\|_{\tilde\dn})]e.
%   \end{aligned}\end{equation}

% Let us show  $\|e/r\|_{\tilde\dn}$ is a Lyapunov function of the closed-loop error equation \eqref{eq:homo_error_closed}. Using the formula $\tilde\dn(s)(I_N\!\otimes\!A)\!\!=\!\!\exp(s)(I_N\!\otimes\!A)\tilde\dn(s)$ and $\tilde\dn(s)(I_N\!\otimes\!B)\!\!=\!\!\exp(s)(I_N\!\otimes\!B)$, we have 
% \begin{equation*}\begin{aligned}
% &\tfrac{d \|e/r\|_{\tilde\dn}}{d t}\!\\&=\!\!\tfrac{\|e/r\|_{\tilde\dn}(e/r)^{\top}\!\tilde\dn^{\top}\!(-\ln \|e/r\|_{\tilde\dn})\tilde\dn^{\top}\!(\hat s) (I_N\!\otimes\!P)\tilde\dn\!(\hat s)\tilde\dn(-\ln \|e/r\|_{\tilde\dn})(\dot e/r)}
% {(e/r)^{\top}\!\tilde\dn^{\top}\!(-\ln \|e/r\|_{\tilde\dn})\tilde\dn^{\top}\!(\hat s)(I_N\!\otimes\!PG_{\dn})\tilde\dn\!(\hat s)\tilde\dn(-\ln \|e/r\|_{\tilde\dn})(e/r)}\\
% \!&=\!\!\tfrac{\|e/r\|_{\tilde\dn}e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e/r\|_{\tilde\dn}) \tilde\dn^{\top}\!(\hat s) (I_N\!\otimes\!P)\tilde\dn\!(\hat s)\tilde\dn(-\ln \|e/r\|_{\tilde\dn})\dot e}
% {e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e/r\|_{\tilde\dn})\tilde\dn^{\top}\!(\hat s)(I_N\!\otimes\!PG_{\dn})\tilde\dn\!(\hat s)\tilde\dn(-\ln \|e/r\|_{\tilde\dn})e}\\
% \!&=\!\!\tfrac{\|e/r\|_{\tilde\dn}e^{\top}\!\!\tilde\dn^{\top}\!\!\!(-\ln \|e/r\|_{\tilde\dn}) \tilde\dn^{\top}\!\!\!(\hat s)(I_N\!\otimes\!P)\tilde\dn\!(\hat s)\tilde\dn(-\ln \|e/r\|_{\tilde\dn})[I_N\!\otimes\!A\!-\!(I_N\!\otimes\!BK)\tilde\dn(\hat s)\tilde\dn(-\!\ln\|e/r\|_{\tilde\dn})]e}
% {e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e/r\|_{\tilde\dn})\tilde\dn^{\top}\!(\hat s)(I_N\!\otimes\!PG_{\dn})\tilde\dn\!(\hat s)\tilde\dn(-\ln \|e/r\|_{\tilde\dn})e}\\
% 	\end{aligned}\end{equation*}
%  where
% \begin{equation*}\begin{aligned}
%   \tilde\dn\!(\hat s)\tilde\dn(-\ln \|e/r\|_{\tilde\dn})&(I_N\!\otimes\!A)\!\!=\!\! \|e/r\|^{-1}_{\tilde\dn}\tilde\dn\!(\hat s)(I_N\!\otimes\!A)\tilde\dn(-\ln \|e/r\|_{\tilde\dn})\\&\!\!=\!\!\exp(\hat s)\|e/r\|^{-1}_{\tilde\dn}(I_N\!\otimes\!A)\tilde\dn\!(\hat s)\tilde\dn(-\ln \|e/r\|_{\tilde\dn}),
% \end{aligned}\end{equation*}
% \begin{equation*}\begin{aligned}
% \tilde\dn\!(\hat s)\tilde\dn(-\ln &\|e/r\|_{\tilde\dn})(I_N\!\otimes\!BK)\tilde\dn(\hat s)\tilde\dn(-\ln\|e/r\|_{\tilde\dn})\\
% &=\exp(\hat s)\|e/r\|_{\tilde\dn}^{-1}(I_N\!\otimes\!BK)\tilde\dn(\hat s)\tilde\dn(-\ln\|e/r\|_{\tilde\dn}).
% \end{aligned}\end{equation*}
% Then
% \begin{equation*}\begin{aligned}
% \tfrac{d \|e/r\|_{\tilde\dn}}{d t}&\!
% \!=\!\!\tfrac{\exp(\hat s)e^{\top}\!\!\tilde\dn^{\top}\!\!\!(-\ln \|e/r\|_{\tilde\dn}) \tilde\dn^{\top}\!\!\!(\hat s)[I_N\!\otimes\!P(A\!-\!BK)]\tilde\dn\!(\hat s)\tilde\dn(-\ln \|e/r\|_{\tilde\dn})}
% {e^{\top}\!\tilde\dn^{\top}\!(-\ln \|e/r\|_{\tilde\dn})\tilde\dn^{\top}\!(\hat s)(I_N\!\otimes\!PG_{\dn})\tilde\dn\!(\hat s)\tilde\dn(-\ln \|e/r\|_{\tilde\dn})e}\\
% &\!\!\leq\!\!-\exp(\hat s)\rho\!\!\leq\!\!-\max\{1/T,\rho\}\!\!\leq\!\!-1/T.
% 	\end{aligned}\end{equation*}
% where $\rho\!\!=\!\!-\lambda_{\max}(Q^{-\frac{1}{2}}ZQ^{-\frac{1}{2}})\!\!>\!\!0$, with
% \begin{equation*}
% \begin{aligned}
%     Q\!\!=\!\!PG_\dn\!\!+\!\!G_\dn P\!\!\succ\!\!0, \;\;Z\!\!=\!\!P(A\!\!-\!\!BK)\!\!+\!\!(A\!\!-\!\!BK)P\!\!\prec\!\!0.
% \end{aligned}
% \end{equation*}





% In this section, a generalized homogeneous consensus protocol is designed by upgrading the classical linear one. The main result shows that such an upgrade is feasible  if there is a supervisor who monitors the MAS and can broadcast a scalar signal $u_g$ simultaneously to all followers. With this homogeneous control scheme, the ISS and the global finite-time stability of the consensus errors can be guaranteed by tuning the homogeneity degree.

% %\textcolor{blue}{
% %Before the main result, the generator of the dilation $G_{\dn}$ is given.}
% %Given $\mu\neq 0$ and let $G_{\dn}\in \R^{n\times n}$ be an anti-Hurwitz matrix satisfying the identities
% %\begin{equation}\label{eq:G_d}
% %	AG_{\dn}=(\mu I_n+G_{\dn})A, \quad G_{\dn}B=B.
% %	\end{equation}
% %In \cite{Zimenk_etal2020:TAC} it is shown that such a matrix $G_{\dn}$ can always be found provided that $A$ is nilpotent.

	
% 	Let the pair $(G_0,Y_0) \in \R^{n\times n} \times \R^{m\times n}$ be a solution of the following algebraic equations
% \begin{equation}\label{eq:G_0}
%   AG_0-G_0A+BY_0=A,\;\; G_0B=\mathbf{0},
% \end{equation}
% such that the matrix $G_0-I_n$ is invertible. Then the matrix $G_{\dn}=\mu G_0+I_n$ is anti-Hurwitz for any $\mu\leq 1/n$ with \begin{equation}\label{eq:homoAB}
% A_{0}G_{\dn}=(\mu I_n+G_{\dn})A_0,\;\; G_{\dn}B=B,
% \end{equation}
% matrix
% $
% 	A_0=A+BK_0
% $
% is 	 nilpotent,  where
% \begin{equation}\label{eq:K0}
% 	K_0=Y_0(G_0-I_n)^{-1}.
% \end{equation}
% \begin{remark}
% According to \cite{Polyakov2020:Book,Zimenk_etal2020:TAC}, if Assumption \ref{assum1} is fulfilled, i.e., the pair $(A,B)$ is controllable, then $(A_0, B)$ is controllable, and such a solution of \eqref{eq:G_0} always exists. In addition, $K_0=\mathbf{0}$ if matrix $A$ is already nilpotent.
% \end{remark}

% %Based on that, we let
% %\begin{equation*}
% %	u_d=u_1+K_0\xi_1,\quad K_0=Y_0(G_0-I_n)^{-1}.
% %	\end{equation*}
% %Denote $\bar k=\|K_0\|$, combining Assumption \ref{assum_bound}, we have
% %\begin{equation*}\begin{aligned}
% %  \|u_d\|\leq \|u_1\|+\|K_0\|\|\xi_1\|\leq \bar u_1+\bar k\bar \xi_1,
% %\end{aligned}\end{equation*}
% %and $u_d\in L^{\infty}(\mathbb{R},\mathbb{R}^m)$.
		

% \begin{thm}\label{thm1}
% 	%{\color{red}Andrey: please do peresent the claim of theorem as follows.}
% 	Let Assumption \ref{assum1}, \ref{assum:bound}, \ref{assum:supervisor} hold.
% Let $(X,Y)\in \R^{n\times n}\times \R^{m\times n}$ be a solution of the linear matrix inequality
% 	\begin{equation}\label{eq:LMI_hom}
% 		\begin{array}{l}
%    	    	I_{N}\otimes (A_0X+XA^{\top}_0)+\tilde{\mathcal{L}}\otimes BY+(\tilde{\mathcal{L}}\otimes BY)^{\top}\prec 0,\\
% 	   	    G_{\dn}X+XG_{\dn}^{\top} \succ0,  \;\; X\succ 0,
% 	 \end{array}
% 	\end{equation}
% where $A_0=A+BK_0$, $K_0$ is given in \eqref{eq:K0}, $\tilde{\mathcal{L}}$ is defined in \eqref{eq:Ltiled}, $G_{\dn}=\mu G_0+I_n$ is anti-Hurwitz with $G_0$ satisfying \eqref{eq:G_0}, $\mu\leq1/n$.
% Let $\|e\|_{\tilde \dn}$ be the canonical homogeneous norm induced by the norm
% $\|e\|_{P}=\sqrt{e^{\top}Pe},~P=I_{N}\otimes X^{-1}$.
% Then the error equation
% \eqref{eq:error_dynamics} with $u_g= \|e\|_{\tilde \dn}$, $K=YX^{-1}$ and
% \begin{equation}\label{eq:control}
% u_{i}=K_0\xi_i+u_g^{\mu+1} K\dn(-\ln u_g) \sum\nolimits^N_{j=0}w_{ij}(\xi_j-\xi_i),\;\; i=\overline{1,N}
% \end{equation}
% has the following properties:
% \begin{itemize}
% \item
% $\tilde \dn$-homogeneous of degree $\mu\in[-1,1/n]$ if $\xi_0=\dot\xi_0=\mathbf{0}$,
% %$e\rightarrow \tilde {\mathbf{d}}(s)e$ and $u_d\rightarrow \diag\{\mathrm{exp}(1+\mu)s\}u_d,~s\in \mathbb{R}$, where
%  $\tilde \dn(s)={\rm exp}(sG_{\tilde\dn})=I_{N}\otimes \dn(s)$
% and $ \dn(s)={\rm exp}(sG_{\dn})$;
% % are  linear dilations in $\R^{(N-1)\times n}$ and $\R^n$, respectively;
% \item
% globally asymptotically stable for $\xi_0=\dot\xi_0=\mathbf{0}$;
% \item
% ISS with respect to $q=(\xi_0,\dot
% \xi_0)$ for $\mu\in(-1,1/n]$;
% \item
% globally uniformly finite-time stable if $\mu=-1$, $f_0$ satisfies \eqref{eq:dyleader_iden}, $\|A_0\xi_0-\dot \xi_0\|_{L^{\infty}}\leq U_{\max}$, and
% \begin{equation}\label{umax}
%   U_{\max}<U_0:=\tfrac{\lambda_{\min}(\Pi_1)}{2\sqrt{Nn\lambda_{\max}(X^{-1})}},
% \end{equation}
% with
% \begin{equation*}\begin{aligned}
% \Pi_1\!&=\!-P^{\frac{1}{2}}(I_{N}\otimes (A_0X\!+\!XA_0^{\top}\!)\!+\! \tilde{\mathcal{L}}\!\otimes\! BY\!+\!(\tilde{\mathcal{L}}\!\otimes\! BY)^{\top}) P^{\frac{1}{2}}.
% \end{aligned}\end{equation*}
% The settling time is estimated as
% \begin{equation}\label{eq:settling_time}
% T(e(0))\leq \tfrac{\|e(0)\|_{\tilde \dn}\lambda_{\max}(\Pi_2)}{2(U_0-U_{\max})\sqrt{Nn\lambda_{\max}(X^{-1})}},
% \end{equation}
% where
% $\Pi_2\!=\!P^{\frac{1}{2}}(I_{N}\otimes\!(\!G_{\dn}X\!+\!XG_{\dn}^{\top}\!) )P^{\frac{1}{2}}.$
% \end{itemize}
% 	\end{thm}

% The detailed proof is provided in Appendix B.

% The following corollary  follows from the asymptotic stability and $\tilde \dn$-homogeneity of the error equation
% \eqref{eq:error_dynamics} for $\xi_0\!=\!\dot\xi_0\!=\!\mathbf{0}$.
% \begin{Coro}
% 	Let all conditions of Theorem \ref{thm1} be fulfilled. Let $\xi_0\!=\!\dot\xi_0\!=\!\mathbf{0}$. Then the error equation \eqref{eq:error_dynamics} is
% 	\begin{itemize}
% 		\item globally uniformly finite-time stable for $\mu<0$;
% 		\item globally uniformly asymptotically stable for $\mu=0$;
% 		\item globally uniformly nearly fixed-time stable for $\mu>0$.
% 	\end{itemize}
% \end{Coro}

% It is worth stressing that for $\mu\!=\!-1$ the control protocol \eqref{eq:control} is a high-order sliding mode algorithm having a discontinuity at $e=\mathbf{0}$ (i.e., when the consensus is reached).  The use of the input $u_g$ in the consensus protocol allows us to avoid large (infinite) gains in the transient phase (before reaching consensus). This reduces overshoots \cite{Polyakov2020:Book} and numerical chatterings which are typical for sliding mode algorithms \cite{acary2010implicit}.
% Moreover, for $\mu\!=\!-1$ the control inputs of all controlled agents  are bounded.
% \begin{Coro}\label{coro:u_bound}
% Let $u=[u_1^{\top}, \ldots, u_N^{\top}]^{\top}$, if $\mu=-1$ then we have
% \begin{equation}\label{eq:umax}
% \|u\|_2\leq \|K_0\|_2\|\xi\|_2+
% \sqrt{\lambda_{\max}\left((P^{-1/2})^{\top}\tilde K^{\top}\tilde K P^{-1/2}\right)},
% %\lambda_{\max}(\tilde{\mathcal{L}}^{\top}\tilde{\mathcal{L}}\otimes (X^{-1})^{\frac{1}{2}}Y^{\top}Y(X^{-1})^{\frac{1}{2}}).
% \end{equation}
% where $\xi=[\xi_1^{\top},\dots,\xi_N^{\top}]^{\top}$, $ \tilde K=\tilde{\mathcal{L}}\otimes K$.
% \end{Coro}

% \begin{proof}
% Recall \eqref{eq:control}, for $\mu=-1$, we have
% $
%   u=\tilde K_0\xi+\tilde K \tilde \dn(-\ln \|e\|_{\tilde\dn})e,
% $
% with $\tilde K_0=I_N\otimes K_0$.
% Then,
% \begin{equation*}
% \begin{aligned}
% \|u\|_2&\leq\|\tilde K_0\xi\|_2+\|\tilde K \tilde \dn(-\ln \|e\|_{\tilde\dn})e\|_2\\
% &\leq\|K_0\|_2\|\xi\|_2+\sqrt{e^{\top}\tilde \dn^{\top}(-\ln \|e\|_{\tilde\dn}) \tilde K^{\top}\tilde K \tilde \dn(-\ln \|e\|_{\tilde\dn})e}\\
% &\leq\|K_0\|_2\|\xi\|_2+\sqrt{\lambda_{\max} \left((P^{-1/2})^{\top}\tilde K^{\top}\tilde K P^{-1/2}\right)}\times\\&\sqrt{e^{\top}\tilde \dn^{\top}(-\ln \|e\|_{\tilde\dn}) P \tilde \dn(-\ln \|e\|_{\tilde\dn})e}.
% \end{aligned}
% \end{equation*}
% By the definition of the canonical homogeneous norm we have $e^{\top}\tilde \dn^{\top}(-\ln \|e\|_{\tilde\dn}) P \tilde \dn(-\ln \|e\|_{\tilde\dn})e=1$. Hence, the inequality \eqref{eq:umax} can be obtained.
% \end{proof}

% \begin{remark}
% If $K_0=\mathbf{0}$ (i.e., matrix A is nilpotent)  and $\mu=-1$ then $u$ is globally uniformly bounded (see the formula \eqref{eq:umax}).
% \end{remark}

% In some cases, a MAS is already regulated by some linear control protocol.
% The following corollary presents an algorithm for its upgrading  to a locally homogeneous one.
% \begin{Coro}\label{coro:localhomo}
%  Let all conditions of Theorem \ref{thm1} be fulfilled. %Let all control parameters be specified from.
%  %
% % The pair
% % $(X,Y)\in \R^{n\times n} \times \R^{m\times n}$ is a solution of \eqref{eq:LMI_hom}, where $G_{\dn}=\mu G_0+I_n$ is anti-Hurwitz, $G_0$ is given in \eqref{eq:G_0}, $\mu\leq1/n$. Canonical homogeneous norm $\|e\|_{\tilde \dn}$ is induced by
% %$\|e\|_{P},~P=I_{N}\otimes X^{-1}\succ 0$.
%  %If
% % \[
% % G_{\dn}X+XG_{\dn}^{\top} \succ0,
% % \]
% % for anti-Hurwitz $G_{\dn}$, $K_0$ satisfying \eqref{eq:K0}, and some $\mu\leq1/n$,
% Then the error equation
% \eqref{eq:error_dynamics} with $u_g= \|e\|_{\tilde \dn}$, $K=YX^{-1}$ and
% %Then all conclusions of Theorem \ref{thm1} remain valid for the control protocol
%  \begin{equation}\label{eq:switchcontrol}
%  	u_{i}\!=\!K_0\xi_i\!+\!\left\{
%  	\begin{array}{ll}
%  		\!\!\!K\sum^N_{j=0}w_{ij}(\xi_j\!-\!\xi_i)  & u_g\!>\! 1,\\
%  	\!\!\!u_g^{\mu+1} \!K\dn(-\ln u_g) \sum^N_{j=0}w_{ij}(\xi_j\!-\!\xi_i) 	 & u_g\!\leq\! 1,
%  	\end{array}
%  \right.
%  \end{equation}
% $i=\overline{1,N}$, has the following properties:
%   \begin{itemize}
%   %\item
% %$\tilde \dn$-homogeneous of degree $\mu\in[-1,1/n]$ for $u_g\!\leq\! 1$;
% % $\tilde \dn(s)={\rm exp}(sG_{\tilde\dn})=I_{N}\otimes \dn(s)$
% %and $ \dn(s)={\rm exp}(sG_{\dn})$;
%   \item
% globally asymptotically stable for $\xi_0=\dot\xi_0=\mathbf{0}$;
% \item
% ISS with respect to $q=(\xi_0,\dot
% \xi_0)$ for $\mu\in(-1,1/n]$;
% \item
% globally uniformly finite-time stable if $\mu\!=\!-1$, $f_0$ satisfies \eqref{eq:dyleader_iden}, $\|A_0\xi_0-\dot \xi_0\|_{L^{\infty}}\!\leq\! U_{\max}$, where $U_{\max}$ is given in \eqref{umax}.
% \end{itemize}
% \end{Coro}

% \begin{proof}
% With the control \eqref{eq:switchcontrol}, the closed-loop error equation $\dot e\!=\!f(e,\xi_0,\dot \xi_0)$ coincides with a $\tilde\dn$-homogeneous system of degree
% $\mu\!=\!0$ (linear system) for $u_g\!\geq\!1$ and a $\tilde\dn$-homogeneous system of degree
% $\mu\in[-1,1/n]$ for $u_g\leq 1$.

% Since the mapping $u_g\mapsto\dn(-\ln u_g)$ is uniformly continuous, and for $u_g=1$
% we have   $\|e\|_{\tilde\dn}=e^{\top} Pe=1$ and $$u_g^{\mu+1} K\dn(-\ln u_g) \sum\nolimits^N_{j=0}w_{ij}(\xi_j-\xi_i)=K\sum\nolimits^N_{j=0}w_{ij}(\xi_j-\xi_i),$$
% then  the locally homogeneous control \eqref{eq:switchcontrol} is continuous. Let us consider the  candidate Lyapunov  function $e\mapsto V(e)$ as
% \[V(e)=\left\{
% \begin{array}{cc}
% 	\!\!\!e^{\top} Pe  & e^{\top} Pe > 1,\\
% 	\!\!\!\|e\|_{\tilde \dn}	 & e^{\top} Pe\leq 1.
% \end{array}
% \right.
% 	\]
% Since the function $V$ is locally Lipschitz continuous  on $\R^n\backslash\{\mathbf{0}\}$ then combining the constructions of Lemma \ref{lem:lin_cont} and Theorem \ref{thm1}  we can complete the proof.
% \end{proof}

% The possible fragility  of the proposed scheme is related to the use of a supervisor, which is
%  considered as an external object with respect to MAS. The existence of a robust communication channel for broadcasting of the supervisor's signal $u_g$ seems to be a rather restrictive assumption in some cases. That is why it is important to investigate the robustness of the proposed control
%  scheme with respect to losses and/or aperiodic sampling of  the supervisor's control signal $u_g$.

% %\begin{Coro}\label{coro_discret}
% %	Let $t_0=0<t_1<t_2\dots$ be an arbitrary sequence of time instances such that $t_k\to +\infty$ as $k\to +\infty$.
% %	Let the control protocol be defined by Theorem \ref{thm1} and
% %	$$
% %	u_g(t)=\|e(t_k)\|_{\tilde \dn}, \;\; t\in [t_k, t_{k+1}).
% %	$$
% %	Then the error equation \eqref{eq:error_dynamics}  is
% %	\begin{itemize}
% %		\item
% %		globally asymptotically stable for  $\xi_0=\dot \xi_0=\mathbf{0}$;
% %		\item
% %		ISS with respect to $q=(\xi_0, \dot \xi_0)$ for $\mu\in(-1, 1/n]$;
% %		\item
% %		globally uniformly asymptotically stable if $\mu\!=\!-1$, $f_0$ satisfies \eqref{eq:dyleader_iden}, $\|A_0\xi_0-\dot \xi_0\|_{L^{\infty}}\!\leq\! U_{\max}$, where $U_{\max}$ is as \eqref{umax}.
% %%\item ISS with respect to $q=(\xi_0, \dot \xi_0)$
% %%if $\mu\!=\!-1$, $f_0$ satisfies \eqref{eq:dyleader_iden}, $\|A_0\xi_0-\dot \xi_0\|_{L^{\infty}}\!\leq\! U_{\max}$, where $U_{\max}$ is given in \eqref{umax}.
% %	\end{itemize}	
% %	\end{Coro}
% %
% %\begin{proof}	
% %For $t\in [t_k,t_{k+1})$,
% %	let us consider the function $e(t)\mapsto V_k(e(t))$ defined as follows
% %	$$
% %	V_k(e(t))=e^{\top}(t) \tilde \dn^{\top}(-\ln \|e(t_k)\|_{\tilde \dn})P \tilde \dn(-\ln \|e(t_k)\|_{\tilde \dn}) e(t).
% %	$$
% %	Notice that  $V_k(e(t))=1$ for $t: \|e(t)\|_{\tilde \dn}=\|e(t_k)\|_{\tilde\dn}$.
% %	The time derivative of $V_k$ along $\dot e=f(e, \xi_0, \dot\xi_0)$ satisfies the inequality
% %	$$
% %	\dot V_k(e(t))\leq -\lambda_{\min}(\Pi_1) \|e(t_k)\|_{\tilde\dn}^{\mu} V_k+\tfrac{C\sqrt{V_k}}{\|e(t_k)\|_{\tilde\dn}}\|A_0\xi_0-\dot \xi_0\|_{L^{\infty}}
% %	$$
% %	 for $t\in [t_k,t_{k+1})$, where $C=2\sqrt{Nn\lambda_{\max}(X^{-1})}$.	
% % For $\xi_0\!=\dot \xi_0=\!\mathbf{0},~\mu\in(-1, 1/n]$ or for  $\mu\!=\!-1,~\|A_0\xi_0-\dot \xi_0\|_{L^{\infty}}\!\leq\! U_{\max}$ we derive  $\dot V_k(e(t))<0$ for  $t: \|e(t)\|_{\tilde \dn}=\|e(t_k)\|_{\tilde\dn}$.
% %	 The latter means $V_k(e(t_{k+1}))<1$ and  $\|e(t_{k+1})\|_{\tilde \dn}<\|e(t_k)\|_{\tilde \dn}$.
% %   Let us show that the monotone sequence $\|e(t_k)\|_{\tilde\dn}$ converges to zero as $k\to +\infty$. 	
% % Suppose the contrary, i.e., there exists $q_*>0$ such that $\|e(t_k)\|_{\tilde \dn}\to q_*$ as $k\to +\infty$.
% % Let us consider the function $e\mapsto V_*(e)$  defined as
% %	$$
% %V_*(e)=e^{\top} \tilde \dn^{\top}(-\ln q_*)P\tilde\dn(-\ln q_*) e.
% %$$
% %Notice that $V_*(e(t_k))\to 1$ as $\|e(t_k)\|_{\tilde \dn}\to q_*$.
% %Denoting $\delta_i=u_i-K_0\xi_i-q_*^{\mu+1} K\dn(-\ln q_*) \sum^N_{j=0}w_{ij}(\xi_j-\xi_i)$, $i=\overline{1,N}$ we
% %derive
% %$$\dot V_*\!\leq\! -\lambda_{\min}(\Pi_1) q_*^{\mu} V_*\!+\!\tfrac{C \sqrt{V_*}}{q_*}(\|A_0\xi_0\!-\!\dot \xi_0\|_{L^{\infty}}\!+\!\max\nolimits_{i= \overline{1,N}} \!\|\delta_i\|_{L^{\infty}}).$$
% %Since
% %$\|\delta_i\|_{L_\infty}$ converges to zero as $k\to +\infty$ and $V_*(e(t_k))\to 1$ as $k\to +\infty$  then
% % there exists $k_*\geq 1$  and $c_*>0$ such that
% %$\dot V_*(e(t))\leq -c_*$ for all $t\geq t_{k_*}$. The latter means that  $V_*(e(t))\to 0$ as $t\to +\infty$.
% %Based on the obtained estimates, the ISS with respect to $q=(\xi_0, \dot \xi_0)$ can be proven using the ISS Lyapunov function technique \cite{sontag1996new}.
% %\end{proof}

% \begin{Coro}\label{coro_discret}
% 	Let $t_0=0<t_1<t_2\dots$ be an arbitrary sequence of time instances such that $t_k\to +\infty$ as $k\to +\infty$.
% 	Let the control protocol be defined by Theorem \ref{thm1} and
% 	$$
% 	u_g(t)=\|e(t_k)\|_{\tilde \dn}, \;\; t\in [t_k, t_{k+1}).
% 	$$
% 	Then the error equation \eqref{eq:error_dynamics}  is
% 	\begin{itemize}
% 		\item
% 		globally asymptotically stable for  $\xi_0=\dot \xi_0=\mathbf{0}$;
% 		\item
% 		ISS with respect to $q=(\xi_0, \dot \xi_0)$ for $\mu\in[-1, 1/n]$.
% 	\end{itemize}	
% 	\end{Coro}

% \begin{proof}	
% For $t\in [t_k,t_{k+1})$,
% 	let us consider the function $e(t)\mapsto V_k(e(t))$ defined as follows
% 	$$
% 	V_k(e(t))=e^{\top}(t) \tilde \dn^{\top}(-\ln \|e(t_k)\|_{\tilde \dn})P \tilde \dn(-\ln \|e(t_k)\|_{\tilde \dn}) e(t).
% 	$$
% 	Notice that  $V_k(e(t))=1$ for $t: \|e(t)\|_{\tilde \dn}=\|e(t_k)\|_{\tilde\dn}$.
% 	The time derivative of $V_k$ along error equation \eqref{eq:error_dynamics} with $\xi_0=\dot \xi_0=\mathbf{0}$ satisfies the inequality
% 	$$
% 	\dot V_k(e(t))\leq -\lambda_{\min}(\Pi_1) \|e(t_k)\|_{\tilde\dn}^{\mu} V_k,
% 	$$
% 	 for $t\in [t_k,t_{k+1})$.	
%  %For $\xi_0\!=\dot \xi_0=\!\mathbf{0},~\mu\in(-1, 1/n]$ or for  $\mu\!=\!-1,~\|A_0\xi_0-\dot \xi_0\|_{L^{\infty}}\!\leq\! U_{\max}$ we derive  $\dot V_k(e(t))<0$ for  $t: \|e(t)\|_{\tilde \dn}=\|e(t_k)\|_{\tilde\dn}$.
% 	 The latter means $V_k(e(t_{k+1}))<1$ and  $\|e(t_{k+1})\|_{\tilde \dn}<\|e(t_k)\|_{\tilde \dn}$.
%    Let us show that the monotone sequence $\|e(t_k)\|_{\tilde\dn}$ converges to zero as $k\to +\infty$. 	
%  Suppose the contrary, i.e., there exists $q_*>0$ such that $\|e(t_k)\|_{\tilde \dn}\to q_*$ as $k\to +\infty$.
%  Let us consider the function $e\mapsto V_*(e)$  defined as
% 	$$
% V_*(e)=e^{\top} \tilde \dn^{\top}(-\ln q_*)P\tilde\dn(-\ln q_*) e.
% $$
% Notice that $V_*(e(t_k))\to 1$ as $\|e(t_k)\|_{\tilde \dn}\to q_*$.
% Denoting $\delta_i=u_i-K_0\xi_i-q_*^{\mu+1} K\dn(-\ln q_*) \sum^N_{j=0}w_{ij}(\xi_j-\xi_i)$, $i=\overline{1,N}$ we
% derive
% $$\dot V_*\!\leq\! -\lambda_{\min}(\Pi_1) q_*^{\mu} V_*\!+\!\tfrac{2\sqrt{NV_*\lambda_{\max}(B^\top X^{-1}B)}}{q_*}\max\nolimits_{i= \overline{1,N}} \!\|\delta_i(t)\|_{2}.$$
% Since
% $\sup_{t\in[t_k,t_{k+1})}\|\delta_i(t)\|_{2}$ converges to zero as $k\to +\infty$ and $V_*(e(t_k))\to 1$ as $k\to +\infty$  then
%  there exists $k_*\geq 1$  and $c_*>0$ such that
% $\dot V_*(e(t))\leq -c_*$ for all $t\geq t_{k_*}$. The latter means that  $V_*(e(t))\to 0$ as $t\to +\infty$.
% Based on the obtained estimates, the ISS with respect to $q=(\xi_0, \dot \xi_0)$ can be proven using the ISS Lyapunov function technique \cite{sontag1996new}.
% \end{proof}

% \begin{remark}
% Corollary \ref{coro_discret} has no restriction (like a dwell time) to the sampling period  $t_{k+1}-t_k$. So, the consensus error with the presented consensus protocol would remain asymptotically stable and robust in the case of sampled broadcasting of the supervisor's signal.  Even in the worst case,
% when the signal $u_g$ is lost (i.e., $u_g=const$ for all $t\geq t_*$, $t_*$ is the moment $u_g$ is lost), the system will be simply governed by a linear consensus protocol. In other words, the system  will not crash  if the supervisor's signal will be damaged, sampled, or completely lost. Therefore, the presence of the supervisor does not increase the fragility of the MAS in comparison with the case of the classical linear consensus protocol.
% % Since here the consensus error $e$ only has ISS/asymptotic stability, and the sampled transmitted signal $u_g$ decreases independent from the sampling period. It means, in any one sampling period, the ISS/asymptotic stability of $e$ can always be guaranteed no matter the sampling period is long or short, i.e., this kind of sampled transmission of $u_g$ is aperiodic. However, if we want to make the consensus error $e$ finite-time stable with a settling time $t^*$, we are supposed to assign as many samplings instants $t_k$ as we can with $t\rightarrow t^*$. Anyway, this additionally justifies a practical feasibility of the proposed technique.
% \end{remark}


% %The proven corollary shows that a sampling in the transmission of  the signal $u_g$ does not destroy the stability and robustness of the system. It just effects the convergence rate. \textcolor{blue}{A larger sampling period will lead slower convergence.} This additionally justifies a practical feasibility of the proposed technique.



==> Revised_paper_0119/data/V_Simulation.tex <==

\section{Simulation Results}\label{SR}

The simulation is given under a scenario as Fig. \ref{fig:scenario}, in which a Multi-Robot System (MRS), comprised of one leader (robot 0) and three followers (robot $\overline{1,3}$).
The robots are omnidirectional and modeled on the point of mass subjecting to the following dynamics, with their motion in the X- and Y-coordinates considered separately,
\begin{equation}\label{eq:MRS}\begin{aligned}
\begin{array}{ll}
     \dot X_i(t)\!\!=\!\!AX_i(t)\!\!+\!\!Bu_{X_i}(t)\!\!+\!\!Bq_{X_i}(t),  \\
     \dot Y_i(t)\!\!=\!\!AY_i(t)\!\!+\!\!Bu_{Y_i}(t)\!\!+\!\!Bq_{Y_i}(t),
\end{array}\;\;
    A\!\!=\!\!\left(\begin{smallmatrix}
    0 & 1\\
    0 & 0
\end{smallmatrix}\right),\;\; B\!\!=\!\!\left(\begin{smallmatrix}
    0 \\
    1
\end{smallmatrix}\right),\;\; i\!\!=\!\!\overline{0,3}.
\end{aligned}\end{equation}
where $X_i\!\!=\!\!(X_{i,1},X_{i,2})^\top\!\!\!\!\in\!\!\R^2$, $Y_i\!\!=\!\!(Y_{i,1},Y_{i,2})^\top\!\!\!\!\in\!\!\R^2$, $(X_{i,1},Y_{i,1})$ represents the position of robot $i$; $X_{i,2}$ and $Y_{i,2}$ represent the velocity of robot $i$ along X- and Y-coordinate, respectively; $u_{X_i}\!\!\in\!\!\R$ and $u_{Y_i}\!\!\in\!\!\R$ are the control input of robot $i$ with $u_{X_0}\!\!=\!\!u_{Y_0}\!\!=\!\!0$; $q_{X_i},q_{Y_i}\!\!\in\!\!\R$ represents some matched disturbance.


% \begin{figure}[htbp]
%   \centering
%   % Requires \usepackage{graphicx}
%   \includegraphics[width=3cm]{topology.pdf}\\
%   \caption{The graph of the MRS.}\label{fig:top}
% \end{figure}

\subsection{Finite-time Non-overshooting Consensus}\label{Sim:non-dis}

In MRS \eqref{eq:MRS}, we let $q_{X_i}\!\!=\!\!q_{Y_i}\!\!=\!\!0$. The leader moves on the smooth barrier surface with a constant velocity, and the followers aim to achieve consensus with the leader. During this process, the followers must be guaranteed a safe move, \textit{i.e.,} followers must keep themself behind the leader in X-coordinate. To this end,
  we aim to design some proper $u_{X_i}$ and $u_{Y_i}$, $i\!\!=\!\!\overline{1,3}$ such that the finite-time leader-following consensus is achieved without overshoots in X-coordinate, \textit{i.e.,} let  $e_X\!\!=\!\!(e_{X_1}^\top,e_{X_2}^\top,e_{X_3}^\top)^\top$, $e_{X_i}\!\!=\!\!X_i\!\!-\!\!X_0$, $e_Y\!\!=\!\!(e_{Y_1}^\top,e_{Y_2}^\top,e_{Y_3}^\top)^\top$, $e_{Y_i}\!\!=\!\!Y_i\!\!-\!\!Y_0$,
  $e_{X}$ and $e_{Y}$  be globally finite-time stable, and for $e_{X}(0)\!\!\in\!\!\Omega\!\!\subset\!\!\Sigma\!\!=\!\!\{e_X\!\!\in\!\!\R^{6}\!:\!(I_3\!\otimes\!\eta_1^\top)e_X\!\!\leq\!\!{0}\}$, $e_{X}(t)\!\!\in\!\!\Omega$, $\forall t\!\!\in\!\!\R_+$, $\eta_1\!\!=\!\!(1,0)^\top$.
 % Through this design, followers realize an accelerated and safe following in the transient phase even without collision-avoidance settings.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.45\linewidth]{scenario.pdf}\quad
%     \includegraphics[width=0.3\linewidth]{topology.pdf}
%     \caption{The diagram of the MRS with the specified initial position $(X_{i,1}(0),Y_{i,1}(0))$, $i\!\!=\!\!\overline{0,3}$ and the communication topology.}
%     \label{fig:scenario}
% \end{figure}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{.5\linewidth}
        \centering
        \includegraphics[width=\linewidth]{scenario.pdf}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{.48\linewidth}
        \centering
        \includegraphics[width=.7\linewidth]{topology.pdf}
        \caption{}
    \end{subfigure}
    \caption{The diagram of (a) the MRS with specified initial position $(X_{i,1}(0),Y_{i,1}(0))$, $i\!\!=\!\!\overline{0,3}$; and (b) communication topology.}
    \label{fig:scenario}
\end{figure}

Let $w_{ij}\!\!=\!\!1$ for $(i,j)\!\!\in\!\!\mathcal{E}$.
% , we have
% \begin{equation*}
%     \TL\!\!=\!\!\left(\begin{array}{ccc}
%          2 & 0 & -1  \\
%          -1 & 2 & 0\\
%          0 & -1 & 1
%     \end{array}\right)
% \end{equation*}
% as \eqref{eq:TL} defines, which is inveritable.
Let $v_i$ be defined in \eqref{eq:def_vi} with $x_i\!\!=\!\!X_i$, $i\!\!=\!\!\overline{0,3}$ and $x_i\!\!=\!\!Y_i$, $i\!\!=\!\!\overline{0,3}$, using Theorem \ref{thm:state_con}, one has the solution $v_X\!\!=\!\!e_X$, $v_X\!\!=\!\!(v_{X_1}^\top,v_{X_2}^\top,v_{X_3}^\top)^\top\!\!\!\in\!\!\R^{6}$ and $v_Y\!\!=\!\!e_Y$, $v_Y\!\!=\!\!(v_{Y_1}^\top,v_{Y_2}^\top,v_{Y_3}^\top)^\top\!\!\!\in\!\!\R^{6}$, respectively. Let $u_{X_i}$ take form of the finite-time non-overshooting consensus control \eqref{eq:homo_control_nonover}, then
\begin{equation}\label{eq:nonover_MRS}
    u_{X_i}\!\!=\!\!-\|v_{X_i}\|_{\dn}^{1+\mu}K_{lin}\dn(-\ln\|v_{X_i}\|_{\dn})v_{X_i},\;\;v_{X_i}\!\!=\!\!e_{X_i},\;\;i\!\!=\!\!\overline{1,3}.
\end{equation}
Let $u_{Y_i}$ take form of the finite-time consensus control \eqref{eq:homo_control}, then
\begin{equation}\label{eq:consensus_MRS}
    u_{Y_i}\!\!=\!\!-\|v_{Y_i}\|_{\dn}^{1+\mu}K\dn(-\ln\|v_{Y_i}\|_{\dn})v_{Y_i},\;\;v_{Y_i}\!\!=\!\!e_{Y_i},\;\;i\!\!=\!\!\overline{1,3}.
\end{equation}

For the controller \eqref{eq:nonover_MRS}, let $\lambda\!\!=\!\!1$, according to equation \eqref{eq:lin_control}, one has $K_{lin}\!\!=\!\!(\lambda^2,2\lambda)\!\!=\!\!(1,2)$.
Let $\mu\!\!=\!\!-0.2$, then
$G_{\dn}\!\!=\!\!\diag\{1.2,1\}$. YALMIP gives the solution of \eqref{eq:LMI_P} as follows,
\begin{equation*}
    P\!\!=\!\!\left(\begin{smallmatrix}
        0.0020 & 0.0005\\
        0.0005 & 0.0012\\
    \end{smallmatrix}\right).
\end{equation*}
Based on the above parameters, the real-time value of $\|e_{X_i}\|_\dn$ in \eqref{eq:nonover_MRS} is provided by a online solution of
$\|\dn(-\ln\|e_{X_i}\|_\dn)e_{X_i}\|_P\!\!=\!\!1$
using the ``HCS Toolbox for MATLAB'' available in \cite{polyakov_hcs_toolbox}.

For the controller \eqref{eq:consensus_MRS}, let $\mu\!\!=\!\!-0.2$, thus
$G_{\dn}\!\!=\!\!\diag\{1.2,1\}$. YALMIP gives the solution of \eqref{eq:LMI_P_U} as follows,
\begin{equation*}
    X\!\!=\!\!\left(\begin{smallmatrix}
        0.8281 & -0.3107\\
        -0.3107 & 0.9377
    \end{smallmatrix}\right),\quad Y\!\!=\!\!\left(\begin{smallmatrix}
        0.7502 & 0.5000\\
    \end{smallmatrix}\right),
\end{equation*}
immediately we have
\begin{equation*}
P\!\!=\!\!X^{-1}\!\!\!=\!\!\left(\begin{smallmatrix}
        1.3791 & 0.4569\\
        0.4569 & 1.2178
    \end{smallmatrix}\right),\quad
    K\!\!=\!\!YX^{-1}\!\!\!=\!\!\left(\begin{smallmatrix}
1.2630 & 0.9517
\end{smallmatrix}\right).
\end{equation*}
 Similarly, the real-time value of $\|e_{Y_i}\|_\dn$ in \eqref{eq:consensus_MRS} is provided by the online solution of
  $\|\dn(-\ln\|e_{Y_i}\|_\dn)e_{Y_i}\|_P\!\!=\!\!1$.


Let the initial position of the MRS be Fig. \ref{fig:scenario} gives, and the initial velocity $(X_{0,2}(0),Y_{0,2}(0))\!\!=\!\!(0[{\mathrm{m}}/{\mathrm{s}}],1[{\mathrm{m}}/{\mathrm{s}}])$, $(X_{i,2}(0),Y_{i,2}(0))\!\!=\!\!(1[{\mathrm{m}}/{\mathrm{s}}],1[{\mathrm{m}}/{\mathrm{s}}])$, $i\!\!=\!\!\overline{1,3}$. The implicit Euler method is employed to solve the closed-loop dynamics equation \eqref{eq:MRS}, \eqref{eq:nonover_MRS}, \eqref{eq:consensus_MRS} on MATLAB. The performance of non-overshooting finite-time consensus is shown in Fig. \ref{fig:homo_consensus}.
%, where the settling time $T\!\!\approx\!\!7.0[{\rm s}]$.
% The homogeneous cone $\Omega_{\dn}\!\!=\!\!\{e_X\!\!\in\!\!\R^{6}:\diag\{H\dn(-\ln \|e_{X,i}\|_{\dn})\}_{i=1}^3e_X\!\!\geq\!\!{0}\}$, $H\!\!=\!\!\left(\begin{smallmatrix}
%     -1 & 0\\
%     -\lambda & -1
% \end{smallmatrix}\right)$ is depicted as Fig. \ref{fig:cone}. As a comparison, the corresponding linear cone by letting $\dn\!\!=\!\!\exp(I_2)$ is depicted as well.
\begin{figure}[htbp]
    \centering
    \includegraphics[width=0.9\linewidth]{mu=-2.pdf}
    \caption{The finite-time non-overshooting leader-following consensus with the homogeneous controller \eqref{eq:nonover_MRS}, \eqref{eq:consensus_MRS}.}
    \label{fig:homo_consensus}
\end{figure}

% In the X-coordinate, a comparison trajectory of $e_{X_i,1}$, $i\!\!=\!\!\overline{1,3}$ is presented in Fig. \ref{fig:error_lin} and Fig. \ref{fig:error_log} by employing the homogeneous controller \eqref{eq:nonover_MRS} and the linear controller (\textit{i.e.,} the homogeneous controller \eqref{eq:nonover_MRS} with $\mu\!\!=\!\!0$). Indeed, these two figures plot the same variables while in different coordinates (linear and logarithm, respectively), and illustrate different features of variable convergence: Fig. \ref{fig:error_lin} shows the non-overshooting performance; Fig. \ref{fig:error_log} confirms the finite-time (with the homogeneous controller) and the exponential (with the linear controller) convergence, in which the finite-time convergence lasts for $3.5[\rm{s}]$.
% We also plot the robots' position in X-coordinate in the transient phase ($0[\rm{s}]$-$3.5[\rm{s}]$) to further illustrate our homogeneous result, which is shown in Fig. \ref{fig:trans_state}. In this figure, the non-overshooting performance for followers in the X-coordinate direction move is confirmed.
% In addition, the time evolution of the velocity along the X-coordinate for robot $i\!\!=\!\!\overline{0,3}$ is shown as Fig. \ref{fig:Xi2}.



% /linear cone for $e_{X_i}$, $i\!\!=\!\!\overline{1,3}$ is depicted in Fig. \ref{fig:cone}, the region surrounded by the red lines is the linear cone, while the yellow region is the homogeneous cone.
% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{error_lin.pdf}
%     \caption{The non-overshooting trajectory of (a) $e_{X_1,1}$, (b) $e_{X_2,1}$, and (c) $e_{X_3,1}$ with the homogeneous controller \eqref{eq:nonover_MRS} and its linear counterpart.}
%     \label{fig:error_lin}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{error_log.pdf}
%     \caption{The convergence trajectory of (a) $e_{X_1,1}$, (b) $e_{X_2,1}$, and (c) $e_{X_3,1}$ with the homogeneous controller \eqref{eq:nonover_MRS} and its linear counterpart.}
%     \label{fig:error_log}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{trans_state.pdf}
%     \caption{The transient evolution of $X_{i,1}$ with the non-overshooting homogeneous controller \eqref{eq:nonover_MRS}.}
%     \label{fig:trans_state}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{trans_state_X2.pdf}
%     \caption{The transient evolution of $X_{i,2}$ with the non-overshooting homogeneous controller \eqref{eq:nonover_MRS}.}
%     \label{fig:Xi2}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\linewidth]{CONE.pdf}
%     \caption{The linear cone (the region surrounded by the red lines) and the homogeneous cone (the yellow region) of $e_{X_i}$, $i\!\!=\!\!\overline{1,3}$.}
%     \label{fig:cone}
% \end{figure}




% For the Y-coordinate, the comparison trajectory of $e_{Y_i,1}$, $i\!\!=\!\!\overline{1,3}$ is presented in Fig. \ref{fig:error_lin_Y} and Fig. \ref{fig:error_log_Y}. These figures illustrate a finite-time stabilization with a settling time $4[\rm{s}]$
% by employing the homogeneous controller \eqref{eq:consensus_MRS}, and an asymptotic stabilization using the linear controller (\textit{i.e.,} the homogeneous controller \eqref{eq:consensus_MRS} with $\mu\!\!=\!\!0$). Moreover, the time evolution of $Y_{i,1}$, $i\!\!=\!\!\overline{0,3}$ and $Y_{i,2}$, $i\!\!=\!\!\overline{0,3}$ in the transient phase are depicted as Fig. \ref{fig:Yi1} and Fig. \ref{fig:Yi2}, respectively.


% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.8\linewidth]{error_lin_Y.pdf}
%     \caption{The convergence trajectory of (a) $e_{Y_1,1}$, (b) $e_{Y_2,1}$, and (c) $e_{Y_3,1}$ with the homogeneous controller \eqref{eq:consensus_MRS} and its linear counterpart.}
%     \label{fig:error_lin_Y}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{error_log_Y.pdf}
%     \caption{The convergence trajectory of (a) $e_{Y_1,1}$, (b) $e_{Y_2,1}$, and (c) $e_{Y_3,1}$ with the homogeneous controller \eqref{eq:consensus_MRS} and its linear counterpart.}
%     \label{fig:error_log_Y}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{trans_state_Y1.pdf}
%     \caption{The transient evolution of $Y_{i,1}$ with the  homogeneous finite-time controller \eqref{eq:consensus_MRS}.}
%     \label{fig:Yi1}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{trans_state_Y2.pdf}
%     \caption{The transient evolution of $Y_{i,2}$ with the  homogeneous finite-time controller \eqref{eq:consensus_MRS}.}
%     \label{fig:Yi2}
% \end{figure}

\subsection{Robust Non-overshooting Finite-time Consensus}


Let the matched disturbances of MRS \eqref{eq:MRS} be defined as below:
% as below:
% \begin{equation}\label{eq:MRS_disturb}\begin{aligned}
% \begin{array}{ll}
%      \dot X_i(t)\!\!=\!\!AX_i(t)\!\!+\!\!Bu_{X_i}(t)\!\!+\!\!B\hat q_{X_i}(t),  \\
%      \dot Y_i(t)\!\!=\!\!AY_i(t)\!\!+\!\!Bu_{Y_i}(t)\!\!+\!\!B\hat q_{Y_i}(t),
% \end{array}
%     \;\;i\!\!=\!\!\overline{0,3}
% \end{aligned}\end{equation}
%where
$\hat q_{X_0}\!\!\!=\!\!0$, $\hat q_{X_i}\!\!\in\!\!\R$ is uniformly
distributed in the interval $(-0.540, 0.540)$, $(-0.444, 0.444)$ and $(-0.462, 0.462)$ for $i\!\!=\!\!1$, $i\!\!=\!\!2$ and $i\!\!=\!\!3$, respectively;
and $\hat q_{Y_i}\!\!\in\!\!\R$ is
distributed in the interval $(-0.030,0.030)$, $(-0.428, 0.428)$, $(-0.533, 0.533)$ and $(-0.441, 0.441)$ for $i\!\!=\!\!0$, $i\!\!=\!\!1$, $i\!\!=\!\!2$ and $i\!\!=\!\!3$, respectively.

Let $\mu\!\!=\!\!-1$. Let the initial conditions be the same with Section \ref{Sim:non-dis}. The homogeneous controller \eqref{eq:nonover_MRS} and \eqref{eq:consensus_MRS} regulate the followers to reach the leader in a finite time without overshoots. As a comparison,  the linear controller (by letting $\mu\!\!=\!\!0$ for \eqref{eq:nonover_MRS} and \eqref{eq:consensus_MRS}) cannot ensure a safe movement for the MAS. This comparative performance is shown in Fig. \ref{fig:ISS}.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{mu=-1.pdf}\\
%     \includegraphics[width=0.9\linewidth]{mu=0.pdf}
%     \caption{The trajectory of the MRS with the homogeneous controller \eqref{eq:nonover_MRS} in the presence of the disturbance.}
%     \label{fig:ISSconsensus}
% \end{figure}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{mu=-1.pdf}
        \caption{}
    \end{subfigure}
    \hfill
    \begin{subfigure}{\linewidth}
        \centering
        \includegraphics[width=0.9\linewidth]{mu=0.pdf}
        \caption{}
    \end{subfigure}
    \caption{The trajectory of the MRS considering disturbance by employing the (a) homogeneous control protocol with $\mu\!\!=\!\!-1$; and (b) linear control protocol.}
    \label{fig:ISS}
\end{figure}
% In this section, we show that the proposed controller \eqref{eq:nonover_MRS} offers improved robustness (in the sense of ISS) compared to its linear counterparts, which are obtained by setting
% $\mu\!\!=\!\!0$ in \eqref{eq:nonover_MRS}. This improved robustness is observed with respect to the transmission noise and the model uncertainty.

% We let each component of the transmitted data $X_i$, $Y_i$, $v_{X_i}$ and  $v_{Y_i}$, $i\!\!=\!\!\overline{0,N}$ be disturbed by Gaussian noise $\mathcal{N}(0,0.1^2)$.
% The disturbed dynamic is presented as
% \begin{equation}\label{eq:MRS_disturb}\begin{aligned}
%     &\dot X_i(t)\!\!=\!\!AX_i(t)\!\!+\!\!Bu_{X_i}(t)\!\!+\!\!(0,q_{X_i}(t))^\top,\\
%    & \dot Y_i(t)\!\!=\!\!AY_i(t)\!\!+\!\!Bu_{Y_i}(t)\!\!+\!\!(0,q_{Y_i}(t))^\top,\;\;i\!\!=\!\!\overline{0,3}
% \end{aligned}\end{equation}
% where $q_{X_i}(t)\!\!\in\!\!\R$ is uniformly
% distributed random numbers within the intervals $(-0.040, 0.040)$, $(-0.150, 0.150)$, $(-0.148, 0.148)$ and $(-0.154, 0.154)$ for $i\!\!=\!\!0$, $i\!\!=\!\!1$, $i\!\!=\!\!2$ and $i\!\!=\!\!3$, respectively;
% and $q_{Y_i}(t)\!\!\in\!\!\R$ is uniformly
% distributed within the intervals $(-0.038,0.038)$, $(-0.170, 0.170)$, $(-0.168, 0.168)$ and $(-0.164, 0.164)$ for $i\!\!=\!\!0$, $i\!\!=\!\!1$, $i\!\!=\!\!2$ and $i\!\!=\!\!3$, respectively.

% Let $\psi_{X_i}(t)\!\!=\!\!|e_{X_i}(t)|$ for $t\!\!\geq\!\!0$, $i\!\!=\!\!\overline{1,3}$, whose evolution is depicted as Fig. \ref{fig:error_log_X_rob}. Using the same control parameters and the initial conditions as the undisturbed simulation, the homogeneous controller \eqref{eq:nonover_MRS} regulates the consensus error to a smaller neighborhood of the origin compared to its linear counterpart.

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{error_log_X_rob.pdf}
%     \caption{The trajectory of (a) $\psi_{X_1}$, (b) $\psi_{X_2}$, and (c) $\psi_{X_3}$ with the homogeneous controller \eqref{eq:nonover_MRS} and its linear counterpart in the presence of the transmission noise and the model uncertainty.}
%     \label{fig:error_log_X_rob}
% \end{figure}

% \begin{figure}[htbp]
%     \centering
%     \includegraphics[width=0.9\linewidth]{error_log_Y_rob.pdf}
%     \caption{The trajectory of (a) $\psi_{Y_1}$, (b) $\psi_{Y_2}$, and (c) $\psi_{Y_3}$ with the homogeneous controller \eqref{eq:consensus_MRS} and its linear counterpart in the presence of the transmission noise and the model uncertainty.}
%     \label{fig:error_log_Y_rob}
% \end{figure}













